Causal Discovery via Conditional Independence Testing with Proxy Variables

Distinguishing causal connections from correlations is important in many scenarios. However, the presence of unobserved variables, such as the latent confounder, can introduce bias in conditional independence testing commonly employed in constraint-based causal discovery for identifying causal relations. To address this issue, existing methods introduced proxy variables to adjust for the bias caused by unobserveness. However, these methods were either limited to categorical variables or relied on strong parametric assumptions for identification. In this paper, we propose a novel hypothesis-testing procedure that can effectively examine the existence of the causal relationship over continuous variables, without any parametric constraint. Our procedure is based on discretization, which under completeness conditions, is able to asymptotically establish a linear equation whose coefficient vector is identifiable under the causal null hypothesis. Based on this, we introduce our test statistic and demonstrate its asymptotic level and power. We validate the effectiveness of our procedure using both synthetic and real-world data.

==> icml24_app/old_versions/completeness.tex <==
\newpage
\section{Rank preservation in discretization}

\subsection{Proof of Example~\ref{exam.comp}: Characterization of completeness}

\begin{assumption}[Completeness]
    We assume the conditional distribution $\mathcal{L}_{U|X}$ is complete. That is, for any measurable function $g$, $E[g(u)|x]=0$ a.s. (for all $x$) \xw{we do not need to highlight ``for all $x$", as $E[g(u)|x]$ is the function of $x$ by definition. We do not need to highlight something that has confused us:)} if and only if $g(u)=0$ a.s. We also assume $\mathcal{L}_{W|X}$ is complete.
    \label{asm.comp}
\end{assumption}

\begin{example}[Addictive noise model with completeness]
    Suppose that random variables $X,U,W$ satisfy the addictive noise model $U=m_1(X)+V_1$, $W=m_2(U)+V_2$, where $V_1,V_2$ are noise variables. If the ranges of $m_1,m_2$ are both $\mathbb{R}$ and the characterization functions of $V_1,V_2$ are both non-zero, then $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|X}$ are both complete.
    \label{exam.comp}
\end{example}

\begin{proof}
    We first show $\mathcal{L}_{U|X}$ is complete. To this end, we show $E[g(u)|x]=0$ a.s. means $g(u)=0$ a.s. Specifically, denote $h(x):=f_{V_1}(-x)$, we have $E[g(u)|x]=\int g(u)f_{V_1}(u-m_1(x))du = \int g(u)h(m_1(x)-u)du=\{g*h\} (m_1(x))$, where $*$ denotes the convolution operator. Since the range of $m_1(x)$ is $\mathbb{R}$, $E[g(u)|x]=0$ a.s. means $g*h=0$ a.s. Applying the convolution theorem, we have $\hat{g} \cdot \hat{h}=0$ a.s., where $\hat{g},\hat{h}$ are (respectively) \xw{respectively} Fourier transforms of $g,h$. Since the characterization function of $V_1$ is non-zero, we have $\hat{h}>0$ and hence $\hat{g}=0$ a.s. Applying the inverse Fourier transform, we have $g=0$ a.s., which means $\mathcal{L}_{U|X}$ is complete.

    Similarly, we can show that $\mathcal{L}_{W|U}$ is complete. Next, given that $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|U}$ are both complete, we show $\mathcal{L}_{W|X}$ is also complete. Specifically, we have $E[g(w)|x]=\int g(w)f_{W|X}(w|x) dw = \iint g(w)f_{W|U}(w|u)dw f_{U|X}(u|x) du = 0$ a.s. if and only if $\int g(w)f_{W|U}(w|u)dw = 0$ a.s. (since $\mathcal{L}_{U|X}$ is complete) \xw{we should not put important clues or notes in brackets. Specifically, ..., if and only if $\int g(w)f_{W|U}(w|u)dw = 0$ a.s., because $\mathcal{L}_{U|X}$ is complete.}
    Because $\mathcal{L}_{W|U}$ is also complete, we have $\int g(w)f_{W|U}(w|u)dw = 0$ a.s. if and only if $g(w)=0$ a.s. Therefore, we have $E[g(w)|x]=0$ a.s. if and only if $g(w)=0$ a.s., which concludes the proof.
\end{proof}

\xw{can we obtain similar conclusions when $U$ is confounder?}\textcolor{blue}{yes, but the conditions are a bit different, is it necessary to mention details? (in the main text)} \xw{no need in the main text, just appendix and ``refer to appendix" in main text is OK:)}

\subsection{Proof of Proposition~\ref{prop.rank-dis}: Rank preserving discretization}

\begin{proposition}[Rank preserving discretization]
    Suppose Assumption~\ref{asm.comp} holds, then for any partition $\{\mathcal{W}_l\}_{l=1}^L$ of $\mathcal{W}$, there exists a partition $\{\mathcal{X}_i\}_{i=1}^I$ of $\mathcal{X}$ (with $I\geq L$) such that the discretized variables $\tilde{W},\tilde{X}$ have a transition matrix $P(\tilde{W}|\tilde{X})$ with full row rank. Similarly, there also exists a partition $\{\mathcal{U}_k\}_{k=1}^K$ of $\mathcal{U}$ (with $K=L$) such that the matrix $P(\tilde{W}|\tilde{U})$ is invertible.
    \label{prop.rank-dis}
\end{proposition}

\begin{proof}
    We show that for any partition $\{\mathcal{W}_l\}_{l=1}^L$, there exists a partition $\{\mathcal{X}_i\}_{i=1}^I$ (with $I\geq L$) such that the matrix $P(\tilde{W}|\tilde{X})$ has rank $L$. To this end \xw{delete}, the proof consists of two parts: in part 1., we first show for any $\{\mathcal{W}_l\}_{l=1}^L$, the set of functions (of $x$'s) \xw{delete} $\{f_{W|X}(W\in\mathcal{W}_l|x)\}_{l=1}^L$ are linear independent. Then, in part 2., we use this conclusion to construct  $I$ points $\{x_i\}_{i=1}^I$ (therefore the partition $\{\mathcal{X}_i\}_{i=1}^I$) such that the matrix $P(\tilde{W}|\tilde{X})$ has rank $L$.

    Part 1. We first show for any $\{\mathcal{W}_l\}_{l=1}^L$, the functions $\{f_{W|X}(W\in\mathcal{W}_l|x)\}_{l=1}^L$ are linear independent. Prove by contradiction. Suppose that there exists a partition $\{\mathcal{W}_l\}_{l=1}^L$ such that the functions $\{f_{W|X}(W\in\mathcal{W}_l|x)\}_{l=1}^L$ are linear dependent. That is, there are $L$ numbers $\{a_l\}_{l=1}^L$ that are not all zero such that $\sum_{l=1}^L a_l f_{W|X}(W\in\mathcal{W}_l|x) = 0$. Let $g(w)$ be the piece-wise constant function defined by $g(w):=a_l, w\in\mathcal{W}_l$, we then have $\int_{\mathcal{W}} g(w) f_{W|X}(w|x)=0$. Since $g(w)\neq 0$, this contradicts with the completeness of $\mathcal{L}_{W|X}$ in Assumption~\ref{asm.comp}.

    We then show for any $\{\mathcal{W}_l\}_{l=1}^L$, the functions $\{F_l(x):=F_{X|W}(x|W\in\mathcal{W}_l)\}_{l=1}^L$ are linear independent. To see this, note that the linear independence of $\{f_{W|X}(W\in\mathcal{W}_l|x)\}_{l=1}^L$ (which has been proved in part 1.) derives that of \xw{implies independence of} $\{f_{X|W}(x|W\in\mathcal{W}_l)\}_{l=1}^L$ by Bayes' theorem, and that the linear independence of $\{f_{X|W}(x|W\in\mathcal{W}_l)\}_{l=1}^L$ derives that of $\{F_{X|W}(x|W\in\mathcal{W}_l)\}_{l=1}^L$ due to the relation \xw{given that} $f_{X|W}(x|W\in\mathcal{W}_l)=F^\prime_{X|W}(x|W\in\mathcal{W}_l)$.

    Part 2. Given that $\{F_l(x)\}_{l=1}^L$ are linear independent, we show there exists $I$ points $\{x_i\}_{i=1}^I$ such that the matrix $P(\tilde{W}|\tilde{X})$ has rank $L$. For this purpose, we show there exists $I$ points such that the vectors $F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})$ (where $F_l(\boldsymbol{x}):=[F_l(x_1),...,F_l(x_I)]^T$) are linear independent. Since $\mathrm{rank}(P(\tilde{W}|\tilde{X}))=\mathrm{rank}(P(\tilde{X}|\tilde{W}))=\mathrm{rank}([F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})])$, this means $\mathrm{rank}(P(\tilde{W}|\tilde{X}))=L$ and concludes the proof.
    
    We first show the case where $I=L$. Denote the matrix $M_L=[F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})]$. We show $F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})$ are linear independent by showing $\mathrm{det}(M_L)\neq 0$. Prove by induction over $L$:
    
    (1) Base: when $L=1$, we have $\exists x_1, F_1(x_1)\neq0$. Therefore, we have $\mathrm{det}(M_1)=F_1(x_1)\neq 0$. 
    
    (2) Induction hypothesis: assume that for any $L-1$ linear independent functions $F_1,...,F_{L-1}$, there exists $L-1$ points $x_1,...,x_{L-1}$ such that $\mathrm{det}(M_{L-1})\neq 0$. 
    
    (3) Induction: show that for any $L$ linear independent functions $F_1,...,F_L$, there exists $L$ points $x_1,...,x_L$ such that $\mathrm{det}(M_L)\neq 0$. To this end, we first have the Laplace expansion of the matrix determinant $\mathrm{det}(M_L)=\sum_{l=1}^L (-1)^{1+l} \mathrm{det}(A_l^L) F_l(x_L)$, where $A_{L,l}$ denotes the matrix obtained by removing the $L$-th row and $l$-th column from $M_L$. That is, $A_{L,l}=[F_1(\boldsymbol{x}^\prime),...,F_{l-1}(\boldsymbol{x}^\prime),F_{l+1}(\boldsymbol{x}^\prime),...,F_L(\boldsymbol{x}^\prime)]$, where $F_l(\boldsymbol{x}^\prime)=[F_l(x_1),...,F_l(x_{L-1})]^T$. Then, since $F_1,...,F_{l-1},F_{l+1},...,F_L$ are $L-1$ linear independent functions, according to the induction hypothesis, there exists $L-1$ points $x_1,...,x_{L-1}$ such that $\mathrm{det}(A_{L,l})\neq 0$. That is, at least one of the cofactors $(-1)^{1+l} \mathrm{det}(A_l)$ in the expansion is not zero. Finally, since $F_1,...,F_L$ are linear independent, there exists $x_L$ such that $\mathrm{det}(M_L)=\sum_{l=1}^L (-1)^{1+l} \mathrm{det}(A_{L,l}) F_l(x_L) \neq 0$, which concludes the induction.

    For cases where $I>L$, We have $F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})$ (where $F_l(\boldsymbol{x}):=[F_l(x_1),...,F_l(x_I)]^T$) are linear independent as long as their truncated versions $F_1(\boldsymbol{x}^\prime),...,F_L(\boldsymbol{x}^\prime)$ (where $F_l(\boldsymbol{x}^\prime):=[F_l(x_1),...,F_l(x_L)]^T$) are linear independent.

    Below, we show for any partition $\{\mathcal{W}_l\}_{l=1}^L$, there exists a partition $\{\mathcal{U}_k\}_{k=1}^K$ (with $K=L$) such that the matrix $P(\tilde{W}|\tilde{U})$ is invertible. We show this by showing that under Assumption~\ref{asm.comp}, $\mathcal{L}_{W|U}$ is complete (then, repeating the proof above derives the invertibility of $P(\tilde{W}|\tilde{U})$) \xw{then we can similarly have $P(\tilde{W}|\tilde{U})$ is invertible}. Specifically, the completeness of $\mathcal{L}_{W|X}$ implies $E\{g(w)|x\} = \int g(w) f(w|x) dw = \iint g(w)f(w|u) dw f(u|x) du = 0$ a.s. if and only if $g(w)=0$ a.s. Since $\mathcal{L}_{U|X}$ is also assumed complete, we have $\iint g(w)f(w|u) dw f(u|x) du = 0$ a.s. if and only if $\int g(w)f(w|u) dw = 0$ a.s. Therefore, we have $\int g(w)f(w|u) dw = 0$ a.s. if and only if $g(w)=0$ a.s., which concludes the proof.

    
\end{proof}

\subsection{Algorithm~\ref{alg.dis}: Discretization with rank preservation}

Denote $F_l(x):=\mathbb{P}(X\leq x|W\in\mathcal{W}_l)$ the conditional cdf of $X$ given $W\in\mathcal{W}_l$. For the vector $\boldsymbol{x}:=[x_1,...,x_I]^T$, denote $F_l(\boldsymbol{x}):=[F_l(x_1),...,F_l(x_I)]^T$ as the column vector, $M_L(\boldsymbol{x}):=[F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})]$ as the matrix, and $M_{L\backslash l}(\boldsymbol{x})$ as the matrix obtained after removing the $l$-th column from $M_L(\boldsymbol{x})$.


\begin{algorithm}[h]
   \caption{Rank preserving discretization}
   \label{alg.dis}
\begin{flushleft}
\textbf{Input:} Observation data of $X$ and $W$. \\
\textbf{Output:} Discretization bins $\{\mathcal{X}_i\}_{i=1}^I$ and $\{\mathcal{W}_l\}_{l=1}^L$.
\end{flushleft}
\begin{algorithmic}[1]
    \STATE Set $\{\mathcal{W}_l\}_{l=1}^L\leftarrow \text{quantile\_bins}(\mathcal{W})$.
    \STATE Estimate $F_1(x),...,F_L(x)$.
    \STATE Search for $x_1$ satisfying $F_1(x_1)\neq 0$.
    \FOR{$l=2,...,L$}
        \STATE Set $a_m \leftarrow (-1)^{1+m} \mathrm{det}(M_{l\backslash m}([x_1,...,x_{l-1}]^T))$ for $m=1,...,l$.
        \STATE Search for $x_l$ satisfying $\sum_{m=1}^l a_m F_m(x)\neq 0$.
    \ENDFOR
    
    
    \STATE Set $\{\mathcal{X}_i\}_{i=1}^{L-1}\leftarrow \{[x_i,x_{i+1}]\}_{i=1}^{L-1}$ and set $\{\mathcal{X}_i\}_{i=L}^I \leftarrow \text{quantile\_bins}(\mathcal{X}\backslash [x_1,x_L])$.
    \STATE \textbf{return} $\{\mathcal{X}_i\}_{i=1}^I$,$\{\mathcal{W}_l\}_{l=1}^L$.
\end{algorithmic}
\end{algorithm}


\subsection{Extra examples of completeness}
\label{app-sec.example-comp}

% \begin{algorithm}[h]
%    \caption{Rank preserving discretization}
%    \label{alg.dis}
% \begin{flushleft}
% \textbf{Input:} Observation data of $X$ and $W$. \\
% \textbf{Output:} Discretization bins $\{\mathcal{X}_i\}_{i=1}^I$ and $\{\mathcal{W}_l\}_{l=1}^L$.
% \end{flushleft}
% \begin{algorithmic}[1]
%     \STATE $\{\mathcal{W}_l\}_{l=1}^L\leftarrow \text{quantile\_bins}(\mathcal{W})$.
%     \STATE Estimate $F_1(x),...,F_L(x)$.
    
%     \FUNCTION{$\text{find}(L)$}
%         \IF{$L=1$}
%             \STATE Search for $x$ satisfying $F_1(x)\neq 0$.
%             \STATE \textbf{return} $x$.
%         \ELSE
%             \STATE $x_1,...,x_{L-1} \leftarrow \text{find}(L-1)$.
%             \STATE Compute cofactors $a_l = (-1)^{1+l} \mathrm{det}(M_{L\backslash l}([x_1,...,x_{L-1}]^T))$.
%             \STATE Search for $x$ satisfying $\sum_{l=1}^L a_l F_l(x)\neq 0$.
%             \STATE \textbf{return} $x_1,...,x_{L-1},x$.
%         \ENDIF
%     \ENDFUNCTION

%     \STATE $x_1,...,x_L \leftarrow \text{find}(L)$.
%     \STATE For $i=1,...,L-1$, $\mathcal{X}_i\leftarrow[x_i,x_{i+1}]$; For $i=L,...,I$, $\mathcal{X}_i \leftarrow \text{quantile\_bins}(\mathcal{X}\backslash [x_1,x_L])$
%     \STATE \textbf{return} $\{\mathcal{X}_i\}_{i=1}^I,\{\mathcal{W}_l\}_{l=1}^L$.
% \end{algorithmic}
% \end{algorithm}

==> icml24_app/old_versions/completeness_xw.tex <==
\section{Rank preservation in discretization}

\subsection{Proof of Example~\ref{exam.comp}: Characterization of completeness}
\label{app-sec.example-comp}

\begin{assumption}[Completeness]
    We assume the conditional distribution $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|X}$ are complete. That is, for any measurable function $g$, 
    \begin{itemize}[topsep=1em]
    \itemsep0em
        \item $\mathbb{E}[g(u)|x]=0$ almost surely if and only if $g(u)=0$ almost surely. 
        \item $\mathbb{E}[g(w)|x]=0$ almost surely if and only if $g(w)=0$ almost surely.
    \end{itemize}
    \label{asm.comp}
\end{assumption}

\begin{example}[Addictive noise model when $U$ is a mediator]
    Suppose the mediation model $X \to U \to W$ satisfies the addictive noise model $U=m_1(X)+V_1$, $W=m_2(U)+V_2$, where $V_1,V_2$ are noise variables. If the ranges of $m_1,m_2$ are both $\mathbb{R}$ and the characterization functions of $V_1,V_2$ are both non-zero, then $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|X}$ are both complete.
    \label{exam.comp}
\end{example}

\begin{proof}
    We first show $\mathcal{L}_{U|X}$ is complete. Denote $h(x):=f_{V_1}(-x)$, we have 
    \begin{align*}
        \mathbb{E}[g(u)|x]=\int g(u)f_{V_1}(u-m_1(x))du = \int g(u)h(m_1(x)-u)du=\{g*h\} (m_1(x)),
    \end{align*}
     where $*$ denotes the convolution operator. Since the range of $m_1(x)$ is $\mathbb{R}$, $\mathbb{E}[g(u)|x]=0$ a.s. means $g*h=0$ a.s. Applying the convolution theorem, we have $\hat{g} \cdot \hat{h}=0$ a.s., where $\hat{g},\hat{h}$ are respectively Fourier transforms of $g,h$. Since the characterization function of $V_1$ is non-zero, we have $\hat{h}>0$ and hence $\hat{g}=0$ a.s. Applying the inverse Fourier transform, we have $g=0$ a.s., which means $\mathcal{L}_{U|X}$ is complete.

    Similarly, we can prove $\mathcal{L}_{W|U}$ is complete. Next, given that $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|U}$ are both complete, we show $\mathcal{L}_{W|X}$ is also complete. Specifically, we have 
    \begin{align*}
        \mathbb{E}[g(w)|x]=\int g(w)f_{W|X}(w|x) dw = \iint g(w)f_{W|U}(w|u)dw f_{U|X}(u|x) du = 0 \text{ a.s. }
    \end{align*}
    if and only if $\int g(w)f_{W|U}(w|u)dw = 0$ a.s., because $\mathcal{L}_{U|X}$ is complete. As $\mathcal{L}_{W|U}$ is also complete, we have $\int g(w)f_{W|U}(w|u)dw = 0$ a.s. if and only if $g(w)=0$ a.s. Therefore, we have $\mathbb{E}[g(w)|x]=0$ a.s. if and only if $g(w)=0$ a.s., which concludes the proof.
\end{proof}


\begin{example}[Additive Noise Model when $U$ is a confounder]
\label{exam.confound}
    Suppose the confounding model $X\leftarrow U \to W$ satisfies the following structural equation model $X = m_1(U) + V_1,  W = m_2(U)+V_2$. Further, we assume they satisfy the following conditions:
    \begin{enumerate}[topsep=0em]
    \itemsep0em
        \item the characterization functions of $V_1,V_2$ are non-zero, 
        \item the support of $U$ and the range of $m_2$ are both $\mathbb{R}$, and
        \item $m_1$ is strictly monotonous and its derivative is non-zero almost everywhere. 
    \end{enumerate}
\end{example}

\begin{remark}
    The monotonicity condition of $m_1$ is to ensure that $f_{U|X}(u|x)$ can be written in a closed form. 
\end{remark}


\begin{proof}
    Similar to the proof in the example~\ref{exam.confound}, we have the completeness for $\mathcal{L}(W|U)$. Besides, if we can prove the completeness for $\mathcal{L}(U|X)$, we can have the completeness of $E\{g(w)|x\}$, following the procedure in the mediation model. 
    

    To show $\mathcal{L}(W|U)$ is complete, note that we have $f_{U|X}(u|x) = f_V(x-m(u))|m^\prime(u)|$. Therefore, the completeness of $E\{g(u)|x\}$ means
    \begin{align*}
        \int g(u)|m^\prime(u)| f_V(x-m(u))du = 0 \text{ a.s. if and only if } g(u) = 0 \text{ a.s. }
    \end{align*}
    Denote $g_1(u):=g(u)|m^\prime(u)|$. We first show that $g_1(u) = 0$ a.s. Let $t=m(u)$ and hence $u=m_1^{-1}(t)$. Further denote $h(t)=m_1^{-1}(t)$ with $h^\prime(t)=\frac{1}{m_1^\prime(m_1^{-1}(t))}\neq 0$. Then, we have:
    \begin{equation*}
        \int g_1(u) f_V(x-m(u)) du = \int g_1(h(t)) h^\prime(t) f_V(x-t) dt.
    \end{equation*}
    Since $V$ has a non-zero characteristic function, we first have $\int g_1(h(t)) h^\prime(t) f_V(x-t) dt =0$ implies $g_1(h(t)) h^\prime(t) = 0$. Since $h^\prime(t)\neq 0$, we then have $g_1(h(t))=g_1(m^{-1}(t))=0$. Since $u$ takes values in $\mathbb{R}$, the range of $m_1^{-1}$ is $\mathbb{R}$, and therefore $g_1=0$. Since $m_1'(u) \neq 0$ a.s., we have $g(u) = 0$ a.s.


\end{proof}


\subsection{Proof of Proposition~\ref{prop.rank-dis}: Rank preserving discretization}
\label{app-sec.discrete}



\begin{proposition}[Rank preserving discretization]
    Suppose Assumption~\ref{asm.comp} holds, then for any partition $\{\mathcal{W}_l\}_{l=1}^L$ of $\mathcal{W}$, there exists a partition $\{\mathcal{X}_i\}_{i=1}^I$ of $\mathcal{X}$ with $I\geq L$, such that the discretized variables $\tilde{W},\tilde{X}$ have a transition matrix $P(\tilde{W}|\tilde{X})$ with full row rank. Similarly, there also exists a partition $\{\mathcal{U}_k\}_{k=1}^K$ of $\mathcal{U}$ (with $K=L$) such that the matrix $P(\tilde{W}|\tilde{U})$ is invertible.
    \label{prop.rank-dis}
\end{proposition}

\begin{proof}
    We show that for any partition $\{\mathcal{W}_l\}_{l=1}^L$, there exists a partition $\{\mathcal{X}_i\}_{i=1}^I$ (with $I\geq L$) such that the matrix $P(\tilde{W}|\tilde{X})$ has rank $L$. The proof contains two parts: in \textbf{part I}, we first show for any $\{\mathcal{W}_l\}_{l=1}^L$, $\{f_{W|X}(W\in\mathcal{W}_l|x)\}_{l=1}^L$ are linear independent. Then, in \textbf{part II}, we use this conclusion to construct $I$ points $\{x_i\}_{i=1}^I$ and therefore the partition $\{\mathcal{X}_i\}_{i=1}^I$, such that the matrix $P(\tilde{W}|\tilde{X})$ has rank $L$.

    \textbf{Part I}. We first show for any $\{\mathcal{W}_l\}_{l=1}^L$, the functions $\{f_{W|X}(W\in\mathcal{W}_l|x)\}_{l=1}^L$ are linear independent. Prove by contradiction. Suppose that there exists a partition $\{\mathcal{W}_l\}_{l=1}^L$ such that $\{f_{W|X}(W\in\mathcal{W}_l|x)\}_{l=1}^L$ are linear dependent. That is, there are $L$ numbers $\{a_l\}_{l=1}^L$ that are not all zero such that $\sum_{l=1}^L a_l f_{W|X}(W\in\mathcal{W}_l|x) = 0$. Let $g(w)$ be the piece-wise constant function defined by $g(w):=a_l, w\in\mathcal{W}_l$, we then have $\int_{\mathcal{W}} g(w) f_{W|X}(w|x)=0$ for all $x$. Since $g(w)\neq 0$, this contradicts with the completeness of $\mathcal{L}_{W|X}$ in Assumption~\ref{asm.comp}.

    We then show for any $\{\mathcal{W}_l\}_{l=1}^L$, the functions $\{F_l(x):=F_{X|W}(x|W\in\mathcal{W}_l)\}_{l=1}^L$ are linear independent. To see this, note that $f_{X|W}(x|W\in\mathcal{W}_l) = \frac{f_{W|X}(W\in\mathcal{W}_l|x)f_X(x)}{\mathbb{P}(W\in\mathcal{W}_l)}$, therefore it is easy to obtain the linear independence of $\{f_{X|W}(x|W\in\mathcal{W}_l)\}_{l=1}^L$ through the independence of  $\{f_{W|X}(W\in\mathcal{W}_l|x)\}_{l=1}^L$. Besides, since $f_{X|W}(x|W\in\mathcal{W}_l)=F^\prime_{X|W}(x|W\in\mathcal{W}_l)$, we can also obtain the linear independence of $\{F_{X|W}(x|W\in\mathcal{W}_l)\}_{l=1}^L$.


    \textbf{Part II}. Given that $\{F_l(x)\}_{l=1}^L$ are linear independent, we show there exists $I$ points $\{x_i\}_{i=1}^I$ such that the matrix $P(\tilde{W}|\tilde{X})$ has rank $L$. For this purpose, we only have to show that there exists $I$ points such that $L$ vectors $F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})$, where $F_l(\boldsymbol{x}):=[F_l(x_1),...,F_l(x_I)]^T$ for each $l$. If this holds, we can complete the proof by showing that
    \begin{align*}
        \mathrm{rank}(P(\tilde{W}|\tilde{X}))=\mathrm{rank}(P(\tilde{X}|\tilde{W}))=\mathrm{rank}([F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})])=L.
    \end{align*}
   
    
    We first show the case where $I=L$. Denote the matrix $M_L=[F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})]$. We show $F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})$ are linear independent by showing $\mathrm{det}(M_L)\neq 0$. Prove by induction over $L$:
    
    (1) Base: when $L=1$, we have $\exists x_1, F_1(x_1)\neq0$. Therefore, we have $\mathrm{det}(M_1)=F_1(x_1)\neq 0$. 
    
    (2) Induction hypothesis: assume that for any $L-1$ linear independent functions $F_1,...,F_{L-1}$, there exists $L-1$ points $x_1,...,x_{L-1}$ such that $\mathrm{det}(M_{L-1})\neq 0$. 
    
    (3) Induction: show that for any $L$ linear independent functions $F_1,...,F_L$, there exists $L$ points $x_1,...,x_L$ such that $\mathrm{det}(M_L)\neq 0$. To this end, we first have the Laplace expansion of the matrix determinant 
    \begin{align}
    \label{eq.det}
        \mathrm{det}(M_L)(x_L)=\sum_{l=1}^L (-1)^{1+l} \mathrm{det}(A_l^L) F_l(x_L),
    \end{align}
    where $A_{L,l}$ denotes the matrix obtained by removing the $L$-th row and $l$-th column from $M_L$. That is, $A_{L,l}=[F_1(\boldsymbol{x}^\prime),...,F_{l-1}(\boldsymbol{x}^\prime),F_{l+1}(\boldsymbol{x}^\prime),...,F_L(\boldsymbol{x}^\prime)]$, where $F_l(\boldsymbol{x}^\prime)=[F_l(x_1),...,F_l(x_{L-1})]^T$. Then, since $F_1,...,F_{l-1},F_{l+1},...,F_L$ are $L-1$ linear independent functions, according to the induction hypothesis, there exists $L-1$ points $x_1,...,x_{L-1}$ such that $\mathrm{det}(A_{L,l})\neq 0$. That is, at least one of the cofactors $(-1)^{1+l} \mathrm{det}(A_l)$ in the expansion is not zero. Finally, since $F_1,...,F_L$ are linear independent, there exists $x_L$ such that $\mathrm{det}(M_L)(x_L) \neq 0$ for $x_L$, which concludes the induction.

    For cases where $I>L$, We have $F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})$ (where $F_l(\boldsymbol{x}):=[F_l(x_1),...,F_l(x_I)]^T$) are linear independent since $F_1(\boldsymbol{x}^\prime),...,F_L(\boldsymbol{x}^\prime)$ (where $F_l(\boldsymbol{x}^\prime):=[F_l(x_1),...,F_l(x_L)]^T$) are linear independent.

    Below, we show for any partition $\{\mathcal{W}_l\}_{l=1}^L$, there exists a partition $\{\mathcal{U}_k\}_{k=1}^K$ (with $K=L$) such that the matrix $P(\tilde{W}|\tilde{U})$ is invertible. We prove this by showing that under Assumption~\ref{asm.comp}, $\mathcal{L}_{W|U}$ is complete. Then, repeating the proof above, we have $P(\tilde{W}|\tilde{U})$ is invertible. To show this, according to the completeness of $\mathcal{L}_{W|X}$, we have
    \begin{align}
    \label{eq.complete-w-u}
        \int g(w)p(w|x)dw = \int \left(\int g(w)p(w|u)dw \right) p(u|x)du = 0 \text{ a.s. }
    \end{align}
    if and only if $g(w) = 0$ a.s., since $\mathcal{L}_{U|X}$ is assumed to be complete, which is further equivalent to $\int g(w) p(w|u)dw = 0$ since $\mathcal{L}_{U|X}$ is complete. 

\end{proof}

\subsection{Algorithm~\ref{alg.dis}: Discretization with rank preservation}

Inspired by Prop.~\ref{prop.rank-dis}, we can iteratively find $x_1,...,x_L$ with $L < I$, such that $F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})$ are linear independent, where $F_l(\boldsymbol{x}) = [F_l(x_1),...,F_l(x_I)]^\top$ with $F_l(x_i) = \mathbb{P}(X \leq x_i | \tilde{W})$ for any $i,l$. We denote $M_L(\boldsymbol{x}):=[F_1(\boldsymbol{x}),...,F_L(\boldsymbol{x})]$ as the matrix, and $M_{L\backslash l}(\boldsymbol{x})$ as the matrix obtained after removing the $l$-th column from $M_L(\boldsymbol{x})$.



% Denote $F_l(x):=\mathbb{P}(X\leq x|W\in\mathcal{W}_l)$ the conditional cdf of $X$ given $W\in\mathcal{W}_l$. For the vector $\boldsymbol{x}:=[x_1,...,x_I]^T$, denote $F_l(\boldsymbol{x}):=[F_l(x_1),...,F_l(x_I)]^T$ as the column vector, 


\begin{algorithm}[h]
   \caption{Rank preserving discretization}
   \label{alg.dis}
\begin{flushleft}
\textbf{Input:} Observation data of $X$ and $W$. \\
\textbf{Output:} Discretization bins $\{\mathcal{X}_i\}_{i=1}^I$ and $\{\mathcal{W}_l\}_{l=1}^L$.
\end{flushleft}
\begin{algorithmic}[1]
    \STATE Set $\{\mathcal{W}_l\}_{l=1}^L\leftarrow \text{quantile\_bins}(\mathcal{W})$.
    \STATE Estimate $F_1(x),...,F_L(x)$.
    \STATE Search for $x_1$ satisfying $F_1(x_1)\neq 0$.
    \FOR{$l=2,...,L$}
        \STATE Set $a_m \leftarrow (-1)^{1+m} \mathrm{det}(M_{l\backslash m}([x_1,...,x_{l-1}]^T))$ for $m=1,...,l$.
        \STATE Search for $x_l$ satisfying $\sum_{m=1}^l a_m F_m(x)\neq 0$.
    \ENDFOR
    
    
    \STATE Set $\{\mathcal{X}_i\}_{i=1}^{L-1}\leftarrow \{[x_i,x_{i+1}]\}_{i=1}^{L-1}$ and set $\{\mathcal{X}_i\}_{i=L}^I \leftarrow \text{quantile\_bins}(\mathcal{X}\backslash [x_1,x_L])$.
    \STATE \textbf{return} $\{\mathcal{X}_i\}_{i=1}^I$,$\{\mathcal{W}_l\}_{l=1}^L$.
\end{algorithmic}
\end{algorithm}


%\subsection{Extra examples of completeness}
%\label{app-sec.example-comp}

% \begin{algorithm}[h]
%    \caption{Rank preserving discretization}
%    \label{alg.dis}
% \begin{flushleft}
% \textbf{Input:} Observation data of $X$ and $W$. \\
% \textbf{Output:} Discretization bins $\{\mathcal{X}_i\}_{i=1}^I$ and $\{\mathcal{W}_l\}_{l=1}^L$.
% \end{flushleft}
% \begin{algorithmic}[1]
%     \STATE $\{\mathcal{W}_l\}_{l=1}^L\leftarrow \text{quantile\_bins}(\mathcal{W})$.
%     \STATE Estimate $F_1(x),...,F_L(x)$.
    
%     \FUNCTION{$\text{find}(L)$}
%         \IF{$L=1$}
%             \STATE Search for $x$ satisfying $F_1(x)\neq 0$.
%             \STATE \textbf{return} $x$.
%         \ELSE
%             \STATE $x_1,...,x_{L-1} \leftarrow \text{find}(L-1)$.
%             \STATE Compute cofactors $a_l = (-1)^{1+l} \mathrm{det}(M_{L\backslash l}([x_1,...,x_{L-1}]^T))$.
%             \STATE Search for $x$ satisfying $\sum_{l=1}^L a_l F_l(x)\neq 0$.
%             \STATE \textbf{return} $x_1,...,x_{L-1},x$.
%         \ENDIF
%     \ENDFUNCTION

%     \STATE $x_1,...,x_L \leftarrow \text{find}(L)$.
%     \STATE For $i=1,...,L-1$, $\mathcal{X}_i\leftarrow[x_i,x_{i+1}]$; For $i=L,...,I$, $\mathcal{X}_i \leftarrow \text{quantile\_bins}(\mathcal{X}\backslash [x_1,x_L])$
%     \STATE \textbf{return} $\{\mathcal{X}_i\}_{i=1}^I,\{\mathcal{W}_l\}_{l=1}^L$.
% \end{algorithmic}
% \end{algorithm}

==> icml24_app/old_versions/dis_err.tex <==
\newpage
\section{Error control in discretization}

\subsection{Proof of Example~\ref{exam.tv-smooth}: Characterization of TV-smoothness}

\begin{assumption}[TV-smoothness]
    We assume the map $u\mapsto \mathcal{L}_{Y|U=u}$ is $L_Y$-Lipschitz continuous wrt the Total Variation (TV) distance, that is $\forall u,u^\prime$, we have $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime}) \leq L_Y|u-u^\prime|$. We also assume the map $u\mapsto \mathcal{L}_{W|U=u}$ is $L_W$-Lipschitz continuous.
\label{asm.tv-smooth}
\end{assumption}


\begin{example}[Addictive noise model with TV-smoothness]
    Suppose that random variables $Y,U,W$ satisfy the addictive noise model $Y=m_1(U)+V_1$, $W=m_2(U)+V_2$, where $V_1\sim f_{V_1}(v), V_2\sim f_{V_2}(v)$ are noise variables. If $m_1,m_2,f_{V_1},f_{V_2}$ are both differentiable, and $f_{V_1}^\prime,f_{V_2}^\prime$ are absolutely integrable, then $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are both Lipschitz continuous.
\label{exam.tv-smooth}
\end{example}

\begin{proof}
    We show $u\mapsto \mathcal{L}_{Y|U=u}$ is Lipschitz continuous. The Lipschitzness of $u\mapsto \mathcal{L}_{W|U=u}$ can be analogously derived. To this end \xw{replaced with ``According to the definition of TV"?} \textcolor{blue}{maybe, according to the relation between tv and l1 distance is better? this is not the definition of tv} \xw{Yes}, we first have $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime})=\frac{1}{2} \int |f_{Y|U}(y|u) - f_{Y|U}(y|u^\prime)|dy$. Since $f_{Y|U}(y|u)=f_E(y-h(u))$, we have $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime})=\frac{1}{2} \int |f_{V_1}(y-m_1(u)) - f_{V_1}(y-m_1(u^\prime))|dy$. Then, consider the map $u \mapsto f_{V_1}(y-m_1(u))$, the mean value theorem implies that $\forall u,u^\prime, \exists\, u_c \in (u,u^\prime)$ such that $|f_{V_1}(y-m_1(u)) - f_{V_1}(y-m_1(u^\prime))| = |f_{V_1}^\prime(y-m_1(u_c)) m_1^\prime(u_c)| \cdot |u-u^\prime|$. Finally, let $L_Y:= \frac{1}{2}\int |f_{V_1}^\prime(y-m_1(u_c)) m_1^\prime(u_c)| dy$, we have $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime})\leq L_Y |u-u^\prime|$, which concludes the proof.
\end{proof}


\subsection{Proof of Proposition~\ref{prop.control-err}: Discretization error control}

\begin{proposition}[Discretization error control]
    Suppose that $\{\mathcal{X}_i\}_i^I$, $\{\mathcal{Y}_j\}_j^J$, $\{\mathcal{U}_k\}_k^K, \{\mathcal{W}_l\}_{l}^L$ are (respectively) partitions of $\mathcal{X},\mathcal{Y}, \mathcal{U}$, and $\mathcal{W}$. Suppose that Assumption~\ref{asm.tv-smooth} holds, and that $len(\mathcal{U}_k) \leq \frac{1}{2} min\{\epsilon/L_Y,\epsilon/L_W\}$. Then under $\mathbb{H}_0$, we have $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|\leq \epsilon$. We also have $|\mathbb{P}(W\in\mathcal{W}_l|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(W\in\mathcal{W}_l|U\in\mathcal{U}_k)|\leq \epsilon$
\label{prop.control-err}
\end{proposition}

\begin{proof}
    We show $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|\leq \epsilon$. The control of $|\mathbb{P}(W\in\mathcal{W}_l|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(W\in\mathcal{W}_l|U\in\mathcal{U}_k)|$ can be derived in a similar way. Specifically, the proof consists of two parts. In part 1., we first show the smoothness of $u\mapsto\mathcal{L}_{Y|U=u}$ together with $\mathrm{len}(\mathcal{U}_k)\leq \epsilon/2L_Y$ implies $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k})\leq\epsilon/2$. Then, in part 2., we show \xw{provide} the control of $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|$ via that of $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k})$.

    Part 1. We show $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k})\leq\epsilon/2$. To show this, first rewrite $\mathcal{L}_{Y|U\in\mathcal{U}_k} = \dashint_{\mathcal{U}_k} \mathcal{L}_{Y|U=u} d\mathcal{L}_{U}(u)$, where $\dashint$ denotes the average integral \xw{what is the mathematical definition?}\textcolor{blue}{the average integral is a common notation? see \cite{warren2021wasserstein}, do we need to define it?} \xw{we can either define it or provide the reference. From my perspective, it is not commonly known:)}. To see this, note that for any $\mathcal{Y}_j\in\mathcal{Y}$, the LHS equals $\mathcal{L}_{Y|U\in\mathcal{U}_k}(\mathcal{Y}_j) = \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)$ \xw{this is from the definition of $\mathcal{L}$? not derivation?} and the RHS equals $\dashint_{\mathcal{U}_k} \mathcal{L}_{Y|U=u}(\mathcal{Y}_j) d\mathcal{L}_{U}(u) = {\int_{\mathcal{U}_k} \mathcal{L}_{Y|U=u}(\mathcal{Y}_j) d\mathcal{L}_{U}(u)}/{\mathbb{P}(U\in\mathcal{U}_k)} = {\mathbb{P}(Y\in\mathcal{Y}_j,U\in\mathcal{U}_k)}/{\mathbb{P}(U\in\mathcal{U}_k)}$. Therefore, LHS=RHS due to Bayes's theorem, and our rewriting is valid \xw{replaced with ``the conclusion holds"}.

    Then, due to the assumed TV-smoothness, for any $u,u^\prime\in \mathcal{U}_K$, we have $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime}) := \sup_{\mathcal{Y}_j\in \mathcal{Y}} |\mathcal{L}_{Y|U=u}(\mathcal{Y}_j)-\mathcal{L}_{Y|U=u^\prime}(\mathcal{Y}_j)| \leq L_Y|u-u^\prime|\leq \epsilon/2$. Now, for \textbf{\emph{any}} $\mathcal{Y}_j \subseteq \mathcal{Y}$, we have (note that $u$ is a fixed point and $u^\prime$ varies in the integration domain):
    \begin{align*}
        |\mathcal{L}_{Y|U=u}(\mathcal{Y}_j) &- \mathcal{L}_{Y|U\in \mathcal{U}_k}(\mathcal{Y}_j)| = \left| \mathcal{L}_{Y|U=u}(\mathcal{Y}_j) - \dashint_{\mathcal{U}_k} \mathcal{L}_{Y|U=u^\prime}(\mathcal{Y}_j) d\mathcal{L}_U(u^\prime)\right| \\
        &=\left| \dashint_{\mathcal{U}_k} \mathcal{L}_{Y|U=u}(\mathcal{Y}_j) d\mathcal{L}_U(u^\prime) - \dashint_{\mathcal{U}_k} \mathcal{L}_{Y|U=u^\prime}(\mathcal{Y}_j) d\mathcal{L}_U(u^\prime)\right| && \text{\#} \dashint_{\mathcal{U}_k} d\mathcal{L}_U(u^\prime) = 1 \\
        &\leq \dashint_{\mathcal{U}_k} \left| \mathcal{L}_{Y|U=u}(\mathcal{Y}_j) - \mathcal{L}_{Y|U=u^\prime}(\mathcal{Y}_j)\right| d\mathcal{L}_U(u^\prime) && \text{\# Triangle inequity} \\
        &\leq \dashint_{\mathcal{U}_k} \epsilon/2 \, d\mathcal{L}_U(u^\prime) = \epsilon/2, 
    \end{align*}
    which means $\sup_{\mathcal{Y}_j\in\mathcal{Y}} |\mathcal{L}_{Y|U=u}(\mathcal{Y}_j)-\mathcal{L}_{Y|U\in\mathcal{U}_k}(\mathcal{Y}_j)| =: \mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k}) \leq \epsilon/2$.

    In a similar way, we can prove $\mathrm{TV}(\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u},\mathcal{L}_{Y|X\in\mathcal{X}_i,U\in\mathcal{U}_k})\leq\epsilon/2$. To be specific, under $\mathbb{H}_0:X\ind Y|U$, we have $\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u}=\mathcal{L}_{Y|U=u}$ for any $\mathcal{X}_i\subseteq\mathcal{X}$. As a result, the map $u\mapsto \mathcal{L}_{Y|X\in\mathcal{X}_i,U=u}$ is also $L_Y$-Lipschitz continuous wrt TV distance. Now, repeat \xw{similar to} the proof above, we have $\mathrm{TV}(\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u},\mathcal{L}_{Y|X\in\mathcal{X}_i,U\in\mathcal{U}_k})\leq\epsilon/2$.

    Part 2. We show $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|\leq \epsilon$. Specifically, since $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k}) \leq \epsilon/2$, we have $|\mathbb{P}(Y\in\mathcal{Y}_j|U=u) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|\leq \epsilon/2$. Since $\mathrm{TV}(\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u},\mathcal{L}_{Y|X\in\mathcal{X}_i,U\in\mathcal{U}_k})\leq \epsilon/2$, we also have $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U=u) - \mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k)|\leq \epsilon/2$. Moreover, under $\mathbb{H}_0:X\ind Y|U$, $\mathbb{P}(Y\in\mathcal{Y}_j|U=u)=\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U=u)$. Therefore, according to the triangle inequity, we have $|\mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k)| \leq \epsilon$.
\end{proof}

\subsection{Definition~\ref{def.tight}: Tightness of distribution}

\begin{definition}[Tightness of distribution] We say the marginal distribution $\mathcal{L}_U$ is tight if $\forall \epsilon>0, \exists T, \forall t\geq T,\mathbb{P}(|U|\geq t)\leq \epsilon$. We say the conditional distribution $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$ if $\forall \epsilon>0, \exists T, \forall t\geq T, \forall x\in [a,b],$ we have $\mathbb{P}(|U|\geq t|x)\leq \epsilon$.
\label{def.tight}
\end{definition}

\begin{remark}
    We use the term ``uniform'' because the $T$ holds uniformly for all $x\in[a,b]$. As we will show below, this uniform tightness is a mild condition (though one can image that uniform tightness for all $x\in \mathbb{R}$ is a strong one).
\end{remark}

\begin{example}[Addictive noise model with uniform tightness]
    Suppose that random variables $X,U$ satisfy the additive noise model $U=m(X)+V$, where $V$ is the noise variable. If $m$ is bounded in $[a,b]$ and $\mathcal{L}_V$ is tight, then $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$.
\end{example}

\begin{proof}
    We prove with definition. Specifically, given $\mathcal{L}_V$ is tight, we first have $\forall \epsilon>0, \exists T, \forall t\geq T, \int_t^\infty f_V(v)dv \leq \epsilon$. Since $m$ is bounded, we have $\exists\, H, \forall x\in [a,b], |m(x)|\leq H$. Then, to show the uniform tightness of $\mathcal{L}_{U|X}$, note that $\forall \epsilon>0, \exists S:=T+H, \forall s>S,$ we have $\int_{s}^\infty f_{U|X}(u|x) du = \int_s^\infty f_V(u-m(x)) du = \int_{s-m(x)}^\infty f_V(v) dv \leq \epsilon$, where we use the fact that $s\geq T + H \geq T + |m(x)| \geq T + h(x)$ therefore  $s-m(x)\geq T$.
\end{proof}

\subsection{Proposition~\ref{prop.dis-err unbd}: Discretization error control; continue}

\begin{proposition}[Discretization error control; continue]
    Suppose that $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$, the map $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz continuous wrt TV distance, and that  $len(\mathcal{X}_i)\leq \epsilon/2L_U$. Then, $\forall\epsilon>0, \exists T, \forall t\geq T$, \xw{for each $\mathcal{X}_i$?}\mz{yes. Is it necessary to write ``for each xi,yj,i,j,k, ect'' everywhere we need them? (in other theorems)} \xw{just $\forall \mathcal{X}_i, \mathcal{Y}_j$} we have $\mathbb{P}(Y\in \mathcal{Y}_j,|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon$ and $\mathbb{P}(W\in \mathcal{W}_l,|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon$.
    \label{prop.dis-err unbd}
\end{proposition}

\begin{proof}
    We show $\mathbb{P}(Y\in \mathcal{Y}_j,|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon$. The control of $\mathbb{P}(W\in \mathcal{W}_l,|U|\geq t|X\in\mathcal{X}_i)$ can be derived analogously. \xw{we only provide the proof of ..., as ... can be derived analogously}. We show this \xw{We obtain this conclusion} by showing $\mathbb{P}(|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon$ and using the fact that $\mathbb{P}(Y\in \mathcal{Y}_j,|U|\geq t|X\in\mathcal{X}_i) = \mathbb{P}(Y\in \mathcal{Y}_j||U|\geq t,X\in\mathcal{X}_i) \mathbb{P}(|U|\geq t|X\in\mathcal{X}_i) \leq \mathbb{P}(|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon$. Specifically, given $\mathcal{L}_{U|X}$ is uniformly tight, we first have $\forall \epsilon/2>0, \exists T_1, \forall t\geq T_1, \forall x\in \mathcal{X}_i, \mathbb{P}(|U|\geq t|x) \leq \epsilon/2$. Then, since $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz, we have $\forall \epsilon/2>0, |\mathbb{P}(|U|>t|x) - \mathbb{P}(|U|>t|\mathcal{X}_i)|\leq \epsilon/2$ for $x\in\mathcal{X}_i$. Finally, the triangle inequity implies $\mathbb{P}(|U|>t|\mathcal{X}_i)\leq \epsilon$.
\end{proof}


\subsection{Extra examples of TV-smoothness}

==> icml24_app/old_versions/dis_err_xw.tex <==
\section{Error control in discretization}

\subsection{Proof of Example~\ref{exam.tv-smooth}: Characterization of TV-smoothness}
\label{app-sec.tv-example}

\begin{assumption}[TV-smoothness]
    We assume the map $u\mapsto \mathcal{L}_{Y|U=u}$ is $L_Y$-Lipschitz continuous with respect to the Total Variation (TV) distance, that is $\forall u,u^\prime$, we have $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime}) \leq L_Y|u-u^\prime|$. Similarly, we also assume the map $u\mapsto \mathcal{L}_{W|U=u}$ is $L_W$-Lipschitz continuous.
\label{asm.tv-smooth}
\end{assumption}


\begin{example}[Addictive noise model with TV-smoothness]
    Suppose that random variables $Y,U,W$ satisfy the addictive noise model $Y=m_1(U)+V_1$, $W=m_2(U)+V_2$, where $V_1\sim f_{V_1}(v), V_2\sim f_{V_2}(v)$ are noise variables. If $m_1,m_2,f_{V_1},f_{V_2}$ are both differentiable, and $f_{V_1}^\prime,f_{V_2}^\prime$ are absolutely integrable, then $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are both Lipschitz continuous.
\label{exam.tv-smooth}
\end{example}
\begin{proof}
    We show $u\mapsto \mathcal{L}_{Y|U=u}$ is Lipschitz continuous, and the Lipschitzness of $u\mapsto \mathcal{L}_{W|U=u}$ can be similarly derived. According to the definition of Total Variation distance, we have:
    \begin{align*}
        \mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime}) & =\frac{1}{2} \int |f_{Y|U}(y|u) - f_{Y|U}(y|u^\prime)|dy, \\
        & \overset{(1)}{=} \frac{1}{2} \int |f_{V_1}(y-m_1(u)) - f_{V_1}(y-m_1(u^\prime))|dy, \\
        & \overset{(2)}{=} \int \frac{1}{2} |f_{V_1}^\prime(y-m_1(u_c)) m_1^\prime(u_c)| \cdot |u-u^\prime| dy
    \end{align*}
    for some $u_c \in (u,u^\prime)$, where ``(1)" is due to ANM that can write $f_{Y|U}(y|u)$ as $f_E(y-h(u))$ and ``(2)" is due to the mean value theorem. Let $L_Y:= \frac{1}{2}\int |f_{V_1}^\prime(y-m_1(u_c)) m_1^\prime(u_c)| dy$, we have $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime})\leq L_Y |u-u^\prime|$, which concludes the proof.
\end{proof}

\begin{example}
    TV for the mediation case
\end{example}


\subsection{Proof of Proposition~\ref{prop.control-err}: Discretization error control}

\begin{proposition}[Discretization error control]
    Suppose that $\{\mathcal{X}_i\}_i^I$, $\{\mathcal{Y}_j\}_j^J$, $\{\mathcal{U}_k\}_k^K, \{\mathcal{W}_l\}_{l}^L$ are (respectively) partitions of $\mathcal{X},\mathcal{Y}, \mathcal{U}$, and $\mathcal{W}$. Suppose that Assumption~\ref{asm.tv-smooth} holds, and that $len(\mathcal{U}_k) \leq \frac{1}{2} min\{\epsilon/L_Y,\epsilon/L_W\}$. Then under $\mathbb{H}_0$, we have $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|\leq \epsilon$. We also have $|\mathbb{P}(W\in\mathcal{W}_l|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(W\in\mathcal{W}_l|U\in\mathcal{U}_k)|\leq \epsilon$.
\label{prop.control-err}
\end{proposition}
\begin{proof}
    We only show $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|\leq \epsilon$, since the bound of $|\mathbb{P}(W\in\mathcal{W}_l|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(W\in\mathcal{W}_l|U\in\mathcal{U}_k)|$ can be derived similarly. The proof contains two parts. In \textbf{part I}, we show the smoothness of $u\mapsto\mathcal{L}_{Y|U=u}$, which together with $\mathrm{len}(\mathcal{U}_k)\leq \epsilon/2L_Y$, implies $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k})\leq\epsilon/2$. Then, in \textbf{part II}, we control $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|$ via that of $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k})$.

    \textbf{Part I}. We show $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k})\leq\epsilon/2$. Note that we first have 
    \begin{align*}
        \mathcal{L}_{Y|U\in\mathcal{U}_k} = \dashint_{\mathcal{U}_k} \mathcal{L}_{Y|U=u} d\mathcal{L}_{U}(u) := \frac{\int_{\mathcal{U}_k} \mathcal{L}_{Y|U=u} d\mathcal{L}_{U}(u)}{\int_{\mathcal{U}_k} d\mathcal{L}_{U}(u)},
    \end{align*}
where $\dashint$ denotes the average integral \cite{warren2021wasserstein}. To see this, according to the definition of $\mathcal{L}$, for any $\mathcal{Y}_j\in\mathcal{Y}$, the LHS equals $\mathcal{L}_{Y|U\in\mathcal{U}_k}(\mathcal{Y}_j) = \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)$, and the RHS equals ${\int_{\mathcal{U}_k} \mathcal{L}_{Y|U=u}(\mathcal{Y}_j) d\mathcal{L}_{U}(u)}/{\mathbb{P}(U\in\mathcal{U}_k)} = {\mathbb{P}(Y\in\mathcal{Y}_j,U\in\mathcal{U}_k)}/{\mathbb{P}(U\in\mathcal{U}_k)}=\mathrm{LHS}$.

    Then, due to the assumed TV-smoothness, for any $u,u^\prime\in \mathcal{U}_K$, we have $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime}) := \sup_{\mathcal{Y}_j\in \mathcal{Y}} |\mathcal{L}_{Y|U=u}(\mathcal{Y}_j)-\mathcal{L}_{Y|U=u^\prime}(\mathcal{Y}_j)| \leq L_Y|u-u^\prime|\leq \epsilon/2$. Now, for \textbf{\emph{any}} $\mathcal{Y}_j \subseteq \mathcal{Y}$, we have (note that $u$ is a fixed point and $u^\prime$ varies in the integration domain):
    \begin{align*}
        |\mathcal{L}_{Y|U=u}(\mathcal{Y}_j) &- \mathcal{L}_{Y|U\in \mathcal{U}_k}(\mathcal{Y}_j)| = \left| \mathcal{L}_{Y|U=u}(\mathcal{Y}_j) - \dashint_{\mathcal{U}_k} \mathcal{L}_{Y|U=u^\prime}(\mathcal{Y}_j) d\mathcal{L}_U(u^\prime)\right| \\
        &=\left| \dashint_{\mathcal{U}_k} \mathcal{L}_{Y|U=u}(\mathcal{Y}_j) d\mathcal{L}_U(u^\prime) - \dashint_{\mathcal{U}_k} \mathcal{L}_{Y|U=u^\prime}(\mathcal{Y}_j) d\mathcal{L}_U(u^\prime)\right| && \text{\#} \dashint_{\mathcal{U}_k} d\mathcal{L}_U(u^\prime) = 1 \\
        &\leq \dashint_{\mathcal{U}_k} \left| \mathcal{L}_{Y|U=u}(\mathcal{Y}_j) - \mathcal{L}_{Y|U=u^\prime}(\mathcal{Y}_j)\right| d\mathcal{L}_U(u^\prime) && \text{\# Triangle inequity} \\
        &\leq \dashint_{\mathcal{U}_k} \epsilon/2 \, d\mathcal{L}_U(u^\prime) = \epsilon/2, 
    \end{align*}
    which means $\sup_{\mathcal{Y}_j\in\mathcal{Y}} |\mathcal{L}_{Y|U=u}(\mathcal{Y}_j)-\mathcal{L}_{Y|U\in\mathcal{U}_k}(\mathcal{Y}_j)| =: \mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k}) \leq \epsilon/2$. In a similar way, we can prove $\mathrm{TV}(\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u},\mathcal{L}_{Y|X\in\mathcal{X}_i,U\in\mathcal{U}_k})\leq\epsilon/2$. To be specific, under $\mathbb{H}_0:X\ind Y|U$, we have $\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u}=\mathcal{L}_{Y|U=u}$ for any $\mathcal{X}_i\subseteq\mathcal{X}$. As a result, the map $u\mapsto \mathcal{L}_{Y|X\in\mathcal{X}_i,U=u}$ is also $L_Y$-Lipschitz continuous wrt TV distance. The rest of the proof is the same as above. 

    \textbf{Part II.} We show $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|\leq \epsilon$. Specifically, since $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U\in\mathcal{U}_k}) \leq \epsilon/2$, we have $|\mathbb{P}(Y\in\mathcal{Y}_j|U=u) - \mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k)|\leq \epsilon/2$. Since $\mathrm{TV}(\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u},\mathcal{L}_{Y|X\in\mathcal{X}_i,U\in\mathcal{U}_k})\leq \epsilon/2$, we also have $|\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U=u) - \mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k)|\leq \epsilon/2$. According to the triangle inequality, we have 
    \begin{align*}
        & |\mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k)| \\
        \leq & |\mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U=u)| + |\mathbb{P}(Y\in\mathcal{Y}_j|U=u) - \mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k)|\\
        = & |\mathbb{P}(Y\in\mathcal{Y}_j|U\in\mathcal{U}_k) - \mathbb{P}(Y\in\mathcal{Y}_j|U=u)| + |\mathbb{P}(Y\in\mathcal{Y}_j|X\in \mathcal{X}_i, U=u) - \mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U\in\mathcal{U}_k)| \leq \frac{\varepsilon}{2} + \frac{\varepsilon}{2} = \varepsilon,
    \end{align*}
    where the 2nd equality is due to $\mathbb{P}(Y\in\mathcal{Y}_j|U=u)=\mathbb{P}(Y\in\mathcal{Y}_j|X\in\mathcal{X}_i,U=u)$ under $\mathbb{H}_0:X\ind Y|U$.
\end{proof}

\subsection{Definition~\ref{def.tight}: Tightness of distribution}

\begin{definition}[Tightness of distribution] We say the marginal distribution $\mathcal{L}_U$ is tight if $\forall \epsilon>0, \exists T, \forall t\geq T,\mathbb{P}(|U|\geq t)\leq \epsilon$. We say the conditional distribution $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$ if $\forall \epsilon>0, \exists T, \forall t\geq T, \forall x\in [a,b],$ we have $\mathbb{P}(|U|\geq t|x)\leq \epsilon$.
\label{def.tight}
\end{definition}

\begin{remark}
    We use the term ``uniform'' because the $T$ holds uniformly for all $x\in[a,b]$. As we will show below, this condition can easily hold for ANM. 
\end{remark}

\begin{example}[Addictive noise model with uniform tightness]
    Suppose that random variables $X,U$ satisfy the additive noise model $U=m(X)+V$, where $V$ is the noise variable. If $m$ is bounded in $[a,b]$ and $\mathcal{L}_V$ is tight, then $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$.
\end{example}

\begin{proof}
    Since $\mathcal{L}_V$ is tight, we first have $\forall \epsilon>0, \exists T, \forall t\geq T, \int_t^\infty f_V(v)dv \leq \epsilon$. Besides, we denote $H$ as the upper bound of $m(x)$, such that $|m(x)| \leq H$ for all $x \in [a,b]$. Then we can obtain the uniform tightness of $\mathcal{L}_{U|X}$ by noting that $\forall \epsilon > 0$, we have $S:=T+H$ such that $\forall s > S$, 
    \begin{align*}
        \int_{s}^\infty f_{U|X}(u|x) du = \int_s^\infty f_V(u-m(x)) du = \int_{s-m(x)}^\infty f_V(v) dv \leq \epsilon, 
    \end{align*}
    where we use the fact that $s\geq T + H \geq T + |m(x)| \geq T + h(x)$ therefore  $s-m(x)\geq T$.
\end{proof}

\subsection{Proposition~\ref{prop.dis-err unbd}: Discretization error control; continue}

\begin{proposition}[Discretization error control; continue]
\label{prop.dis-err unbd}
    Suppose that $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$, the map $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz continuous wrt TV distance, and that  $len(\mathcal{X}_i)\leq \epsilon/2L_U$. Then, $\forall \mathcal{X}_i, \mathcal{Y}_j$ and $\forall\epsilon>0$, there exists $T$, such that for all $t\geq T$, we have 
    \begin{align*}
        \mathbb{P}(Y\in \mathcal{Y}_j,|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon, \ \mathbb{P}(W\in \mathcal{W}_l,|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon.
    \end{align*}
\end{proposition}

\begin{proof}
    We only provide the proof of $\mathbb{P}(Y\in \mathcal{Y}_j,|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon$, as $\mathbb{P}(W\in \mathcal{W}_l,|U|\geq t|X\in\mathcal{X}_i)$ can be derived analogously. We obtain this conclusion by showing $\mathbb{P}(|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon$ and using the fact that
    \begin{align*}
        \mathbb{P}(Y\in \mathcal{Y}_j,|U|\geq t|X\in\mathcal{X}_i) = \mathbb{P}(Y\in \mathcal{Y}_j||U|\geq t,X\in\mathcal{X}_i) \mathbb{P}(|U|\geq t|X\in\mathcal{X}_i) \leq \mathbb{P}(|U|\geq t|X\in\mathcal{X}_i)\leq \epsilon.
    \end{align*}
   Given $\mathcal{L}_{U|X}$ is uniformly tight, we first have $\forall \epsilon/2>0, \exists T_1, \forall t\geq T_1, \forall x\in \mathcal{X}_i, \mathbb{P}(|U|\geq t|x) \leq \epsilon/2$. Then, since $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz, we have $\forall \epsilon/2>0, |\mathbb{P}(|U|>t|x) - \mathbb{P}(|U|>t|\mathcal{X}_i)|\leq \epsilon/2$ for $x\in\mathcal{X}_i$. Applying the triangle inequality, we have $\mathbb{P}(|U|>t|\mathcal{X}_i)\leq \epsilon$.
\end{proof}

==> icml24_app/old_versions/notation.tex <==
\textcolor{red}{Todo:long equations, not inline; (adjust them after finishing the main text)}

\textcolor{blue}{Those in blue are my response/question to some of your questions. For those without response, I will modify as suggested :).}

\section{Preliminary}

Consider continuous random variables $X,Y,U$. That is, $(\Omega,\mathcal{F},\mathbb{P})$ is the probability space, and $X:\Omega\mapsto\mathcal{X}$, $Y:\Omega\mapsto\mathcal{Y}$, $U:\Omega\mapsto\mathcal{U}$ are all measurable functions, with $\mathcal{X}$, $\mathcal{Y}$, $\mathcal{U}$ being intervals or the real line. We denote $\mathcal{L}_X:=\mathbb{P}\circ X^{-1}$ the law of $X$, and denote $f_X(\cdot)$, $F_X(\cdot)$ the probability density function (pdf) and cumulative density function (cdf), respectively. We use $n$ to denote the sample size.

For discretization, we use $\{\mathcal{X}_i\}_{i=1}^I$ to denote a partition of $\mathcal{X}$ with $I$ subintervals (bins), and thereby define the discretized variable $\tilde{X}$ by assigning $\tilde{X}:=\tilde{x}_i$ iff $X\in\mathcal{X}_i$. For two discretized variable $\tilde{X},\tilde{Y}$ (with $I,J$ levels, respectively), we use the column vector $P(\tilde{X}|\tilde{y}):=[\mathbb{P}(\tilde{x}_1|\tilde{y}),...,\mathbb{P}(\tilde{x}_I|\tilde{y})]^T$, the row vector $P(\tilde{x}|\tilde{Y}):=[\mathbb{P}(\tilde{x}|\tilde{y}_1),...,\mathbb{P}(\tilde{x}|\tilde{y}_J)]$, and the matrix $P(\tilde{X}|\tilde{Y}):=[P(\tilde{X}|\tilde{y}_1),...,P(\tilde{X}|\tilde{y}_J)]$ to represent conditional probabilities $\mathbb{P}(\tilde{x}|\tilde{y})$.

Our goal is to test the null hypothesis $\mathbb{H}_0:X\ind Y|U$ against the alternative $\mathbb{H}_1: X\not\ind Y|U$. Here, we assume $U$ can only be measured with error by a proxy variable $W$ satisfying $X\ind W|U$. Several graphical examples to illustrate the relation among $X,Y,U$ and $W$ are provided in Figure~??.

\begin{remark}
    Note that our theory can adapt to scenarios where there are more than one proxy. Here, we illustrate with the single-proxy case because testing under this case is considered the most challenging [??].
\end{remark}


% ToC appendix
% notations, goal
% regular probablity
% error control discretization
% -> tv-smoothness, tightness
% rank-preserving discretization
% ci-test
% -> type-i/ii, explain the condition "integral equation has no solution"

% ToC main
% Sec. Preliminary
% -> Notations & problem setup
% -> Proximal model (Pearl) P(W|X)=... P(y|X)=... 
% -> Chi-sq test (Miao) To test the above linearty, ...

% Sec. Discretization theories
% -> dis-err (put bin number setting discusion here)
% -> rank-preserving

% Sec. CI-Test
% -> Type-i/ii error


==> icml24_app/old_versions/notation_xw.tex <==
\section{Preliminary}

Consider the continuous treatment $X \in \mathcal{X}$, response variable $Y \in \mathcal{Y}$, and unobserved confounder $U \in \mathcal{U}$ over $(\Omega,\mathcal{F},\mathbb{P})$, with $\mathcal{X}=\mathcal{Y}=\mathcal{U}=\mathbb{R}$. We denote $\mathcal{L}_X:=\mathbb{P}\circ X^{-1}$ as the law of $X$, and $f_X(\cdot)$, $F_X(\cdot)$ as the probability density function (pdf) and cumulative density function (cdf), respectively. We use $n$ to denote the sample size.

For discretization, we use $\{\mathcal{X}_i\}_{i=1}^I$ to denote a partition of $\mathcal{X}$ with $I$ subintervals (bins), and thereby define the discretized variable $\tilde{X}$ by assigning $\tilde{X}=i$ iff $X\in\mathcal{X}_i$. For two discretized variable $\tilde{X},\tilde{Y}$ with respectively $I$ and $J$ levels, we use the column vector $P(\tilde{X}|\tilde{y}):=[\mathbb{P}(\tilde{x}_1|\tilde{y}),...,\mathbb{P}(\tilde{x}_I|\tilde{y})]^T$ with $\mathbb{P}(\tilde{x}_i|\tilde{y}) := \mathbb{P}(\tilde{X}=i|\tilde{y})$ for all $i \in [I]$, the row vector $P(\tilde{x}_i|\tilde{Y}):=[\mathbb{P}(\tilde{x}|\tilde{y}_1),...,\mathbb{P}(\tilde{x}|\tilde{y}_J)]$ with $\mathbb{P}(\tilde{x}_i|\tilde{y}_j):=\mathbb{P}(\tilde{X}=i|\tilde{Y}=j)$ for all $i \in [I]$ and $j \in [J]$, and the matrix $P(\tilde{X}|\tilde{Y}):=[P(\tilde{X}|\tilde{y}_1),...,P(\tilde{X}|\tilde{y}_J)]$ to represent conditional probabilitity matrix. We say $f:\mathcal{X} \mapsto \mathbb{R}$ is an integrable function, if $\int_{\mathcal{X}} |f(x)| dx < \infty$. For a matrix $A$, we denote $\mathrm{det}(A)$ as the determinant of $A$. Besides, we denote $\mathrm{ker}(A):=\{x:Ax=0\}$ and $\mathrm{im}(A):=\{y: y =Ax \text{ for some $x$} \}$ as the kernel space and the image space of $A$, respectively.  

Our goal is to test the causal null hypothesis $\mathbb{H}_0:X\ind Y|U$ against the alternative $\mathbb{H}_1: X\not\ind Y|U$. Here, we assume $U$ is associated with a proxy variable $W$ satisfying $X\ind W|U$. Several graphical examples to illustrate the relation among $X,Y,U$ and $W$ are provided in Fig.~\ref{fig.proxy}.

\begin{remark}
    We only consider the case with a single proxy since it is more challenging than the scenario when multiple proxies are available, where our method can be certainly applied. 
\end{remark}


% ToC appendix
% notations, goal
% regular probablity
% error control discretization
% -> tv-smoothness, tightness
% rank-preserving discretization
% ci-test
% -> type-i/ii, explain the condition "integral equation has no solution"

% ToC main
% Sec. Preliminary
% -> Notations & problem setup
% -> Proximal model (Pearl) P(W|X)=... P(y|X)=... 
% -> Chi-sq test (Miao) To test the above linearty, ...

% Sec. Discretization theories
% -> dis-err (put bin number setting discusion here)
% -> rank-preserving

% Sec. CI-Test
% -> Type-i/ii error


==> icml24_app/old_versions/regular_prob.tex <==
\section{Regular conditional probability}
\label{sec.regular-prob}

In this section, we use the regular conditional probability to define ``conditioning on a zero-probability event'' rigorously \xw{replaced with ``to rigorously define the conditional probability given the zero-probability event"?}. We start from the standard Kolmogorov definition of conditional expectation.

\begin{definition}[\cite{williams1991probability}, Definition~9.2]
    Let $(\Omega,\mathcal{F},\mathbb{P})$ be the probability space, and let $X$ be a random variable with $E(|X|)<\infty$. Let $\mathcal{G}$ be a sub-$\sigma$-algebra of $\mathcal{F}$. Then there exists a $\mathcal{G}$-measurable random variable $Y$ such that $E[|Y|]<\infty$, and that for every set $G\in \mathcal{G}$, we have $\int_G Yd\mathbb{P} = \int_G Xd\mathbb{P}$. Moreover, if $Y^\prime$ is another random variable with these properties, then $Y^\prime=Y$ a.s. A random variable $Y$ with the above properties is called a version of the conditional expectation $E[X|\mathcal{G}]$ of $X$ given $\mathcal{G}$, and we write $Y=E[X|\mathcal{G}]$ a.s.
\end{definition}

\begin{remark}
    The existence of $Y$ satisfying the above properties is guaranteed by the Radon-Nikodym theorem \cite{durrett2019probability} (Theorem A.4.8). $Y=dX/d \mathbb{P}$ is also called the Radon-Nikodym derivative.
\end{remark}

We often write $E[X|Z]$ in short for $E[X|\sigma(Z)]$, which is the conditional expectation of $X$ given $\sigma(Z)$. For $F\in \mathcal{F}$, define the conditional probability $\mathbb{P}(F|Z)$ as a version of $E[\mathbbm{1}_{F}|Z]$. In this regard, the map $\mathbb{P}(\cdot,\cdot): \Omega\times \mathcal{F}\mapsto [0,1)$ defined by $\mathbb{P}(\omega,F):=\mathbb{P}(F|Z)(\omega)$ is a measurable function that maps a tuple $(\omega,F)$ to a real value in $[0,1]$. 

Now, suppose that the map $\mathbb{P}(\cdot,\cdot)$ satisfies the following regular properties:
\vspace{-1em}
\begin{enumerate}[label={(\arabic*)}]
    \itemsep0em
    \item for $F\in\mathcal{F}$, the function $\omega\mapsto \mathbb{P}(\omega,F)$ is a version of $\mathbb{P}(F|\mathcal{G})$,
    \item for every $\omega$, the map $F\mapsto \mathbb{P}(\omega,F)$ is a probability measure on $\mathcal{F}$\footnote{Strictly speaking, the regular conditional probability requires that for \emph{almost} every $\omega$, the map $F\mapsto \mathbb{P}(\omega,F)$ is a probability measure. Nonetheless, for those $\{\omega\}$ (a set of measure zero) where $\mathbb{P}(\omega,F)$ is not well-defined, one can redefine $\mathbb{P}(\omega,F):=\lim_{r\to 0} \frac{1}{|B_r(\omega)|}\int_{B_r(\omega)} \mathbb{P}(t,F) dt$ (where $B_r(\omega)$ is a ball with radius $r$), so that $\mathbb{P}(\omega,F)$ is now well-defined strictly everywhere.}.
\end{enumerate}
\vspace{-1em}
It is then called a \textbf{regular conditional probability} (rcp) \cite{williams1991probability} (Section~9.9). The existence of rcps under mild conditions is guaranteed by the disintegration theorem \cite{chang1997conditioning} (Definition~1 and Theorem~1). 

We then define the conditional probability $\mathrm{Pr}(X\in F|Z(\omega)=z)$ given the zero-probability event $Z=z$ as the rcp $\mathbb{P}(\omega,F)$. Thanks to the above properties (1)-(2), our definition is well-defined.

\xw{do we need to mention the ``Sobolev embedding theorem" to ensure the conditional probability is well defined everywhere?}

==> icml24_app/old_versions/regular_prob_xw.tex <==
\section{Regular conditional probability}
\label{sec.regular-prob}

In this section, we use the regular conditional probability to rigorously define the conditional probability $\mathbb{P}(Y \in F_Y | U=u)$ and $\mathbb{P}(W \in F_W | U=u)$, where $U=u$ can be a zero probability event. We start from the standard Kolmogorov definition of conditional expectation.

%\begin{definition}[Condition Expectation %\cite{williams1991probability}, Definition~9.2]
%    Let $(\Omega,\mathcal{F},\mathbb{P})$ be the probability space, and let $X$ be a random variable with $\mathbb{E}[|X|]<\infty$. Let $\mathcal{G}$ be a sub-$\sigma$-algebra of $\mathcal{F}$. Then there exists a $\mathcal{G}$-measurable random variable $Y$ such that $\mathbb{E}[|Y|]<\infty$, and that for every set $G\in \mathcal{G}$, we have $\int_G Yd\mathbb{P} = \int_G Xd\mathbb{P}$. Moreover, if $Y^\prime$ is another random variable with these properties, then $Y^\prime=Y$ a.s. A random variable $Y$ with the above properties is called a version of the conditional expectation $\mathbb{E}[X|\mathcal{G}]$ of $X$ given $\mathcal{G}$, and we write $Y=\mathbb{E}[X|\mathcal{G}]$ a.s.
%\end{definition}

\begin{definition}[Condition Expectation \cite{williams1991probability}, Definition~9.2]
Let $(\Omega,\mathcal{F},\mathbb{P})$ be a probability triple, $X$ a random variable with $E(|X|)<\infty$, and $\mathcal{G}$ a sub-$\sigma$-algebra of $\mathcal{F}$. Then there exists a random variable $Y$ such that:
\begin{enumerate}
    \itemsep0em
    \item $Y$ is $\mathcal{G}$-measurable,
    \item $E[|Y|]<\infty$,
    \item for every set $G\in \mathcal{G}$, we have:
    \begin{equation*}
        \int_G Yd\mathbb{P} = \int_G Xd\mathbb{P}.
    \end{equation*}
\end{enumerate}

Moreover, if $Y^\prime$ is another random variable with these properties then $Y^\prime=Y$, a.e., that is $\mathbb{P}(\{w:Y(w)=Y^\prime(w)\})=1$. A random variable $Y$ with the above properties is called a version of the \textbf{conditional expectation} $E[X|\mathcal{G}]$ of $X$ given $\mathcal{G}$, and we write $Y=E[X|\mathcal{G}]$, a.e.
\end{definition}


\begin{remark}
    The existence of $Y$ satisfying the above properties is guaranteed by the Radon-Nikodym theorem \cite{durrett2019probability} (Theorem A.4.8). $Y=dX/d \mathbb{P}$ is also called the Radon-Nikodym derivative.
\end{remark}

We often write $\mathbb{E}[X|Z]$ in short for $\mathbb{E}[X|\sigma(Z)]$, which is the conditional expectation of $X$ given $\sigma(Z)$. For $F\in \mathcal{F}$, define the conditional probability $\mathbb{P}(F|Z)$ as a version of $\mathbb{E}[\mathbbm{1}_{F}|Z]$. In this regard, the map $\mathbb{P}(\cdot,\cdot): \Omega\times \mathcal{F}\mapsto [0,1)$ defined by $\mathbb{P}(\omega,F):=\mathbb{P}(F|Z)(\omega)$ is a measurable function that maps a tuple $(\omega,F)$ to a real value in $[0,1]$. 


According to the disintegration theorem \cite{chang1997conditioning} (def.1 and thm.1) and \cite{williams1991probability} (page.91), there exists $\mathbb{P}(\cdot,\cdot)$ with $\mathbb{P}(F|Z)$ being as a version of $\mathbb{E}[\mathbbm{1}_{F}|Z]$, satisfying the following regular properties:
\begin{enumerate}[label={(\arabic*)}]
    \itemsep0em
    \item for $F\in\mathcal{F}$, the function $\omega\mapsto \mathbb{P}(\omega,F)$ is a version of $\mathbb{P}(F|\mathcal{G})$,
    \item for almost every $\omega$, the map $F\mapsto \mathbb{P}(\omega,F)$ is a probability measure on $\mathcal{F}$.
\end{enumerate}
Then, for those $\{\omega\}$ (a set of measure zero) where $\mathbb{P}(\omega,F)$ is not well-defined, one can redefine $\mathbb{P}(\omega,F):=\lim_{r\to 0} \frac{1}{|B_r(\omega)|}\int_{B_r(\omega)} \mathbb{P}(t,F) dt$ (where $B_r(\omega)$ is a ball with radius $r$), so that $\mathbb{P}(\omega,F)$ is now well-defined strictly everywhere. By applying $\mathbb{P}(\omega,F)$ to $\mathbb{P}(Y| U)$ and $\mathbb{P}(W| U)$, we obtain that they are well defined. 







==> icml24_app/old_versions/type-ii_xw.tex <==
\section{Conditional independence test}

In this section, we provide details about the type-I and type-II error control by our procedure. 

\textbf{Test statistic.} Denote $q^T:=[P(\tilde{y}_1|\tilde{X}),...,P(\tilde{y}_{J-1}|\tilde{X})]$ and denote $Q:=\mathrm{diag}[P(\tilde{W}|\tilde{X}),...,P(\tilde{W}|\tilde{X})]$ as the block diagonal matrix with $(J-1)$ blocks of $P(\tilde{W}|\tilde{X})$ in the diagonal. Suppose that we have available estimators $(\hat{q},\hat{Q})$ satisfying that
\begin{align*}
    & n^{1/2}(\hat{q} - q) \to_d N(0,\Sigma), \\
    \hat{Q} \to_p Q, & \ \hat{\Sigma} \to_p \Sigma, \text{ where $\hat{\Sigma}, \Sigma$ are positive definite. }
\end{align*}
Then similar to \cite{miao2018identifying}, we denote the least square residual of regressing $\hat{\Sigma}^{-1/2} \hat{q}$ on $\hat{\Sigma}^{-1/2} \hat{Q}$ as 
\begin{align*}
    \hat{\xi} := \{\mathrm{I} - \hat{\Sigma}^{-1/2} \hat{Q}^T (\hat{Q} \hat{\Sigma}^{-1} \hat{Q}^T)^{-1} \hat{Q} \hat{\Sigma}^{-1/2}\} \hat{\Sigma}^{-1/2} \hat{q}.
\end{align*}
Define the squared residual $T:=n^{1/2}\xi^T \xi$ as our test statistics and denote the corresponding estimator as $\hat{T}:=n^{1/2}\hat{\xi}^T \hat{\xi}$.

\subsection{Proof of Theorem~\ref{thm.control.type-i}: Type-i error control}

Let $r:=(I-L)(J-1)$, and $z_{1-\alpha}$ the $1-\alpha$ quantile of chi-square distribution $\chi_{r}^2$ with freedom $r$.

\begin{theorem}
    Suppose that Assumptions~\ref{asm.tv-smooth}, \ref{asm.comp} and the conditions in Proposition~\ref{prop.dis-err unbd} hold, then under $\mathbb{H}_0:X\ind Y|U$, it holds that $\hat{T} \to \chi_{r}^2$ in distribution as $n,L\to \infty$. As a consequence, for any $\alpha\in (0,1)$, $\lim_{n,L\to \infty} \mathbb{P}(\hat{T}>z_{1-\alpha}) = \alpha$. In other words, the test we define has uniform asymptotic level $\alpha$.
\label{thm.control.type-i}
\end{theorem}

\begin{proof}
    We first consider testing with a single level $\tilde{y}$. To this end, denote (with slight overuse of notations) $r:=I-L$, $q^T:=P(\tilde{y}|\tilde{X})$, $Q:=P(\tilde{W}|\tilde{X})$, and $\Sigma,\hat{\Sigma}$ the corresponded covariance matrices. The proof consists of two parts. In \textbf{part I}, we first show the asymptotic linearity between $q^T$ and $Q$. Then, in \textbf{part II}, we analyze the asymptotic distribution of the test statistics.

    \textbf{Part I.} In the following, we show the asymptotic linearity $q^T=P(\tilde{y}|\tilde{U})P(\tilde{W}|\tilde{U})^{-1}Q + \boldsymbol{e}$ with $\lim_{L\to\infty} \boldsymbol{e}=\boldsymbol{0}$.
    
    We first consider cases where $\mathcal{U}$ is a compact interval. To show the asymptotic linearity , we first show 
    \begin{align}
        q^T & = P(\tilde{y}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_1, \ \lim_{L\to\infty} \boldsymbol{e}_1 = 0, \label{eq.linear-q}\\
        Q & = P(\tilde{W}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_2, \ 
        \lim_{L\to\infty} \boldsymbol{e}_2 = \boldsymbol{0}. \label{eq.linear-Q}
    \end{align}
    Then under Assumption~\ref{asm.comp}), we have 
    \begin{align*}
        q^T= P(\tilde{y}|\tilde{U})P(\tilde{W}|\tilde{U})^{-1} Q + \boldsymbol{e}, \ \lim_{L\to\infty}\boldsymbol{e}=\lim_{L\to\infty} \{\boldsymbol{e}_1 - P(\tilde{y}|\tilde{U})P(\tilde{W}|\tilde{U})^{-1} \boldsymbol{e}_2\} =\boldsymbol{0}.  
    \end{align*}
    To show Eq.~\eqref{eq.linear-q}, note that we first have 
    \begin{align*}
        q^T:=P(\tilde{y}|\tilde{X}) = P(\tilde{y}_l|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_1, \ \boldsymbol{e}_1 = [\{P(\tilde{y}_l|\tilde{U},\tilde{x}_i) - P(\tilde{y}_l|\tilde{U})\}P(\tilde{U}|\tilde{x}_i)]_{i=1}^I.
    \end{align*}
    Let $K=L$, according to Prop.~\ref{prop.control-err}, we have $\lim_{L\to\infty} \boldsymbol{e}_1 = \boldsymbol{0}$. Similarly, we can show
    \begin{align*}
        Q = P(\tilde{W}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_2, \text{ where } \boldsymbol{e}_2 = [\{P(\tilde{W}|\tilde{U},\tilde{x}_i) - P(\tilde{W}|\tilde{U})\}P(\tilde{U}|\tilde{x}_i)]_{i=1}^I, 
    \end{align*}
    and $\lim_{L\to\infty} \boldsymbol{e}_2 = \boldsymbol{0}$.

    We then consider the case where $\mathcal{U}=\mathbb{R}$. Still, we want to establish Eq.~\eqref{eq.linear-q},~\eqref{eq.linear-Q}. We first derive the form of $\boldsymbol{e}_1$. For a given $t$, divide $\mathcal{U}$ into $\mathcal{U}^\prime:=\{u:|u|>t\}$ and $\mathcal{U}^{''}:=\mathcal{U}\backslash\mathcal{U}^\prime$, and further partition $\mathcal{U}^{''}$ into $K$ bins $\{\mathcal{U}_k\}_{k=1}^K$. We then have 
    \begin{align*}
        \mathbb{P}(\tilde{y}|\tilde{x}_i) = P(\tilde{y}|\tilde{U},\tilde{x}_i) P(\tilde{U}|\tilde{x}_i) + \mathbb{P}(\tilde{y}|U\in\mathcal{U}^\prime,\tilde{x}_i) \mathbb{P}(U\in\mathcal{U}^\prime|\tilde{x}_i).
    \end{align*}
    Therefore, we have 
    \begin{align*}
        P(\tilde{y}|\tilde{X}) & = P(\tilde{y}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_{\text{bd}} + \boldsymbol{e}_{\text{ubd}}, \\
        \boldsymbol{e}_{\text{bd}} & = \{[P(\tilde{y}|\tilde{U},\tilde{x}_i)-P(\tilde{y}|\tilde{U})] P(\tilde{U}|\tilde{x_i})\}_{i=1}^I, \\
        \boldsymbol{e}_{\text{ubd}} & = \{\mathbb{P}(\tilde{y},U\in\mathcal{U}^\prime|\tilde{x}_i)\mathbb{P}(U\in\mathcal{U}^\prime|\tilde{x}_i)\}_{i=1}^I. 
    \end{align*}
    where $\boldsymbol{e}_{\text{bd}}$ is the error in the compact interval $\mathcal{U}^\prime$ and $\boldsymbol{e}_{\text{ubd}}$ is the error in the unbounded $\mathcal{U}^{''}$. We have $\lim_{L \to \infty} \boldsymbol{e}_1=\boldsymbol{e}_{\text{bd}} + \boldsymbol{e}_{\text{ubd}} = 0$, since $\lim_{L \to \infty} \boldsymbol{e}_{\text{bd}} = 0$ by repeating the previous proof and $\lim_{L \to \infty} \boldsymbol{e}_{\text{ubd}} = 0$ can be shown in Proposition~\ref{prop.dis-err unbd}. Similarly, we have
    \begin{align*}
        Q=P(\tilde{W}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_{\text{2}}, \ \boldsymbol{e}_2=\{[P(\tilde{W}|\tilde{U},\tilde{x}_i)-P(\tilde{W}|\tilde{U})] P(\tilde{U}|\tilde{x_i})\}_{i=1}^I+\{P(\tilde{W}|U\in\mathcal{U}^\prime,\tilde{x}_i)\mathbb{P}(U\in\mathcal{U}^\prime|\tilde{x}_i)\}_{i=1}^I, 
    \end{align*}
    and $\lim_{t,L\to\infty} \boldsymbol{x}_2=\boldsymbol{0}$.

    \textbf{Part II.} We analyze the asymptotic distribution of the statistics $\hat{T}:=n^{1/2}\hat{\xi}^T \hat{\xi}$. We first show $n^{1/2} \hat{\xi} \to N(0,\Omega)$. Specifically, given that $\hat{Q} \to Q$, $\hat{\Sigma}_l \to \Sigma_l$ in probability, and that $n^{1/2}(\hat{q} - q) \to N(0,\Sigma)$ in distribution, apply Slutsky's theorem, we have 
    \begin{align}
    \label{eq.omega}
        n^{1/2}(\hat{\xi} - \Omega\Sigma^{1/2}q_l)\to_d N(0,\Omega_l), \ \Omega:=\mathrm{I}_I - {\Sigma}^{-1/2} {Q}^T ({Q} {\Sigma}^{-1} {Q}^T)^{-1} {Q} {\Sigma}^{-1/2}.
    \end{align}
    Then, under $\mathbb{H}_0:X\ind Y|U$, according to the asymptotic linearity in \textbf{part I}, we have $\Omega\Sigma^{-1/2}q \to 0$ as $L\to\infty$. Applying Slutsky's theorem again, we have $n^{1/2} \hat{\xi} \xrightarrow{\mathcal{D}} N(0,\Omega)$. 
    
    Then, we show $\mathrm{rank}(\Omega)=r$. Specifically, we have $\mathrm{rank}(Q)=L$ according to Proposition~\ref{prop.rank-dis}. Since $\Sigma^{-1/2}$ is invertible, we have $\mathrm{rank}(Q\Sigma^{-1/2})=L$. Thus, the idempotent matrix $M:={\Sigma}^{-1/2} {Q}^T ({Q} {\Sigma}^{-1} {Q}^T)^{-1} {Q} {\Sigma}_l^{-1/2}$ has rank $L$. According to Corollary~11.5 of \citep{banerjee2014linear}, $M$ has $K$ eigenvalues equal to one and $I-L$ eigenvalues equal to zero. Thus, we have $\Omega=\mathrm{I}-M$ being an idempotent matrix with rank $r=I-L$.

    Finally, we show $\hat{T} \to \chi_{r}^2$ in distribution. To be specific, given that $n^{1/2} \hat{\xi} \to N(0,\Omega)$, we have $\hat{T}:=n\hat{\xi}^T \hat{\xi} \to N(0,\Omega)^T N(0,\Omega)$ according to Theorem~1.12 of \cite{shao2003mathematical}. What is left is to show $N(0,\Omega)^T N(0,\Omega)=\chi^2_r$. To see this, note that we have the orthogonal decomposition $V\Omega V^T= \mathrm{diag}(1,...,1,0,...,0)$, where $V$ is an orthogonal matrix and $\mathrm{diag}(1,...,1,0,...,0)$ is a diagonal matrix with $r$ $1$s and $I-r$ $0$s in the diagonal. Therefore, we have $VN(0,\Omega) = N(0,\mathrm{diag}(1,...,1,0,...,0))$ and $N(0,\Omega)^T N(0,\Omega) = \left[VN(0,\Omega)\right]^T \left[VN(0,\Omega)\right] = \chi^2_r$.

    We now discuss testing with all levels $\tilde{y}_1,...,\tilde{y}_J$. For this case, we have $\mathrm{rank}(\Omega)=(I-L)(J-1)$ by aggregating the rank of each level together. Therefore, we have $\hat{T} \to \chi_{r}^2$ in distribution, where $r=(I-L)(J-1)$.
\end{proof}


\subsection{Proof of Theorem~\ref{thm.type-ii}: Type-ii error control}


\begin{assumption}
    \label{asm.H1}
    Denote $\mathbb{C}(\mathcal{W},\mathcal{Y})$ the set of almost surely continuous functions over $\mathcal{W}\times \mathcal{Y}$. For $h\in \mathbb{C}(\mathcal{W},\mathcal{Y})$, let the averaged residual of fitting the integral equation $f(y|x)=\int h(y,w)f(w|x)dw$ be 
    \begin{align*}
        \mathrm{res}_h:=\iint |f(y|x)-\int h(y,w)f(w|x)dw|dy f(x) dx.
    \end{align*}
    Then we assume there exists $\epsilon_0>0$, such that $\min_{h\in \mathbb{C}(\mathcal{W},\mathcal{Y})} \mathrm{res}_h>\epsilon_0$ under $\mathbb{H}_1$. 
\end{assumption}

\begin{remark}
    This assumption means there is no solution to $f(y|x) = \int h(y,w)f(w|x)dw$ under $\mathbb{H}_1$. 
\end{remark}

\begin{theorem}
    Suppose that Assumptions~\ref{asm.tv-smooth}, \ref{asm.comp},~\ref{asm.H1} and the conditions in Proposition~\ref{prop.dis-err unbd} hold, and that $p(y|x)$ (\emph{resp.}, $p(w|x)$) is continuous over $\mathcal{X} \times \mathcal{Y}$ (\emph{resp.}, $\mathcal{X} \times \mathcal{W}$), then for any significance level $0<\alpha<1$, it holds that $\lim_{n,L\to\infty}\mathbb{P}_{\Theta}(T\leq z_{1-\alpha})=0$. In other words, the probability of making a type-ii error can be controlled to zero asymptotically.
    \label{thm.type-ii}
\end{theorem}


\begin{remark}
    According to the following proof, we have that under the same condition, there exists a solution $h \in \mathbb{C}(\mathcal{W},\mathcal{Y})$ such that $f(y|x) = \int h(y,w)f(w|x)dw$ under $\mathbb{H}_0$. 
\end{remark}


\begin{proof}
    The proof consists of two parts. In \textbf{part I}, we show that under ${\Theta}$, $q\not \in \mathrm{im}(Q)$ ($\mathrm{im}(Q)$ is the image space of $Q$) as $L\to\infty$. Then, in \textbf{part II}, given that $q\not \in \mathrm{im}(Q)$, we show $\mathbb{P}_{\Theta}(T\leq z_{1-\alpha})$ can be controlled to zero.

    \textbf{Part I.} We show that under ${\Theta}$, $q\not \in \mathrm{im}(Q)$ as $L\to\infty$. To see this, we first show that there exists $L_0$ such that as long as $I>K=L>L_0$, $q\not \in \mathrm{im}(Q)$. Specifically, let 
    \begin{align*}
        \mathrm{res}(h):=\iint |f(y|x)-\int h(y,w)f(w|x)dw|dy f(x) dx,
    \end{align*}
    and let $\arg\min_h \mathrm{res}(h)$. Since $f(y|x)\geq 0$ and $f(w|x)\geq 0$, since $h_0$ minimizes $\mathrm{res}(h)$, we have $h_0\geq 0$ a.s. Besides, we have the following by taking $M$ sufficiently large, 
    \begin{align*}
        \int_{|x|\leq M} \int_{|y|\leq M} \left|f(y|x)-\int h(y,w)f(w|x)dw \right|dy f(x) dx > \frac{1}{2} \epsilon_0, \text{ for any $h\geq 0$}. 
    \end{align*}
     To see this, note that for any $M$, we have $\mathrm{res}(h)=\mathrm{res}_{\leq M}{h} + \mathrm{res}_{>M}(h)$, where 
     \begin{align*}
         \mathrm{res}_{\leq M}(h) & :=\int_{|x|\leq M} \int_{|y|\leq M} |f(y|x)-\int h(y,w)f(w|x)dw|dy f(x) dx \\
         \mathrm{res}_{> M}(h) & :=\left(\int_{|x|> M} \int_{|y|\leq M}+\int_{|x|\leq M} \int_{|y|> M}+\int_{|x|> M} \int_{|y|> M} \right) \left|f(y|x)-\int h(y,w)f(w|x)dw \right|dy f(x) dx.
     \end{align*}
     For $\mathrm{res}_{>M}(h)$, we have 
     \begin{align*}
         \mathrm{res}_{>M}(h) & \geq \left(\int_{|x|> M} \int_{|y|\leq M}+\int_{|x|\leq M} \int_{|y|> M}+\int_{|x|> M} \int_{|y|> M} \right) f(y|x)f(x)dydx \\
         & = \mathbb{P}(|X|>M)+\mathbb{P}(|X|\leq M,|Y|>M) < \frac{1}{2}\epsilon_0
     \end{align*}
     if $M$ is sufficiently large. Then, without loss of generality, we have $\mathrm{res}(h)>\epsilon_0$ for some $\epsilon_0$ and $M > 0$ such that $|X| \leq M, |Y|\leq M$. Since $f(y|x)$ is continuous, there exists $M_0$ such that $f(y|x)\leq M_0$ on $\{(x,y):|x|\leq M, |y|\leq M\}$. Therefore, we have $0\leq h_0\leq M_0$, which means we only need to consider $h$ with $0\leq h\leq M_0$.

    Further, there exists $M_w>0$ such that 
    \begin{align*}
        \int_{|x|\leq M}\int_{|y|\leq M} \left|f(y|x)-\int_{|w|\leq M_w} h(w,y) f(w|x) dw \right| dyf(x)dx >\frac{3}{4}\epsilon_0
    \end{align*}
    for any $0\leq h \leq M_0$. To see this, note that 
    \begin{align*}
        \mathrm{res}(h) & =\int_{|x|\leq M} \int_{|y|\leq M} \left|f(y|x)-\int_{|w|\leq M_w} h(y,w)f(w|x)dw\right|dy f(x) dx \\
        & \quad \quad \quad \quad \quad \quad \quad \quad + \int_{|x|\leq M}\int_{|y|\leq M} \int_{|w|>M_w} h(w,y)f(w|x)dwdyf(x)dx \\
        & \leq \int_{|x|\leq M} \int_{|y|\leq M} |f(y|x)-\int_{|w|\leq M_w} h(y,w)f(w|x)dw|dy f(x) dx + M\cdot M_0 \mathbb{P}(|W|>M_w,|X|\leq M) \\
        & \leq \int_{|x|\leq M} \int_{|y|\leq M} |f(y|x)-\int_{|w|\leq M_w} h(y,w)f(w|x)dw|dy f(x) dx + M\cdot M_0 \mathbb{P}(|W|>M_w).
    \end{align*}
    Therefore, for any $0\leq h\leq M_0$, we have $\mathrm{res}^{M_w}(h)>\frac{3}{4}\epsilon_0$. Note that 
    \begin{align*}
        \mathrm{res}^{M_w}(h)=\sum_{i=1}^I \sum_{j=1}^J \int_{\mathcal{X}_i} \int_{\mathcal{Y}_j} \left|f(y|x)-\int_{|w|\leq M_w} h(w,y) f(w|x) dw \right|dyf(x)dx.
    \end{align*}
    Since $f(y|x)$ and $f(w|x)$ are respectively uniformly continuous in $\{(x,y):|x|\leq M, |y|\leq M\}$ and $\{(x,w):|x|\leq M, |w|\leq M_w\}$, there exists $I_{0,1}$ $J_{0,1}$ such that for any $I>I_{0,1}, J>J_{0,1}$, we have 
    \begin{align}
    \label{eq.bound-01}
        \left|\mathrm{res}^{M_w}(h)-\sum_{i=1}^I \sum_{j=1}^J\left|f(\bar{y}_j|\bar{x}_i)-\int_{|w|\leq M_w} h(w,y) f(w|\bar{x}_i)dw\right| \mathbb{P}(X \in \mathcal{X}_i)\mathrm{len}(\mathcal{Y}_j) \right| < \frac{1}{4} \epsilon_0
    \end{align}
    for any $\bar{x}_i \in \mathcal{X}_i, \bar{y}_j \in \mathcal{Y}_j$, and $h$ that is constant for any $w$ and $y\in\mathcal{Y}_j$. To see this, note that $f(y|x)$ and $f(w|x)$ are uniformly continuous. Then $\forall\epsilon>0$, there exists $\delta>0$ such that 
    \begin{align*}
        \left|f(w_1|x_1)-f(w_2|x_2) \right| \leq \epsilon, \
        \left|f(y_1|x_1)-f(y_2|x_2)\right|\leq \epsilon
    \end{align*}
    for any $\sqrt{(w_1-w_2)^2+(x_1+x_2)^2}<\delta$ and $\sqrt{(y_1-y_2)^2+(x_1+x_2)^2}<\delta$. Therefore, as long as the partition satisfies that for each $i,j, \mathrm{len}(\mathcal{X}_i)\leq \delta,\mathrm{len}(\mathcal{Y}_j)<\delta$, then for any $h$ that is constant for any $w$ and $y\in\mathcal{Y}_j$, we have
    \begin{align*}
        & \iint_{\mathcal{X}_i,\mathcal{Y}_j}|\mathbb{P}(\bar{y}_j|\bar{x}_i)-f(y|x)|f(x) dxdy  \leq \epsilon \delta, \\
        & \iint_{\mathcal{X}_i,\mathcal{Y}_j} \left| \int_{|w|\leq M_w} h(w,\bar{y}_j) f(w|\bar{x}_i) dw - \int_{|w|\leq M_w} h(w,y)f(w|x)dw \right|f(x)dxdy \\
        & \leq \iint_{\mathcal{X}_i,\mathcal{Y}_j}  \int_{|w|\leq M_w} h(w,\bar{y}_j) \left|f(w|\bar{x}_i)-f(w|x)\right| dw f(x)dxdy \leq M_0M_w \epsilon\delta,
    \end{align*}
    for some $\bar{x}_i \in \mathcal{X}_i$ and $\bar{y}_j \in \mathcal{Y}_i$. By taking the $\epsilon$ small enough, we have the desired conclusion.

    Similarly, there exists $I_{0,2},J_{0,2}$ such that as long as $I>I_{0,2},J>J_{0,2}$, we have 
    \begin{align}
        & \left|\sum_{i=1}^I \sum_{j=1}^J  \left| \int_{\mathcal{X}_i}\int_{\mathcal{Y}_j} f(y|x)-\int_{|w|\leq M_w} h(w,y) f(w|x)dw  dyf(x) dx \right|  - \right. \nonumber \\
        & \left. \sum_{i=1}^I \sum_{j=1}^J \left| f(\bar{y}_j|\bar{x}_i) -\int_{|w|\leq M_w} h(w,y)f(w|\bar{x}_i) dw \right| \mathbb{P}(X \in \mathcal{X}_i)\mathrm{len}(\mathcal{Y}_j) \right|<\frac{1}{4}\epsilon_0 \label{eq.bound-02}
    \end{align}
   for any $h$ that is constant for any $w$ and $y\in\mathcal{Y}_j$. In addition, by noting that 
   \begin{align*}
       \int_{\mathcal{X}_i}\int_{\mathcal{Y}_j}\left(f(y|x)-\int h(w,y)f(w|x)dw\right)dyf(x)dx=\mathbb{P}(\tilde{y}_j|\tilde{x}_i)-\int g_l(w)f(w|X\in\mathcal{X}_i)dw \mathbb{P}(X \in \mathcal{X}_i),
   \end{align*}
   where $g_l(w):=\int_{Y\in\mathcal{Y}_j} h(w,y)dy$, we have 
   \begin{align}
   \label{eq.bound-03}
       \sum_{i=1}^I \sum_{j=1}^J \left| \int_{\mathcal{X}_i} \int_{\mathcal{Y}_j} \left(f(y|x)-\int h(w,y)f(w|x)dw\right)dyf(x)dx \right|=\sum_{i=1}^I \sum_{j=1}^J \left| \mathbb{P}(\tilde{y}_j|\tilde{x}_i)-\int g_l(w)f(w|X\in\mathcal{X}_i)dw \right| \mathbb{P}(X\in \mathcal{X}_i).
   \end{align}
  

    By combining Eq.~\eqref{eq.bound-01},~\eqref{eq.bound-02},~\eqref{eq.bound-03}, for any $I>\max(I_{0,1},I_{0,2})$, $J> \max(J_{0,1},J_{0,2})$, we have 
    \begin{align*}
        \left|\mathrm{res}^{M_w}(h)-\sum_{i=1}^I \sum_{j=1}^J \left|\mathbb{P}(\tilde{y}_j|\tilde{x}_i)-\int g_l(w)f(w|X\in\mathcal{X}_i)dw \right|\mathbb{P}(X\in \mathcal{X}_i) \right| \leq \frac{1}{2}\epsilon_0.
    \end{align*}
    Then for any $I,J$, there exist $L_0$ such that for any $L>L_0$, we have 
    \begin{align*}
        \left|\mathrm{res}^{M_w}(h)-\sum_{i=1}^I \sum_{j=1}^J \left|\mathbb{P}(\tilde{y}_j|\tilde{x}_i)-\sum_k \mathbb{P}(\tilde{w}_k|\tilde{x}_i) g_l(w)f(w|X\in\mathcal{X}_i)dw \right|\mathbb{P}(X\in \mathcal{X}_i) \right| \leq \frac{3}{4}\epsilon_0.
    \end{align*}
    If $q=Q^T c$ for some $c=[[c_{1,1},...,c_{L,1}],...,[c_{1,J},...,C_{L,J}]]^T$, with $c_{l,i,j}=c_{l,i^',j}$, then we let $h(w,y)=c_{k,l}$ for $w\in\mathcal{W}_l,y\in\mathcal{Y}_j$ and have $\mathbb{P}(\tilde{y}_j|\tilde{x}_i)=\sum_l \mathbb{P}(\tilde{w}_k|\tilde{x}_i) c_{l,j}$. Therefore, we have $\sum_{i=1}^I\sum_{j=1}^J |\mathbb{P}(\tilde{y}_l|\tilde{x}_i)-\sum_l \mathbb{P}(\tilde{w}_l|\tilde{x}_i) g_l(\tilde{u}_l)|\mathbb{P}(X\in \mathcal{X}_i)=0$ for some $h$ that is constant in each $\mathcal{Y}_j$. Therefore, we have $\mathrm{res}^{M_w}(h)<\frac{3}{4}\epsilon_0$, which obtains the contradiction.

    \textbf{Part II.} Given that $q\not \in \mathrm{im}(Q)$, we show $\lim_{n,L\to \infty} \mathbb{P}_{\Theta}(T\leq z_{1-\alpha})=0$. To show this, we first discuss the distribution of $T$ given $q\not \in \mathrm{im}(Q)$. First, we have $||\Omega \Sigma_y^{-1/2} q_y||^2_2>0$. To see this, we first have that $\mathrm{ker}(\Omega)=\mathrm{im}(\Sigma^{-1/2}Q^T)$. 

    To see this, we have $\forall \vec{a}\in \mathrm{im}(\Sigma^{-1/2}Q^T), \exists \vec{b}, s.t. \vec{a} = \Sigma^{-1/2}Q^T \vec{b}$. According to the definition of $\Omega$ in Eq.~\eqref{eq.omega}, we have $\Omega \vec{a} = \Omega \Sigma^{-1/2}Q^T \vec{b} = \vec{0}$, which means $\mathrm{im}(\Sigma^{-1/2}Q^T) \subseteq \mathrm{ker}(\Omega)$. What is left is to show $\mathrm{dim}(\mathrm{im}(\Sigma^{-1/2}Q^T)) = \mathrm{dim}(\mathrm{ker}(\Omega))$. First, we have $\mathrm{dim}(\mathrm{im}(\Sigma^{-1/2}Q^T)) = \mathrm{rank}(\Sigma^{-1/2}Q^T) = L(J-1)$. Since $\mathrm{rank}(\Omega)=(I-L)(J-1)$ and $\Omega \in \mathbb{R}^{I(J-1) \times I(J-1)}$, we have $\mathrm{nul}(\Omega)=I*(J-1)-(I-L)(J-1)=L(J-1)$ ($\mathrm{nul}(\Omega)$ is the null space of $\Omega$) and therefore $\mathrm{dim}(\mathrm{ker}(\Omega))=L(J-1)=\mathrm{dim}(\mathrm{im}(\Sigma^{-1/2}Q^T))$. Therefore, we have $\mathrm{ker}(\Omega)=\mathrm{im}(\Sigma^{-1/2}Q^T)$.
    
    
    
    Therefore, $q\not \in \mathrm{im}(Q)$ means $\Sigma^{-1/2} q \not \in \mathrm{img}(\Sigma^{-1/2} Q^T) = \mathrm{ker}(\Omega)$, and we have $\Omega\Sigma^{-1/2} q \neq \vec{0}$ and $|| \Omega\Sigma^{-1/2} q ||^2_2>0$. Second, let $\vec{c} := \Omega \Sigma^{-1/2} q$, we show $T$ follows the noncentral chi square distribution $\chi^2(r,\lambda)$ with $\lambda=n||\vec{c}||^2_2$ and $r=(I-L)(J-1)$. To be specific, we have $\sqrt{n} (\xi - \vec{c}) \to N(0,\Omega)$ and therefore $\sqrt{n} \xi \to N(\sqrt{n}\vec{c}, \Omega)$. Repeating the orthogonal decomposition trick used in the proof of Theorem~\ref{thm.control.type-i}, we have:
    \begin{align*}
            T := n \xi^T \xi &\to N(\sqrt{n}\vec{c},\Omega)^T N(\sqrt{n}\vec{c},\Omega) = \{V N(\sqrt{n}\vec{c},\Omega)\}^T \{V N(\sqrt{n}\vec{c},\Omega)\} \\
            &= N(\sqrt{n}V\vec{c}, \mathrm{diag}(1,...,1,0,...,0))^T N(\sqrt{n}V\vec{c}, \mathrm{diag}(1,...,1,0,...,0)) = \chi^2(r,\lambda),
    \end{align*}

    Given that $T$ follows the noncentral $\chi^2(r,\lambda)$ distribution as $L\to\infty$, we then show $\lim_{n,L\to\infty}\mathbb{P}_{\Theta}(T\leq z_{1-\alpha})=0$, which is equivalent to show that $\forall \epsilon>0, \exists N, \forall n\geq N, \mathbb{P}_{\Theta}(T_y\leq z_{1-\alpha}) \leq\epsilon$. In details, denote $F(x;r,\lambda)$ the cdf of $\chi^2(r,\lambda)$ and let $f(\lambda):=F(x;r,\lambda)$. We first show for fixed ($x,r$) (the $x$ is $z_{1-\alpha}$ in our problem), $\lim_{\lambda\to\infty} f(\lambda) = 0$. According to \cite{nuttall1972some}, we can represent the cdf with Marcum Q function, \emph{i.e.}, $F(\lambda;x,r) = 1 - Q_{r/2}(\sqrt{\lambda},\sqrt{x})$, where
    \begin{align*}
        &Q_v(a,b) = 1 + H_v(a,b) + C_v(a,b) \\
        &H_v(a,b) = \frac{(a/b)^{1-v}}{2\pi} \exp\left(-\frac{1}{2}(a^2+b^2)\right) \int_{0}^{2\pi} \frac{\mathrm{cos}(v-1)\theta - (a/b)\mathrm{cos}(v\theta)}{1-2(a/b)\mathrm{cos}\theta + (a/b)^2} \exp(ab\mathrm{cos}\theta)\mathrm{d}\theta, \\
        &C_v(a,b) = \frac{\mathrm{sin}(v\pi)}{\pi} \exp\left(-\frac{1}{2}(a^2+b^2)\right) \int_0^1 \frac{x^{v-1} (b/a)^{v-1}}{(a/b)+x} \exp(-\frac{ab}{2}(x+\frac{1}{x})) \mathrm{d}x.
    \end{align*}

    Therefore, to show $\lim_{\lambda\to\infty} f(\lambda) = 0$, we show $\lim_{\lambda\to\infty} Q_{k/2}(\sqrt{\lambda},\sqrt{x}) = 0$, which needs $\lim_{a\to\infty} H_v(a,b) = 0$ and $\lim_{a\to\infty} C_v(a,b) = 0$. To see $\lim_{a\to\infty} H_v(a,b) = 0$, note that:
    \begin{align*}
        &\lim_{a\to \infty} \frac{(a/b)^{1-v}}{2\pi} = 0, \quad \hfill\#\, v \,\text{is a large number, so}\, 1-v<0, \\
        &\lim_{a\to \infty} \exp\left(-\frac{1}{2}(a^2+b^2)\right) \exp (ab\mathrm{cos}\theta) = 0, \quad \hfill\#\,\text{because}\, \lim_{a\to \infty}a^2-2ab\mathrm{cos}\theta+b^2 = \infty, \\
        &\lim_{a\to \infty} \frac{\mathrm{cos}(v-1)\theta-(a/b)\mathrm{cos}(v\theta)}{1-2(a/b)\mathrm{cos}\theta+(a/b)^2} = 0 \quad \#\, \text{this is like}\, \lim_{a\to \infty} \frac{a}{1-a+a^2}= 0.
    \end{align*}

    Therefore, use Lebesgue’s dominated convergence theorem (our integrand can be dominated by $1$ when $a$ is sufficiently large, and $1$ is an integrable function) to exchange the limitation and integration, we have $\lim_{a\to\infty} H_v(a,b) = 0$. A similar process can show $\lim_{a\to\infty} C_v(a,b) = 0$. Now, with $\lim_{\lambda\to\infty} f(\lambda) = 0$, we have $\forall \epsilon>0,\exists\, \Lambda,\forall\lambda>\Lambda, f(\lambda):=\mathbb{P}_{\chi^2(r,\lambda)}(T_y\leq z_{1-\alpha})\leq \epsilon$. Therefore, we have $\forall \epsilon>0,\exists N:=\frac{\Lambda}{||\vec{c}||^2_2},\forall n\geq N,\lambda:=n||\vec{c}||^2_2 \geq \Lambda$ and hence $\mathbb{P}_{\Theta}(T_y\leq z_{1-\alpha})\leq \epsilon$, which concludes the proof.
\end{proof}


\subsection{Characterization of Assumption~\ref{asm.H1}}
\label{app-sec.int-eq}

Theorem~\ref{thm.type-ii} involves an important condition that the integral equation $f(y|x)=\int h(y,w)f(w|x)dw$ does not have a solution. Intuitively, this condition means the correlation between $X$ and $Y$ can not be fully explained by that between $X$ and $W$. Indeed, we empirically find that this condition can hold in many cases. Specifically, we consider four cases in the following numerical experiment: 
\begin{itemize}
\itemsep0em
    \item \textbf{Linear Gaussian Model.} $U=X+N_1, Y=a X+U+N_2, W=U+N_3, \  X, N_1, N_2, N_3 \sim N(0, 0.1)$, where $a$ ranges from 1 to 10. 
    \item \textbf{Linear non-Gaussian Model.} $U=X+N_1, Y=a X+U+N_2, W=U+N_3,  X \sim \mathrm{ Uniform}(-0.5, 0.5), N_1, N_2, N_3 \sim \operatorname{Exp}(0.1)$, where $a$ ranges from 1 to 10. 
    \item \textbf{Nonlinear Additive Noise Model.} $U=X^2+N_1, Y=a e^X+U+N_2,  W=\tan (U)+N_3, \ X \sim \mathrm{Uniform}(-0.5, 0.5), \ N_1, N_2, N_3 \sim \operatorname{Exp}(0.1)$,  where $a$ ranges from 1 to 10. 
    \item \textbf{Gaussian Nonlinear Model.} $U=|X| N_1, Y=a e^{X+N_2}+U, \  W=\tan \left(U+N_3\right), \ X \sim \mathrm{Uniform}(-0.5, 0.5), \ N_1, N_2, N_3 \sim \operatorname{Exp}(0.1)$, where $a$ ranges from 1 to 10. 
\end{itemize}

For each case, we implement the Maximum Moment Restriction (MMR) with Gaussian kernels in the $\mathrm{mliv}$ package\footnote{\url{https://github.com/causal-machine-learning-lab/mliv}} to find the solution to the conditional moment equation $E[Y-h(W)|X]=0$. The results are shown in Figure~\ref{fig.exam-integral-equation-no-solution}. As we can see, when $X$ and $Y$ becomes correlated $X\not\ind Y|U$, there is no valid solution to the conditional moment function, which indicates the insolubility of the integral equation (\ref{eq.int-eq}).

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{icml24_figs/intgeral_solution.pdf}
    \caption{Insolubility of the integral equation when $X\not\perp Y|U$. We consider four examples, namely the linear Gaussian model, the linear nonGaussian model, the nonlinear additive noise model, and the general nonlinear models. For each example, we report the averaged residual of the best fit of the integral equation $f(y|x)=\int h(y,w)f(w|x)dw$ wrt to the correlation strength of $X$ and $Y$. As we can see, when $X$ and $Y$ become correlated ($X\not\perp Y|U$), the residual becomes non-zero, indicating the insolubility of the integral equation. }
    \label{fig.exam-integral-equation-no-solution}
\end{figure*}

However, this condition may not constantly hold, as shown by the following theorem. 
\begin{theorem}
    Suppose the following conditions hold:
    \begin{enumerate}
    \itemsep0em
        \item Completeness of $X \mid U: E[g(x) \mid u]=0$ a.s. $x \rightarrow g(x)=0$ a.s.
        \item $\iint p(u \mid x) p(x \mid u) d x d u<+\infty$.
        \item $\int p^2(y \mid x) p(x) d x<+\infty$.
        \item Denote $K: L^2(p(u)) \rightarrow L^2(p(x))$, where $L^2(p(x)):=\{h(x): \int h^2(x) p(x)dx < \infty\}$. Denote $\left(\lambda_n, \phi_n, \psi_n\right)_{n=1}^{\infty}$ a singular value decomposition of $K$. Then we assume $\sum_{n=1}^{\infty} \lambda_n^{-2}\left|\left\langle p(y \mid x), \psi_n\right\rangle\right|<+\infty$, where $\left\langle p(y \mid x), \psi_n\right\rangle:=\int p^2(y \mid x) \psi_n(x) p(x) d x$.
    \end{enumerate}
Then there exists $h(u, y)$ such that $\int h(u, y) p(u \mid \mathrm{x})=p(y \mid x)$ holds for all $(x, y)$.
\end{theorem}

\begin{remark}
    These conditions should be compatible with our completeness condition in assump.~\ref{asm.comp}. Particularly, the completeness of $\mathcal{L}(U|X)$ and that of $\mathcal{L}(X|U)$ roughly means the $U$ and $X$ have similar levels of variation. To explain, note that if $U$ and $X$ are discrete, then we have $\mathbb{P}(U|X)$ and $\mathbb{P}(X|U)$ are both invertible. 
\end{remark}

\begin{remark}
    This result, which means assump.~\ref{asm.H1} does not always hold, means it is reasonable to take assump.~\ref{asm.H1} as a condition, instead of a theorem or a claim/hypothesis. 
\end{remark}

\begin{proof}
    Simply follow the proof of Prop. 1 in \cite{miao2018identifying}, by replacing $p(w | z, x)$ with $p(u | x), p(z | w, x)$ with $p(x | u), p(y | z, x)$ with $p(y | x),\left(K_x, L^2(p(w | x)), L^2(p(z | x)), \lambda_{x, n}, \phi_{x, n}, \psi_{x, n}\right)$ with $\left(K, L^2(p(u)), L^2(p(x)), \lambda_n, \phi_n, \psi_n\right)$. 
\end{proof}
 
 












\subsection{Estimating the conditional probability vector}
\label{app-sec.mle}

Consider discrete random variables $X,Y$ that (respectively) take values $\{x_1,...,x_I\}$ and $\{y_1,...,y_J\}$. Suppose that we have $n$ iid samples. Denote $Z_{ij}$ the number of samples that take the value $(x_i,y_j)$, and denote $Z_{i:}:=\sum_j Z_{ij}$. Then, the MLE estimator of conditional probability vector $P(y|X)$ is $\hat{P}(y|X) = \left[\hat{p}(y|x_1),...,\hat{p}(y|x_I)\right]$, where $\hat{p}(y_j|x_i) = Z_{ij}/Z_{i:}$.

The MLE estimator satisfies that $\hat{P}(y|X)\to P(y|X)$ in probability, and that $n^{1/2}(\hat{P}(y|X)-P(y|X)) \to N(0,\Sigma)$ in distribution. The covariance matrix is $\Sigma=\mathrm{diag}[\frac{p(y_j|x_1)(1-p(y_j|x_1))}
{p(x_1)},...,\frac{p(y_j|x_I)(1-p(y_j|x_I))}{p(x_I)}]$ and is positive definite. The corresponding estimator $\hat{\Sigma}$ that satisfies $\hat{\Sigma}\to \Sigma$ in probability can be obtained by replacing $p(y_j|x_i)$ with $\hat{p}(y_j|x_i)$, and replacing $p(x_i)$ with $\hat{p}(x_i)=Z_{i:}/n$. These results are obtained by noting that $Z_{ij}$ follows the multinomial distribution, and by applying the Fisher information matrix (in the sandwich form) and the Cramer-Rao lower bound \cite{casella2021statistical} (Theorem 7.3.9).

==> icml24_app/old_versions/typei-ii.tex <==
\newpage
\section{Conditional independence test}

\textbf{Test statistic.} Denote $q^T:=[P(\tilde{y}_1|\tilde{X}),...,P(\tilde{y}_{J-1}|\tilde{X})]$ and denote $Q:=\mathrm{diag}[P(\tilde{W}|\tilde{X}),...,P(\tilde{W}|\tilde{X})]$ as the block diagonal matrix with $(J-1)$ blocks of $P(\tilde{W}|\tilde{X})$ in the diagonal. Suppose that we have available estimators $(\hat{q},\hat{Q})$ satisfying that 
\begin{align*}
    n^{1/2}(\hat{q} - q) \to_d N(0,\Sigma), \\
    \hat{Q}\to_p Q, \ \hat{\Sigma} \to_p \Sigma, \text{ where $\hat{\Sigma}, \Sigma$ are positive definite. }
\end{align*}


(1) $n^{1/2}(\hat{q} - q) \to N(0,\Sigma)$ in distribution, (2) $\hat{Q}\to Q$, $\hat{\Sigma} \to \Sigma$ in probability, with $\hat{\Sigma}, \Sigma$ both positive definite. Then, denote the least square residual of regressing $\hat{\Sigma}^{-1/2} \hat{q}$ on $\hat{\Sigma}^{-1/2} \hat{Q}$ as $\hat{\xi} := \{\mathrm{I} - \hat{\Sigma}^{-1/2} \hat{Q}^T (\hat{Q} \hat{\Sigma}^{-1} \hat{Q}^T)^{-1} \hat{Q} \hat{\Sigma}^{-1/2}\} \hat{\Sigma}^{-1/2} \hat{q}$ ($\mathrm{I}$ is the identity matrix). Define the squared residual $T:=n^{1/2}\xi^T \xi$ as our test statistics and denote the corresponding estimator as $\hat{T}:=n^{1/2}\hat{\xi}^T \hat{\xi}$.

\subsection{Proof of Theorem~\ref{thm.control.type-i}: Type-i error control}

Let $r:=(I-L)(J-1)$, and $z_{1-\alpha}$ the $1-\alpha$ quantile of chi-square distribution $\chi_{r}^2$ with freedom $r$.

\begin{theorem}
    Suppose that Assumptions~\ref{asm.tv-smooth}, \ref{asm.comp} and the conditions in Proposition~\ref{prop.dis-err unbd} hold, then under $\mathbb{H}_0:X\ind Y|U$, it holds that $\hat{T} \to \chi_{r}^2$ in distribution as $n,L\to \infty$. As a consequence, for any $\alpha\in (0,1)$, $\lim_{n,L\to \infty} \mathbb{P}(\hat{T}>z_{1-\alpha}) = \alpha$. In other words, the test we define has uniform asymptotic level $\alpha$.
\label{thm.control.type-i}
\end{theorem}

\begin{proof}
    We first discuss \xw{consider} testing with a single level $\tilde{y}$. To this end, denote (with slight overuse of notations) $r:=I-L$, $q^T:=P(\tilde{y}|\tilde{X})$, $Q:=P(\tilde{W}|\tilde{X})$, and $\Sigma,\hat{\Sigma}$ the corresponded covariance matrices. The proof consists of two parts. In part 1., we first show the asymptotic linearity between $q^T$ and $Q$. Then, in part 2., we analyze the asymptotic distribution of the test statistics.

    \textbf{Part 1.} In the following, we show the asymptotic linearity $q^T=P(\tilde{y}|\tilde{U})P(\tilde{W}|\tilde{U})^{-1}Q + \boldsymbol{e}$ with $\lim_{L\to\infty} \boldsymbol{e}=\boldsymbol{0}$.
    
    We first consider cases where $\mathcal{U}$ is a compact interval. To show the asymptotic linearity , we first show $q^T= P(\tilde{y}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_1$ and $Q = P(\tilde{W}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_2$, with $\lim_{L\to\infty} \boldsymbol{e}_1 = \lim_{L\to\infty} \boldsymbol{e}_2 = \boldsymbol{0}$. In this regard, we have (under Assumption~\ref{asm.comp}) \xw{Under assump.~\ref{asm.comp}, we have} $q^T= P(\tilde{y}|\tilde{U})P(\tilde{W}|\tilde{U})^{-1} Q + \boldsymbol{e}$, with $\lim_{L\to\infty}\boldsymbol{e}=\lim_{L\to\infty} \{\boldsymbol{e}_1 - P(\tilde{y}|\tilde{U})P(\tilde{W}|\tilde{U})^{-1} \boldsymbol{e}_2\} =\boldsymbol{0}$. In details, to show $q^T= P(\tilde{y}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_1$, note that $\mathbb{P}(\tilde{y}|\tilde{x}_i)=P(\tilde{y}|\tilde{U})P(\tilde{U}|\tilde{x}_i) +\{P(\tilde{y}|\tilde{U},\tilde{x}_i) - P(\tilde{y}|\tilde{U})\}P(\tilde{U}|\tilde{x}_i)$. Thus, we have $q^T:=P(\tilde{y}|\tilde{X}) = P(\tilde{y}_l|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_1$, where $\boldsymbol{e}_1 = [\{P(\tilde{y}_l|\tilde{U},\tilde{x}_i) - P(\tilde{y}_l|\tilde{U})\}P(\tilde{U}|\tilde{x}_i)]_{i=1}^I$. Let $K=L$, according to Proposition~\ref{prop.control-err}, we have $\lim_{L\to\infty} \boldsymbol{e}_1 = \boldsymbol{0}$. In a similar way, we can show $Q = P(\tilde{W}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_2$, where $\boldsymbol{e}_2 = [\{P(\tilde{W}|\tilde{U},\tilde{x}_i) - P(\tilde{W}|\tilde{U})\}P(\tilde{U}|\tilde{x}_i)]_{i=1}^I$ and $\lim_{L\to\infty} \boldsymbol{e}_2 = \boldsymbol{0}$.

    We then consider the case where $\mathcal{U}$ is the real line \xw{$\mathcal{U} = \mathbb{R}^d$?}. We still show \xw{Still, we want to prove} $q^T= P(\tilde{y}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_1$ and $Q = P(\tilde{W}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_2$, where $\boldsymbol{e}_1,\boldsymbol{e}_2$ have different forms but still converge to zeros \xw{$\boldsymbol{e}_1,\boldsymbol{e}_2$ converge to 0 as $L \to \infty$}. For this purpose \xw{delete}, we first show the form of $\boldsymbol{e}_1$. Specifically, for a given $t$, divide $\mathcal{U}$ into $\mathcal{U}^\prime:=\{u:|u|>t\}$ and $\mathcal{U}^{''}:=\mathcal{U}\backslash\mathcal{U}^\prime$, and further partition $\mathcal{U}^{''}$ into $K$ bins $\{\mathcal{U}_k\}_{k=1}^K$. We then have $\mathbb{P}(\tilde{y}|\tilde{x}_i) = P(\tilde{y}|\tilde{U},\tilde{x}_i) P(\tilde{U}|\tilde{x}_i) + \mathbb{P}(\tilde{y}|U\in\mathcal{U}^\prime,\tilde{x}_i) \mathbb{P}(U\in\mathcal{U}^\prime|\tilde{x}_i)$. Therefore, we have $P(\tilde{y}|\tilde{X}) = P(\tilde{y}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_{\text{bd}} + \boldsymbol{e}_{\text{ubd}}$, where $\boldsymbol{e}_{\text{bd}} = \{[P(\tilde{y}|\tilde{U},\tilde{x}_i)-P(\tilde{y}|\tilde{U})] P(\tilde{U}|\tilde{x_i})\}_{i=1}^I$ is the error in the compact interval $\mathcal{U}^\prime$ and $\boldsymbol{e}_{\text{ubd}} = \{\mathbb{P}(\tilde{y},U\in\mathcal{U}^\prime|\tilde{x}_i)\mathbb{P}(U\in\mathcal{U}^\prime|\tilde{x}_i)\}_{i=1}^I$ is the error in the unbounded $\mathcal{U}^{''}$. To control $\boldsymbol{e}_1=\boldsymbol{e}_{\text{bd}} + \boldsymbol{e}_{\text{ubd}}$, note that the control of $\boldsymbol{e}_{\text{bd}}$ has been discussed above and the control of $\boldsymbol{e}_{\text{ubd}}$ has been shown in Proposition~\ref{prop.dis-err unbd}. In a similar way, we can show $Q=P(\tilde{W}|\tilde{U})P(\tilde{U}|\tilde{X}) + \boldsymbol{e}_{\text{2}}$, where $\boldsymbol{e}_2=\{[P(\tilde{W}|\tilde{U},\tilde{x}_i)-P(\tilde{W}|\tilde{U})] P(\tilde{U}|\tilde{x_i})\}_{i=1}^I+\{P(\tilde{W}|U\in\mathcal{U}^\prime,\tilde{x}_i)\mathbb{P}(U\in\mathcal{U}^\prime|\tilde{x}_i)\}_{i=1}^I$ and $\lim_{t,L\to\infty} \boldsymbol{x}_2=\boldsymbol{0}$.

    \textbf{Part 2.} We analyze the asymptotic distribution of the statistics $\hat{T}:=n^{1/2}\hat{\xi}^T \hat{\xi}$. We first show $n^{1/2} \hat{\xi} \to N(0,\Omega)$. Specifically, given that $\hat{Q} \to Q$, $\hat{\Sigma}_l \to \Sigma_l$ in probability, and that $n^{1/2}(\hat{q} - q) \to N(0,\Sigma)$ in distribution, apply Slutsky's theorem, we have $n^{1/2}(\hat{\xi} - \Omega\Sigma^{1/2}q_l)\to N(0,\Omega_l)$ in distribution, where $\Omega:=\mathrm{I} - {\Sigma}^{-1/2} {Q}^T ({Q} {\Sigma}^{-1} {Q}^T)^{-1} {Q} {\Sigma}^{-1/2}$. Then, under $\mathbb{H}_0:X\ind Y|U$, according to the asymptotic linearity in part 1., we have $\Omega\Sigma^{-1/2}q \to 0$ as $L\to\infty$. Applying Slutsky's theorem again, we have $n^{1/2} \hat{\xi} \xrightarrow{\mathcal{D}} N(0,\Omega)$. 
    
    Then, we show $\mathrm{rank}(\Omega)=r$. Specifically, we have $\mathrm{rank}(Q)=L$ according to Proposition~\ref{prop.rank-dis}. Since $\Sigma^{-1/2}$ is invertible, we have $\mathrm{rank}(Q\Sigma^{-1/2})=L$. Thus, the idempotent matrix $M:={\Sigma}^{-1/2} {Q}^T ({Q} {\Sigma}^{-1} {Q}^T)^{-1} {Q} {\Sigma}_l^{-1/2}$ has rank $L$. According to Corollary~11.5 of \citep{banerjee2014linear}, $M$ has $K$ eigenvalues equal to one and $I-L$ eigenvalues equal to zero. Thus, we have $\Omega=\mathrm{I}-M$ being an idempotent matrix with rank $r=I-L$.

    Finally, we show $\hat{T} \to \chi_{r}^2$ in distribution. To be specific, given that $n^{1/2} \hat{\xi} \to N(0,\Omega)$, we have $\hat{T}:=n\hat{\xi}^T \hat{\xi} \to N(0,\Omega)^T N(0,\Omega)$ according to Theorem~1.12 of \cite{shao2003mathematical}. What is left is to show $N(0,\Omega)^T N(0,\Omega)=\chi^2_r$. To see this, note that we have the orthogonal decomposition $V\Omega V^T= \mathrm{diag}(1,...,1,0,...,0)$, where $V$ is an orthogonal matrix and $\mathrm{diag}(1,...,1,0,...,0)$ is a diagonal matrix with $r$ $1$s and $I-r$ $0$s in the diagonal. Therefore, we have $VN(0,\Omega) = N(0,\mathrm{diag}(1,...,1,0,...,0))$ and $N(0,\Omega)^T N(0,\Omega) = \left[VN(0,\Omega)\right]^T \left[VN(0,\Omega)\right] = \chi^2_r$.

    We now discuss testing with all levels $\tilde{y}_1,...,\tilde{y}_J$. For this case, we have $\mathrm{rank}(\Omega)=(I-L)(J-1)$ by aggregating the rank of each level together. Therefore, we have $\hat{T} \to \chi_{r}^2$ in distribution, where $r=(I-L)(J-1)$.
\end{proof}


\subsection{Proof of Theorem~\ref{thm.type-ii}: Type-ii error control}

Denote $\mathbb{C}(\mathcal{W},\mathcal{Y})$ the set of almost surely continuous functions over $\mathcal{W}\times \mathcal{Y}$. For $h\in \mathbb{C}(\mathcal{W},\mathcal{Y})$, let the averaged residual of fitting the integral equation $f_\theta(y|x)=\int h(y,w)f_\theta(w|x)dw$ be $\mathrm{res}_\theta:=\iint |f_\theta(y|x)-\int h(y,w)f_\theta(w|x)dw|dy f_\theta(x) dx$. Let $\Theta:=\{\theta: \exists\epsilon_0>0, \min_{h\in \mathbb{C}(\mathcal{W},\mathcal{Y})} \mathrm{res}_\theta>\epsilon_0\}$ be the set of $\mathbb{H}_1$ models under which the integral equation has no solution.

\begin{theorem}
    Suppose that Assumptions~\ref{asm.tv-smooth}, \ref{asm.comp} and the conditions in Proposition~\ref{prop.dis-err unbd} hold, then for any significance level $0<\alpha<1$, it holds that $\lim_{n,L\to\infty}\mathbb{P}_{\Theta}(T\leq z_{1-\alpha})=0$. In other words, the probability of making a type-ii error can be controlled to zero asymptotically.
    \label{thm.type-ii}
\end{theorem}

\begin{proof}
    The proof consists of two parts. In part 1., we show that under ${\Theta}$, $q\not \in \mathrm{im}(Q)$ ($\mathrm{im}(Q)$ is the image space of $Q$) as $L\to\infty$. Then, in part 2., given that $q\not \in \mathrm{im}(Q)$, we show $\mathbb{P}_{\Theta}(T\leq z_{1-\alpha})$ can be controlled to zero.

    \textbf{Part 1.} We show that under ${\Theta}$, $q\not \in \mathrm{im}(Q)$ as $L\to\infty$. To show this, we show \xw{To see this, we first show} that there exists $L_0$ such that as long as $I>K=L>L_0$, $q\not \in \mathrm{im}(Q)$. Specifically, let $\mathrm{res}(h):=\iint |f(y|x)-\int h(y,w)f(w|x)dw|dy f(x) dx$ and let $h_0:=\min_h \mathrm{res}(h)$ \xw{$\arg\min_h \mathrm{res}(h)$?}. Since $f(y|x)\geq 0$ and $f(w|x)\geq 0$, we have $h_0\geq 0$ a.s. Therefore, there exists $M$ such that $\int_{|x|\leq M} \int_{|y|\leq M} |f(y|x)-\int h(y,w)f(w|x)dw|dy f(x) dx > \frac{1}{2} \epsilon_0$ for any $h\geq 0$. To see this, note that for any $M$, we have $\mathrm{res}(h)=\mathrm{res}_{\leq M}{h} + \mathrm{res}_{>M}(h)$, where $\mathrm{res}_{\leq M}(h):=\int_{|x|\leq M} \int_{|y|\leq M} |f(y|x)-\int h(y,w)f(w|x)dw|dy f(x) dx$ and $\mathrm{res}_{> M}(h):=(\int_{|x|> M} \int_{|y|\leq M}+\int_{|x|\leq M} \int_{|y|> M}+\int_{|x|> M} \int_{|y|> M}) |f(y|x)-\int h(y,w)f(w|x)dw|dy f(x) dx$. Then, we have $\mathrm{res}_{>M}(h)\geq (\int_{|x|> M} \int_{|y|\leq M}+\int_{|x|\leq M} \int_{|y|> M}+\int_{|x|> M} \int_{|y|> M}) f(y|x)f(x)dydx = \mathbb{P}(|X|>M)+\mathbb{P}(|X|\leq M,|Y|>M) < \frac{1}{2}\epsilon_0$ for some $M$. Then, without loss of generality, we have the above assumption for $|X| \leq M, |Y|\leq M$, that is, there exists $\epsilon_0>0$ such that $\mathrm{res}(h)>\epsilon_0$. Since $f(y|x)$ is continuous, there exists $M_0$ such that $f(y|x)\leq M_0$ on $\{(x,y):|x|\leq M, |y|\leq M\}$. Therefore, we have $0\leq h_0\leq M_0$, which means we only need to consider $h$ with $0\leq h\leq M_0$.

    Further, there exists $M_w>0$ such that $\int_{|x|\leq M}\int_{|y|\leq M} |f(y|x)-\int_{|w|\leq M_w} h(w,y) f(w|x) dw| dyf(x)dx >\frac{3}{4}\epsilon_0$ for any $0\leq h \leq M_0$. To see this note that $\mathrm{res}(h)=\int_{|x|\leq M} \int_{|y|\leq M} |f(y|x)-\int_{|w|\leq M_w} h(y,w)f(w|x)dw|dy f(x) dx+ \int_{|x|\leq M}\int_{|y|\leq M} \int_{|w|>M_w} h(w,y)f(w|x)dwdyf(x)dx\leq \int_{|x|\leq M} \int_{|y|\leq M} |f(y|x)-\int_{|w|\leq M_w} h(y,w)f(w|x)dw|dy f(x) dx + M\cdot M_0 \mathbb{P}(|W|>M_w,|X|\leq M) \leq \int_{|x|\leq M} \int_{|y|\leq M} |f(y|x)-\int_{|w|\leq M_w} h(y,w)f(w|x)dw|dy f(x) dx + M\cdot M_0 \mathbb{P}(|W|>M_w)$. By letting $M_w$ sufficiently large, we have the conclusion. Denote $\mathrm{res}^{M_w}(h):=\int_{|x|\leq M} \int_{|y|\leq M} |f(y|x)-\int_{|w|\leq M_w} h(y,w)f(w|x)dw|dy f(x) dx$, we have for any $0\leq h\leq M_0$, we have $\mathrm{res}^{M_w}(h)>\frac{3}{4}\epsilon_0$.

    Note that $\mathrm{res}^{M_w}(h)=\sum_{i=1}^I \sum_{j=1}^J \int_{\mathcal{X}_i} \int \mathcal{Y}_j |f(y|x)-\int_{|w|\leq M_w} h(w,y) f(w|x) dw|dyf(x)dx$. Since $f(y|x)$ and $f(w|x)$ are (respectively) \xw{respectively} uniformly continuous in $\{(x,y):|x|\leq M, |y|\leq M\}$ and $\{(x,w):|x|\leq M, |w|\leq M_w\}$, there exists $I_{0,1}$ $J_{0,1}$ such that for any $I>I_{0,1}, J>J_{0,1}$, we have $|\mathrm{res}^{M_w}(h)-\sum_{i=1}^I \sum_{j=1}^J|\mathbb{P}(\tilde{y}_j|\tilde{x}_i)-\int_{|w|\leq M_w} h(w,y) f(w|\tilde{x}_i)dw| \mathbb{P}(\tilde{x}_i)\mathrm{len}(\mathcal{Y}_j)| < \frac{1}{4} \epsilon_0$ for any $h$ that is constant for any $w$ and $y\in\mathcal{Y}_j$. To see this, note that $f(y|x)$ and $f(w|x)$ are uniformly continuous. Then $\forall\epsilon>0$, there exists $\delta>0$ such that $|\mathbb{P}(\tilde{w}_1|\tilde{x}_1)-\mathbb{P}(\tilde{w}_2|\tilde{x}_2)|\leq \epsilon$, $|\mathbb{P}(\tilde{y}_1|\tilde{x}_1)-\mathbb{P}(\tilde{y}_2|\tilde{x}_2)|\leq \epsilon$ for any $\sqrt{(w_1-w_2)^2+(x_1+x_2)^2}<\delta$ and $\sqrt{(y_1-y_2)^2+(x_1+x_2)^2}<\delta$. Therefore, as long as the partition satisfies that for each $i,j, \mathrm{len}(\mathcal{X}_i)\leq \delta,\mathrm{len}(\mathcal{Y_j})<\delta$, $\iint_{\mathcal{X}_i,\mathcal{Y}_j}|\mathbb{P}(y_0|x_0)-f(y|x)|f(x) dxdy\leq \epsilon$ and $\iint_{\mathcal{X}_i,\mathcal{Y}_j}|\int_{|w|\leq M_w} h(w,y_0) f(w|x_0) dw - \int_{|w|\leq M_w} h(w,y)f(w|x)dw|f(x)dwdy\leq 2M_0M\epsilon$ for ant $h$ that is constant for any $w$ and $y\in\mathcal{Y}_j$. By taking the $\epsilon$ small enough, we have the desired conclusion.

    Similarly, there exists $I_{0,2},J_{0,2}$ such that as long as $I>I_{0,2},J>J_{0,2}$, we have $|\sum_{i=1}^I \sum_{j=1}^J |\int_{\mathcal{X}_i}\int_{\mathcal{Y}_j} (f(y|x)-\int_{|w|\leq M_w} h(w,y) f(w|x)dw) dyf(x) dx|-\sum_{i=1}^I \sum_{j=1}^J |\mathbb{P}(\tilde{y}_j|\tilde{x}_i) \int_{|w|\leq M_w} h(w,\tilde{y}_j)f(w|\tilde{x}_i) dw|\mathbb{P}(\tilde{x}_i)\mathrm{len}(\mathcal{Y}_j)|<\frac{1}{4}\epsilon_0$. For any $h$ that is constant for any $w$ and $y\in\mathcal{Y}_j$. In addition, note that $\int_{\mathcal{X}_i}\int_{\mathcal{Y}_j}(f(y|x)-\int h_0(w,y)f(w|x)dw)dyf(x)dx=(\mathbb{P}(\tilde{y}_j|\tilde{x}_i-\int g_l(w)f(w|X\in\mathcal{X}_i)dw \mathbb{P}(\tilde{x}_i)$, where $g_l(w):=\int_{Y\in\mathcal{Y}_j} h_0(w,y)dy$. Therefore, we have $\sum_{i=1}^I \sum_{j=1}^J \int_{\mathcal{X}_i}|\int_{\mathcal{Y}_j} (f(y|x)-\int h_0(w,y)f(w|x)dw)dyf(x)dx|=\sum_{i=1}^I \sum_{j=1}^J||\mathbb{P}(\tilde{y}_j|\tilde{x}_i-\int g_l(w)f(w|X\in\mathcal{X}_i)dw||_2 \mathbb{P}(\tilde{x}_i)$.

    Recall that we have for any $I\leq\max(I_{0,1},I_{0,2}), J\leq \max(J_{0,1},J_{0,2})$ \xw{$I>\max(I_{0,1},I_{0,2})$, $J> \max(J_{0,1},J_{0,2})$}, we have $|\mathrm{res}^{M_w}(h)-\sum_{i=1}^I \sum_{j=1}^J|\mathbb{P}(\tilde{y}_j|\tilde{x}_i-\int g_l(w)f(w|X\in\mathcal{X}_i)dw|\mathbb{P}(\tilde{x}_i)\leq \frac{1}{2}\epsilon_0$. Then for any $I,J$, there exist $L_0$ such that for any $L>L_0$, we have $|\mathrm{res}^{M_w}(h)-\sum_{i=1}^I \sum_{j=1}^J|\mathbb{P}(\tilde{y}_j|\tilde{x}_i-\sum_k \mathbb{P}(\tilde{w}_k|\tilde{x}_i) g_l(w)f(w|X\in\mathcal{X}_i)dw|\mathbb{P}(\tilde{x}_i)\leq \frac{3}{4}\epsilon_0$. If $q=Q^T c$ for some $c=[[c_{1,1},...,c_{L,1}],...,[c_{1,J},...,C_{L,J}]]^T$, with $c_{l,i,j}=c_{l,i^',j}$, then we let $h(w,y)=c_{k,l}$ for $w\in\mathcal{W}_l,y\in\mathcal{Y}_j$ and have $\mathbb{P}(\tilde{y}_j|\tilde{x}_i)=\sum_l \mathbb{P}(\tilde{w}_k|\tilde{x}_i) c_{l,j}$. Therefore, we have $\sum_{i=1}^I\sum_{j=1}^J |\mathbb{P}(\tilde{y}_l|\tilde{x}_i)-\sum_l \mathbb{P}(\tilde{w}_l|\tilde{x}_i) g_l(\tilde{u}_l)|\mathbb{P}(\tilde{x}_i)=0$ for some $h$ that is constant in each $\mathcal{Y}_j$. Therefore, we have $\mathrm{res}^{M_w}(h)<\frac{3}{4}\epsilon_0$, which obtains the contradiction.

    \textbf{Part 2.} Given that $q\not \in \mathrm{im}(Q)$, we show $\lim_{n,L\to \infty} \mathbb{P}_{\Theta}(T\leq z_{1-\alpha})=0$. To show this, we first discuss the distribution of $T$ given $q\not \in \mathrm{im}(Q)$. First, we have $||\Omega_y \Sigma_y^{-1/2} q_y||^2_2>0$. To see this, note that $\mathrm{ker}(\Omega)=\mathrm{im}(\Sigma^{-1/2}Q^T)$\footnote{To see this, we have $\forall \vec{a}\in \mathrm{im}(\Sigma^{-1/2}Q^T), \exists \vec{b}, s.t. \vec{a} = \Sigma^{-1/2}Q^T \vec{b}$. Therefore, we have $\Omega \vec{a} = \Omega \Sigma^{-1/2}Q^T \vec{b} = \vec{0}$, which means $\mathrm{im}(\Sigma^{-1/2}Q^T)$ is the subspace of $\mathrm{ker}(\Omega)$. What is left is to show $\mathrm{dim}(\mathrm{im}(\Sigma^{-1/2}Q^T)) = \mathrm{dim}(\mathrm{ker}(\Omega))$. In details, since we have $\mathrm{rank}(\Sigma^{-1/2}Q^T)=L(J-1)$, we have $\mathrm{dim}(\mathrm{im}(\Sigma^{-1/2}Q^T)) = L(J-1)$. Since $\mathrm{rank}(\Omega)=(I-L)(J-1)$, we have $\mathrm{nul}(\Omega)=(I-(I-L))(J-1)=L(J-1)$ ($\mathrm{nul}(\Omega)$ is the null space of $\Omega$) and therefore $\mathrm{dim}(\mathrm{ker}(\Omega_y))=L(J-1)=\mathrm{dim}(\mathrm{im}(\Sigma^{-1/2}Q^T))$. Therefore, we have $\mathrm{ker}(\Omega)=\mathrm{im}(\Sigma^{-1/2}Q^T)$.} ($\mathrm{ker}(\Omega)$ is the kernel space of $\Omega$), therefore, $q\not \in \mathrm{im}(Q)$ means $\Sigma^{-1/2} q \not \in \mathrm{img}(\Sigma^{-1/2} Q^T) = \mathrm{ker}(\Omega_y)$, and we have $\Omega\Sigma^{-1/2} q \neq \vec{0}$ and $|| \Omega\Sigma^{-1/2} q ||^2_2>0$. Second, let $\vec{c} := \Omega_y \Sigma^{-1/2} q_y$, we show $T$ follows the noncentral chi square distribution $\chi^2(r,\lambda)$ with $\lambda=n||\vec{c}||^2_2$ \xw{$r=I-L$?}. To be specific, we have $\sqrt{n} (\xi - \vec{c}) \to N(0,\Omega)$ and therefore $\sqrt{n} \xi \to N(\sqrt{n}\vec{c}, \Omega)$. Repeating the orthogonal decomposition trick used in the proof of Theorem~\ref{thm.control.type-i}, we have:
    \begin{align*}
            T := n \xi^T \xi &\to N(\sqrt{n}\vec{c},\Omega)^T N(\sqrt{n}\vec{c},\Omega) = \{V N(\sqrt{n}\vec{c},\Omega)\}^T \{V N(\sqrt{n}\vec{c},\Omega)\} \\
            &= N(\sqrt{n}V\vec{c}, \mathrm{diag}(1,...,1,0,...,0))^T N(\sqrt{n}V\vec{c}, \mathrm{diag}(1,...,1,0,...,0)) = \chi^2(r,\lambda),
    \end{align*}

    Given that $T$ follows the noncentral $\chi^2(r,\lambda)$ distribution as $L\to\infty$, we then show $\lim_{n,L\to\infty}\mathbb{P}_{\Theta}(T\leq z_{1-\alpha})=0$. To show this, we use the $\epsilon-N$ language, that is $\forall \epsilon>0, \exists N, \forall n\geq N, \mathbb{P}_{\Theta}(T_y\leq z_{1-\alpha}) \leq\epsilon$ \xw{, which is equivalent to show that $\forall \epsilon>0, \exists N$...}. In details, denote $F(x;r,\lambda)$ the cdf of $\chi^2(r,\lambda)$ and let $f(\lambda):=F(\lambda;x,r)$ \xw{$F(x;r,\lambda)$?}. We first show for fixed ($x,r$) (the $x$ is $z_{1-\alpha}$ in our problem), $\lim_{\lambda\to\infty} f(\lambda) = 0$. Specifically, we first have $F(\lambda;x,r) = 1 - Q_{r/2}(\sqrt{\lambda},\sqrt{x})$ \xw{why?} \textcolor{blue}{see wiki of noncentral chi-sq distribution, it says the cdf has this derivation} \xw{According to \cite{nuttall1972some}, we can represent the cdf with Marcum Q function}, where
    
    \begin{align*}
        &Q_v(a,b) = 1 + H_v(a,b) + C_v(a,b) \\
        &H_v(a,b) = \frac{(a/b)^{1-v}}{2\pi} \mathrm{exp}(-\frac{1}{2}(a^2+b^2)) \int_{0}^{2\pi} \frac{\mathrm{cos}(v-1)\theta - (a/b)\mathrm{cos}(v\theta)}{1-2(a/b)\mathrm{cos}\theta + (a/b)^2} \mathrm{exp}(ab\mathrm{cos}\theta)\mathrm{d}\theta, \\
        &C_v(a,b) = \frac{\mathrm{sin}(v\pi)}{\pi} \mathrm{exp}(-\frac{1}{2}(a^2+b^2)) \int_0^1 \frac{x^{v-1} (b/a)^{v-1}}{(a/b)+x} \mathrm{exp}(-\frac{ab}{2}(x+\frac{1}{x})) \mathrm{d}x.
    \end{align*}

    Therefore, to show $\lim_{\lambda\to\infty} f(\lambda) = 0$, we show $\lim_{\lambda\to\infty} Q_{k/2}(\sqrt{\lambda},\sqrt{x}) = 0$, which needs $\lim_{a\to\infty} H_v(a,b) = 0$ and $\lim_{a\to\infty} C_v(a,b) = 0$. To see $\lim_{a\to\infty} H_v(a,b) = 0$, note that:
    \begin{align*}
        &\lim_{a\to \infty} \frac{(a/b)^{1-v}}{2\pi} = 0, \quad \hfill\#\, v \,\text{is a large number, so}\, 1-v<0, \\
        &\lim_{a\to \infty} \mathrm{exp}(-\frac{1}{2}(a^2+b^2)) \mathrm{exp} (ab\mathrm{cos}\theta) = 0, \quad \hfill\#\,\text{because}\, \lim_{a\to \infty}a^2-2ab\mathrm{cos}\theta+b^2 = \infty, \\
        &\lim_{a\to \infty} \frac{\mathrm{cos}(v-1)\theta-(a/b)\mathrm{cos}(v\theta)}{1-2(a/b)\mathrm{cos}\theta+(a/b)^2} = 0 \quad \#\, \text{this is like}\, \lim_{a\to \infty} \frac{a}{1-a+a^2}= 0.
    \end{align*}

    Therefore, use Lebesgue’s dominated convergence theorem (our integrand can be dominated by $1$ when $a$ is sufficiently large, and $1$ is an integrable function) to exchange the limitation and integration, we have $\lim_{a\to\infty} H_v(a,b) = 0$. A similar process can show $\lim_{a\to\infty} C_v(a,b) = 0$. Now, with $\lim_{\lambda\to\infty} f(\lambda) = 0$, we have $\forall \epsilon>0,\exists\, \Lambda,\forall\lambda>\Lambda, f(\lambda):=\mathbb{P}_{\chi^2(r,\lambda)}(T_y\leq z_{1-\alpha})\leq \epsilon$. Therefore, we have $\forall \epsilon>0,\exists N:=\frac{\Lambda}{||\vec{c}||^2_2},\forall n\geq N,\lambda:=n||\vec{c}||^2_2 \geq \Lambda$ and hence $\mathbb{P}_{\Theta}(T_y\leq z_{1-\alpha})\leq \epsilon$, which concludes the proof.
\end{proof}

\subsection{Characterization of the ``integral equation insolubility'' condition}

Theorem~\ref{thm.type-ii} involves an important but rather obscure condition that the integral equation $f(y|x)=\int h(y,w)f(w|x)dw$ is insolvable. Intuitively, this condition means the correlation between $X,Y$ can not be (totally) explained by that between $X,U$ and $U,Y$. Although we can not yet provide a thorough theoretic characterization (\xw{we do not need to claim this?} \textcolor{blue}{is it necessary to say something like the theoretic characterization is challenging?} \xw{Not necessary unless we can figure out the reason and clearly present it?}), we in Figure~\ref{fig.exam-integral-equation-no-solution} provide several examples, which shows that this condition generally holds when $X\not\perp Y|U$ and the correlation between $X,Y$ is strong.

\begin{figure*}[th]
    \centering
    \includegraphics[width=\textwidth]{icml24_figs/intgeral_solution.pdf}
    \caption{\xw{shall we put settings of structural equations in the text?} Insolubility of the integral equation when $X\not\perp Y|U$. We consider four examples, namely the linear Gaussian model, the linear nonGaussian model, the nonlinear additive noise model, and the general nonlinear models. For each example, we report the averaged residual of the best fit of the integral equation $f(y|x)=\int h(y,w)f(w|x)dw$ wrt to the correlation strength of $X$ and $Y$. As we can see, when $X$ and $Y$ become correlated ($X\not\perp Y|U$), the residual becomes non-zero, indicating the insolubility of the integral equation. }
    \label{fig.exam-integral-equation-no-solution}
\end{figure*}


\xw{do we need to present a theorem to characterize conditions when the solution exists under $H_1$?} \textcolor{blue}{if you think we should, i can put it on :)}

Indeed, the following example shows that the solution may exist even when $\mathbb{H}_1:X\not\ind Y|U$ holds.


\subsection{Estimating the conditional probability vector}
\label{app-sec.mle}

Consider discrete random variables $X,Y$ that (respectively) take values $\{x_1,...,x_I\}$ and $\{y_1,...,y_J\}$. Suppose that we have $n$ iid samples. Denote $Z_{ij}$ the number of samples that take the value $(x_i,y_j)$, and denote $Z_{i:}:=\sum_j Z_{ij}$. Then, the MLE estimator of conditional probability vector $P(y|X)$ is $\hat{P}(y|X) = \left[\hat{p}(y|x_1),...,\hat{p}(y|x_I)\right]$, where $\hat{p}(y_j|x_i) = Z_{ij}/Z_{i:}$.

The MLE estimator satisfies that $\hat{P}(y|X)\to P(y|X)$ in probability, and that $n^{1/2}(\hat{P}(y|X)-P(y|X)) \to N(0,\Sigma)$ in distribution. The covariance matrix is $\Sigma=\mathrm{diag}[\frac{p(y_j|x_1)(1-p(y_j|x_1))}
{p(x_1)},...,\frac{p(y_j|x_I)(1-p(y_j|x_I))}{p(x_I)}]$ and is positive definite. The corresponding estimator $\hat{\Sigma}$ that satisfies $\hat{\Sigma}\to \Sigma$ in probability can be obtained by replacing $p(y_j|x_i)$ with $\hat{p}(y_j|x_i)$, and replacing $p(x_i)$ with $\hat{p}(x_i)=Z_{i:}/n$\footnote{These results are obtained by noting that $Z_{ij}$ follows the multinomial distribution, and by applying the Fisher information matrix (in the sandwich form) and the Cramer-Rao lower bound \cite{casella2021statistical} (Theorem 7.3.9).}.




==> icml24_para/abstract.tex <==
\begin{abstract}
    Identifying causal relationships from observational data is desirable. The existence of unobserved variables, such as the latent confounder, can mislead the causal identification. To address this issue, proximal causal discovery methods proposed to adjust for the bias using the proxy of the unobserved variable. However, these methods were either limited to the discrete case or relied on strong parametric assumptions for identification. In this paper, we propose a proxy-based hypothesis testing procedure to examine the existence of the causal relationship, without any parametric constraint. Specifically, we first discretize the variables, then connect the null causal hypothesis to the identification problem of a linear system over the discretized variables. Under the completeness and smoothness assumptions, we show that one can construct proper discretization so that the established linear system is identifiable, and hence the null hypothesis is testable. Based on this, we introduce our test statistic, and demonstrate the asymptotic level and power of our test. Theoretical advantages are reflected in synthetic and real-world experiments.
\end{abstract}

==> icml24_para/abstract_xw.tex <==
\begin{abstract}
    Bivariate causal discovery from observational data is important in many scenarios. However, the presence of unobserved variables, such as the latent confounder, can mislead the causal identification. To address this issue, proximal causal learning proposed to adjust for the bias using the proxy of the unobserved variable. However, these methods were either limited to categorical variables or relied on strong parametric assumptions for identification. In this paper, we propose a novel hypothesis testing procedure that can effectively examine the existence of the causal relationship over continuous variables, without any parametric constraint. Our procedure is based on discretization, which under completeness condition, is able to asymptotically establish a linear equation whose coefficient vector is identifiable under causal null hypothesis. Based on this, we introduce our test statistic, and demonstrate the asymptotic level and power of our test. We validate the effectiveness of our procedure using both synthetic and real-world data.
    
    %Specifically, we first discretize the variables, then connect the null causal hypothesis to the identification problem of a linear system over the discretized variables. Under the completeness and smoothness assumptions, we show that one can construct proper discretization so that the established linear system is identifiable, and hence the null hypothesis is testable. 
    
    
\end{abstract}

==> icml24_para/conclusion.tex <==
\section{Conclusion and discussion}

In this paper, we propose a proxy-based hypothesis testing procedure for bivariate causal discovery. Our procedure involves the discretization of continuous variables, for which we provide comprehensive analyses for the identifiability of the system over discretized variables, and meanwhile controlling the discretization errors. Benefiting from these, our test enjoys uniform level and power, asymptotically.

\textbf{Limitation and future work.} Our method relies on discretization and hence may be affected by the dimension of the conditional variable. Indeed, the curse of dimensionality is a common issued faced by all conditional independence (CI) tests used for causal discovery, as noticed by \cite{ramdas2015decreasing}. For alleviation, we will investigate theories on high dimensional discretization (\citealt{van2014probability}, Lem.~5.12) for a delicate solution. Besides, we are also interested in plugging our test to multivariate causal discovery algorithms such as the FCI \cite{spirtes2000causation}, to enhance their ability for structure identification.

==> icml24_para/conclusion_xw.tex <==
\section{Conclusion and discussion}

In this paper, we propose a proxy-based hypothesis testing procedure for bivariate causal discovery. Our procedure involves the discretization of continuous variables, for which we control the discretization errors in  a linear system over discretized variables, and meanwhile establishing the identifiability of such a linear system. Benefiting from these, our test enjoys uniform level and power, asymptotically.

% establish identifiability of the linear system over discretized variables, and meanwhile controlling the discretization errors. 

\textbf{Limitations and future works.} Our method relies on discretization and hence may lose its power when the dimension of the conditional variable is high. Indeed, such a curse of dimensionality issue is common in all conditional independence (CI) tests, as noticed by \cite{ramdas2015decreasing}. For alleviation, we will investigate theories on high dimensional discretization (\citealt{van2014probability}, Lem.~5.12) for a delicate solution. Besides, we are also interested in plugging our test to multivariate causal discovery algorithms such as the FCI \cite{spirtes2000causation}, to enhance their ability for structure identification.

==> icml24_para/dis_err_v4_xw.tex <==

\subsection{Discretization error analysis}
\label{sec.dis-error}

In this section, we discuss the discretization error control. Our goal is to asymptotically maintain the conditional independence $X\ind Y|U$ and $X\ind W|U$ after discretization by controlling the error $|p(\tilde{y}|\tilde{u})-p(\tilde{y}|\tilde{x},\tilde{u})|$ and $|p(\tilde{w}|\tilde{u})-p(\tilde{w}|\tilde{x},\tilde{u})|$ over discretized variables under the null hypothesis $\mathbb{H}_0$, which allows us to establish the linear relation in Eq.~\eqref{eq.miao} asymptotically. 


For this purpose, we first introduce the following Total Variation (TV) smoothness condition, which states that the conditional distributions $\mathcal{L}_{Y|U=u}$ and $\mathcal{L}_{W|U=u}$ should change smoothly with respect to $u$.


\begin{assumption}[TV smoothness]
\label{asm.tv-smooth-main}
    We assume the maps $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are Lipschitz continuous with respect to TV distance. That is, for any $u,u^\prime \in \mathcal{U}$, we assume there exist $L_Y$ and $L_W$, respectively, such that:
    \begin{align*}
        \mathrm{TV}(\mathcal{L}_{Y|U=u},&\mathcal{L}_{Y|U=u^\prime}) \leq L_Y |u-u^\prime|, \\
        \mathrm{TV}(\mathcal{L}_{W|U=u},&\mathcal{L}_{W|U=u^\prime}) \leq L_W |u-u^\prime|,
    \end{align*}
    where $\mathrm{TV}(P_1,P_2) := \sup_A \left| \int_A (p_1(x) - p_2(x)) dx\right|$.
\end{assumption}



To understand the role of assump.~\ref{asm.tv-smooth-main} in discretization error control, note that for a small bin $\mathcal{U}_i$ of $\mathcal{U}$ and any $u\in\mathcal{U}_i$, assump.~\ref{asm.tv-smooth-main} means that the distance
\begin{equation*}
    \mathrm{TV}(\mathcal{L}_{Y|U\in \mathcal{U}_i},\mathcal{L}_{Y|U=u})
\end{equation*}
is small. Similarly, it also indicates that the distance
\begin{equation*}
    \mathrm{TV}(\mathcal{L}_{Y|X\in\mathcal{X}_j,U\in \mathcal{U}_i},\mathcal{L}_{Y|X\in\mathcal{X}_j,U=u})
\end{equation*}
is small. Since we have $\mathcal{L}_{Y|U=u}=\mathcal{L}_{Y|X\in\mathcal{X}_j,U=u}$ under $\mathbb{H}_0: X\ind Y|U$, by applying triangle inequality, we can control the distance $\mathrm{TV}(\mathcal{L}_{Y|U\in \mathcal{U}_i},\mathcal{L}_{Y|X\in\mathcal{X}_j,U\in \mathcal{U}_i})$, and hence control the error $|p(\tilde{y}|\tilde{u})-p(\tilde{y}|\tilde{x},\tilde{u})|$. The $|p(\tilde{w}|\tilde{u})-p(\tilde{w}|\tilde{x},\tilde{u})|$ can be controlled in a similar way when $\mathrm{TV}(\mathcal{L}_{W|U=u},\mathcal{L}_{W|U=u^\prime})$ is small. 

The following example shows that assump.~\ref{asm.tv-smooth-main} can hold for a wide range of ANM models.


\begin{example}[ANM with TV smoothness]
    Suppose that $Y,U,W$ satisfy the ANM, i.e., $Y=g_Y(U)+N_Y, W=g_W(U)+N_W$, with $N_Y, N_W$ being the noises. If $g_Y$ and $g_W$ are differentiable, and the probability densities of $N_Y$ and $N_W$ have absolutely integrable derivatives, then the maps $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are Lipschitz continuous with respect to TV distance.
    \label{exam.tv-smooth}
\end{example}

\begin{remark}
    We also provide an example where $U$ is a mediator. Please refer to Appx.~\ref{app-sec.tv-example} for details.
\end{remark}


Under this assumption, we show that the discretization error can be controlled, as long as the bin length is small.
\begin{proposition}
\label{prop.control-err-main}
    Suppose that $\{\mathcal{U}_i\}_{l_{U}}$ is a partition of $\mathcal{U}$, and that for every bin $\mathcal{U}_i$,
    \begin{equation*}
        len(\mathcal{U}_i)\leq \frac{1}{2}min\{\epsilon/L_Y,\epsilon/L_W\}.
    \end{equation*}
    Then, under assump.~\ref{asm.tv-smooth-main} and $\mathbb{H}_0:X\ind Y|U$, we have:
    \begin{align*}
        |p(\tilde{y}|\tilde{u}_i) - p(\tilde{y}|\tilde{x},\tilde{u}_i)| \leq \epsilon, \,\, |p(\tilde{w}|\tilde{u}_i) - p(\tilde{w}|\tilde{x},\tilde{u}_i)| \leq \epsilon.
    \end{align*}
\end{proposition}
According to Prop.~\ref{prop.control-err-main}, when $\mathcal{U}$ is a compact interval, we can (implicitly) partition $\mathcal{U}$ into sufficiently refined bins, by setting the bin number large enough. However, when considering $\mathcal{U}=\mathbb{R}$, it is intractable to partition into finite bins with finite length. To extend the above result to $\mathbb{R}$, we assume $\mathcal{L}_{U|X}$ to be tight, meaning that for large values of $u$'s, the conditional probability $p(u|x)$ is close to zero. The formal definition of tight distribution is given below. 


\begin{definition}[Tight distribution] The marginal distribution $\mathcal{L}_U$ is said to be tight if $\forall \epsilon>0, \exists t_0, \forall t\geq t_0,\mathcal{L}(|U|\geq t)\leq \epsilon$. The conditional distribution $\mathcal{L}_{U|X}$ is said to be uniformly tight in $[a,b]$ if $\forall \epsilon>0, \exists t_0, \forall t\geq t_0, \forall x\in [a,b],\mathcal{L}(|U|\geq t|x)\leq \epsilon$.
\label{def.tight-main}
\end{definition}
% \footnote{We use the term ``uniform'' because it holds uniformly for all $x\in[a,b]$.}

We then assume the following tightness condition:
\begin{assumption}
    We assume the conditional distribution $\mathcal{L}_{U|X}$ is uniformly tight for any compact interval $[a,b]$.
    \label{asm.tight-main}
\end{assumption}

To see the role of assump.~\ref{asm.tight-main} in discretization error control under non-compact domains, note that we can partition $\mathcal{U}$ into a compact part $\mathcal{U}_c$ and a non-compact part $\mathcal{U}_{nc}$, whose errors can be respectively controlled by exploiting Prop.~\ref{prop.control-err-main} and assump.~\ref{asm.tight-main}. In this way, we can establish Eq.~\eqref{eq.miao} asymptotically with respect to the bin length. 

The following example shows that assump.~\ref{asm.tight-main} can easily hold when the distribution of the noise is tight.
\begin{example}[ANM with tightness]
    Suppose that $X$ and $U$ satisfy the ANM, i.e., $X=g_X(U)+N_X$, with $N_X$ the noise. As long as $g_X$ is invertible and the distribution of $N_X$ is tight\footnote{This holds for many distributions, including those from the exponential family.}, then $\mathcal{L}_{U|X}$ is uniformly tight in an arbitrary compact interval $[a,b]$.
    \label{exam.anm.tight}
\end{example}


Equipped with assump.~\ref{asm.tight-main}, we have the following result for controlling the discretization error induced by the non-compact part of the domain $\mathcal{U}$.

\begin{proposition}
    Suppose that $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$, and that the map $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz continuous wrt TV distance. Suppose that $\{\mathcal{X}_i\}_{l_X}$ is a partition of $[a,b]$ satisfying $len(\mathcal{X}_i)\leq \epsilon/2L_U$. Then, $\forall\epsilon>0, \exists T$, let $\mathcal{U}_{nc}:=\{u:|u|\geq T\}$, we have $p(\tilde{u}_{nc}|\tilde{x}_i) \leq \epsilon$.
    \label{prop.dis-err unbd}
\end{proposition}

Prop.~\ref{prop.dis-err unbd} means that we can take a compact subspace of $\mathcal{X}$ for discretization to establish Eq.~\eqref{eq.miao}, since the additional error introduced by the non-compact part of $\mathcal{U}$ can be effectively controlled.


==> icml24_para/dis_err_v5_mz.tex <==
% older version at dis_err_v4_xw.tex

\subsection{Discretization error analysis}
\label{sec.dis-error}

In this section, we discuss the discretization error control. Given $\mathbb{H}_0:X\ind Y|U$ and $X\ind W|U$, our goal is to have:
\begin{subequations}
\label{eq.dis-ind}
\begin{align}
    P(\tilde{y}|\tilde{X})&=P(\tilde{y}|\tilde{U}) P(\tilde{U}|\tilde{X}) + E_y, \\
    P(\tilde{W}|\tilde{X})&=P(\tilde{W}|\tilde{U}) P(\tilde{U}|\tilde{X}) + E_w,
\end{align}
\end{subequations}
with the error terms $E_y$ and $E_w$ controlled to zeros asymptotically. In this regard, we can establish the linear relationships in Eq.~(\ref{eq.miao}) asymptotically. 

We first consider cases where $\mathcal{U}$ is a compact set, then extend the results to $\mathcal{U}=\mathbb{R}$. Specifically, when $\mathcal{U}$ is a compact interval, we can partition $\mathcal{U}$ into sufficiently many bins, such that in each small bin, the distances  $|p(\tilde{y}|\tilde{u})-p(\tilde{y}|\tilde{x},\tilde{u})|$ and $|p(\tilde{w}|\tilde{u})-p(\tilde{w}|\tilde{x},\tilde{u})|$ are close. To achieve this, we first introduce the following smoothness condition which ensures the conditional distribution does not vary too much in each small bin:

\begin{assumption}[TV smoothness]
\label{asm.tv-smooth-main}
    We assume that the maps $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are Lipschitz continuous wrt the Total Variation (TV) distance. That is, for any $u,u^\prime \in \mathcal{U}$, we assume there exist $L_Y$ and $L_W$ such that:
    \begin{align*}
        \mathrm{TV}(\mathcal{L}_{Y|U=u},&\mathcal{L}_{Y|U=u^\prime}) \leq L_Y |u-u^\prime|, \\
        \mathrm{TV}(\mathcal{L}_{W|U=u},&\mathcal{L}_{W|U=u^\prime}) \leq L_W |u-u^\prime|,
    \end{align*}
    respectively, with $\mathrm{TV}(\mathcal{L}_1,\mathcal{L}_2):=\sup_A |\mathcal{L}_1(A)-\mathcal{L}_2(A)|$.
\end{assumption}



To understand the role of Asm.~\ref{asm.tv-smooth-main} in controlling the distance $|p(\tilde{y}|\tilde{u})-p(\tilde{y}|\tilde{x},\tilde{u})|$, note that for a small bin $\mathcal{U}_i$ of $\mathcal{U}$ and any $u\in\mathcal{U}_i$, Asm.~\ref{asm.tv-smooth-main} means that the distance:
\begin{equation*}
    \mathrm{TV}(\mathcal{L}_{Y|U\in \mathcal{U}_i},\mathcal{L}_{Y|U=u})
\end{equation*}
is close. Similarly, it also indicates that the distance:
\begin{equation*}
    \mathrm{TV}(\mathcal{L}_{Y|X\in\mathcal{X}_j,U\in \mathcal{U}_i},\mathcal{L}_{Y|X\in\mathcal{X}_j,U=u})
\end{equation*}
is close. Since we have $\mathcal{L}_{Y|U=u}=\mathcal{L}_{Y|X\in\mathcal{X}_j,U=u}$ under $\mathbb{H}_0: X\ind Y|U$, by applying the triangle inequality, we can control the distance $\mathrm{TV}(\mathcal{L}_{Y|U\in \mathcal{U}_i},\mathcal{L}_{Y|X\in\mathcal{X}_j,U\in \mathcal{U}_i})$, and hence control the term $|p(\tilde{y}|\tilde{u})-p(\tilde{y}|\tilde{x},\tilde{u})|$. 


The following example shows that Asm.~\ref{asm.tv-smooth-main} can hold for a wide range of ANM models.

\begin{example}[ANM with TV smoothness]
    Suppose that $Y,U,W$ satisfy the ANM, \emph{i.e.}, $Y=g_Y(U)+N_Y, W=g_W(U)+N_W$, with $N_Y, N_W$ being the noises. If $g_Y$ and $g_W$ are differentiable, and the probability densities of $N_Y$ and $N_W$ have absolutely integrable derivatives, then the maps $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are Lipschitz continuous with respect to TV distance.
    \label{exam.tv-smooth}
\end{example}

% 注 这里不需要区分 U 是 mediator 还是 confounder, 因为不涉及 X

Under Asm.~\ref{asm.tv-smooth-main}, we can control the discretization error as long as the length of the bin is sufficiently small. This is summarized as the following proposition:

\begin{proposition}
\label{prop.control-err-main}
    Suppose that $\{\mathcal{U}_i\}_{l_{U}}$ is a partition of $\mathcal{U}$, and that for every bin $\mathcal{U}_i$,
    \begin{equation*}
        len(\mathcal{U}_i)\leq \frac{1}{2}min\{\epsilon/L_Y,\epsilon/L_W\}.
    \end{equation*}
    Then, under Asm.~\ref{asm.tv-smooth-main} and $\mathbb{H}_0:X\ind Y|U$, we have:
    \begin{align*}
        |p(\tilde{y}|\tilde{u}_i) - p(\tilde{y}|\tilde{x},\tilde{u}_i)| \leq \epsilon, \,\, |p(\tilde{w}|\tilde{u}_i) - p(\tilde{w}|\tilde{x},\tilde{u}_i)| \leq \epsilon.
    \end{align*}
\end{proposition}

According to Prop.~\ref{prop.control-err-main}, when $\mathcal{U}$ is a compact interval, we can (implicitly) partition $\mathcal{U}$ into sufficiently refined bins, by setting the bin number large enough. However, when considering $\mathcal{U}=\mathbb{R}$, it is intractable to partition into finite bins with finite length. To extend the above result to $\mathbb{R}$, we further assume the conditional distribution $\mathcal{L}_{U|X}$ to be tight, meaning that for large values of $u$'s, the conditional probability $p(u|x)$ is close to zero. The formal definition of tight distribution is given below. 


\begin{definition}[Tight distribution] The marginal distribution $\mathcal{L}_U$ is said to be tight if $\forall \epsilon>0, \exists t_0, \forall t\geq t_0,\mathcal{L}(|U|\geq t)\leq \epsilon$. The conditional distribution $\mathcal{L}_{U|X}$ is said to be uniformly tight in $[a,b]$ if $\forall \epsilon>0, \exists t_0, \forall t\geq t_0, \forall x\in [a,b],\mathcal{L}(|U|\geq t|x)\leq \epsilon$.
\label{def.tight-main}
\end{definition}

We then assume the following tightness condition:
\begin{assumption}
    We assume the conditional distribution $\mathcal{L}_{U|X}$ is uniformly tight for any compact interval $[a,b]$.
    \label{asm.tight-main}
\end{assumption}

To understand the role of Asm.~\ref{asm.tight-main} when $\mathcal{U}=\mathbb{R}$, note that for the limiting ends of $\mathcal{U}$, the probability $p(u|x)$ and hence $p(y|u,x)p(u|x), p(w|u,x)p(u|x)$ vanish to zero, and do not affect to the error terms $E_y, E_w$ anymore. 

The following example shows that Asm.~\ref{asm.tight-main} can easily hold when the distribution of the noise is tight.
\begin{example}[ANM with tightness]
    Suppose that $X$ and $U$ satisfy the ANM, \emph{i.e.}, $X=g_X(U)+N_X$, with $N_X$ being the noise. If $g_X$ is invertible and the distribution of $N_X$ is tight\footnote{E.g., distributions from the exponential family.}, then $\mathcal{L}_{U|X}$ is uniformly tight in an arbitrary compact interval $[a,b]$.
    \label{exam.anm.tight}
\end{example}


Equipped with assump.~\ref{asm.tight-main}, we have the following result for controlling the discretization error induced by the non-compact part of the domain $\mathcal{U}$.

\begin{proposition}
    Suppose that $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$, and that the map $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz continuous wrt TV distance. Suppose that $\{\mathcal{X}_i\}_{l_X}$ is a partition of $[a,b]$ satisfying $len(\mathcal{X}_i)\leq \epsilon/2L_U$. Then, $\forall\epsilon>0, \exists T$, let $\mathcal{U}_{nc}:=\{u:|u|\geq T\}$, we have $p(\tilde{u}_{nc}|\tilde{x}_i) \leq \epsilon$.
    \label{prop.dis-err unbd}
\end{proposition}

Prop.~\ref{prop.dis-err unbd} means that we can take a compact subspace of $\mathcal{X}$ for discretization to establish Eq.~\eqref{eq.miao}, since the additional error introduced by the non-compact part of $\mathcal{U}$ can be effectively controlled.


==> icml24_para/hypo_test_v4_xw.tex <==
\subsection{Hypothesis test}
\label{sec.hypo-test}

In this section, we present our hypothesis testing procedure. Specifically, we adopt the test statistic proposed by \cite{miao2018identifying} and analyze its asymptotic distribution under the null hypothesis. Additionally, we investigate the behavior of the statistic under the alternative hypothesis and establish the asymptotic power of our test.

We first introduce our test statistic. The idea is that we can assess whether $\mathbb{H}_0$ is correct by looking at the residual of the least-square solution of Eq.~\eqref{eq.miao}. If $\mathbb{H}_0$ is correct, then the linear relation in Eq.~\eqref{eq.miao} holds, hence the least-square residual should be close to zero. In practice, to enhance the capacity of the statistic, we can aggregate the residuals obtained from the solutions of Eq.~\eqref{eq.miao} with respect to all levels of $\tilde{Y}$. Specifically, we let
\begin{equation*}
    q:=[P(\tilde{y}_1|\tilde{X}),...,P(\tilde{y}_{l_{\tilde{Y}}-1}|\tilde{X})]^T
\end{equation*}
be the column vector that aggregates $P(\tilde{y}|\tilde{X})$ for all (free) levels of $\tilde{Y}$, and let
\begin{equation*}
    Q:=\mathrm{diag}[P(\tilde{W}|\tilde{X}),...,P(\tilde{W}|\tilde{X})]
\end{equation*}
be the block diagonal matrix with $(l_{\tilde{Y}}-1)$ repeating blocks of $P(\tilde{W}|\tilde{X})$ in the diagonal. After performing maximum likelihood estimation\footnote{Please refer to Appx.~\ref{app-sec.mle} for details.}, we can estimate $\hat{q}$ and $\hat{Q}$, such that
\begin{align*}
    n^{1/2}(\hat{q} - q) &\to N(0,\Sigma) \,\, \text{in distribution}, \\
    \hat{Q}\to Q, \hat{\Sigma} &\to \Sigma \,\, \text{in probability,} 
\end{align*}
with $\hat{\Sigma}, \Sigma$ both positive definite. Then, we have the least-square residual of regressing $\hat{\Sigma}^{-1/2} \hat{q}$ on $\hat{\Sigma}^{-1/2} \hat{Q}$ to be
\begin{equation*}
    \xi := \{I - \hat{\Sigma}^{-1/2} \hat{Q}^T (\hat{Q} \hat{\Sigma}^{-1} \hat{Q}^T)^{-1} \hat{Q} \hat{\Sigma}^{-1/2}\} \hat{\Sigma}^{-1/2} \hat{q}.
\end{equation*}
Following \cite{miao2018identifying}, we adopt the squared residual $T_{n,l_{\tilde{X}},l_{\tilde{Y}},l_{\tilde{W}}}:=n\xi^T \xi$ as our test statistic. 

In the following, we show that $T_{n,l_{\tilde{X}},l_{\tilde{Y}},l_{\tilde{W}}}$ asymptotically follows a chi-squared distribution $\chi^2_k$, where the degree of freedom $k=(l_{\tilde{X}}-l_{\tilde{W}})(l_{\tilde{Y}}-1)$ is determined by the additional levels that $\tilde{X}$ has beyond $\tilde{W}$, multiplied by the level of $\tilde{Y}$. Formally, denote $z_{1-\alpha}$ as the $(1-\alpha)$-th quantile of $\chi^2_k$, we have the following result:


\begin{theorem}
    Suppose that assump.~\ref{asm.comp-main},~\ref{asm.tv-smooth-main},~\ref{asm.tight-main} hold, then under $H_0$, we have that:
    \begin{equation*}
        T_{n,l_{\tilde{X}},l_{\tilde{Y}},l_{\tilde{W}}} \to \chi_{k}^2 \,\, \text{in distribution, as $n,l_{\tilde{X}}, l_{\tilde{W}}\to \infty$.}
    \end{equation*}
    As a result, for any $\alpha\in (0,1)$, we have:
    \begin{equation*}
        \lim_{n,l_{\tilde{X}}, l_{\tilde{W}}\to \infty} P(T_{n,l_{\tilde{X}},l_{\tilde{Y}},l_{\tilde{W}}}> z_{1-\alpha}) = \alpha.
    \end{equation*}
    In other words, the testing procedure we define has uniform asymptotic level $\alpha$.
\label{thm.control.type-i-main}
\end{theorem}

In general, we cannot expect that the test has power against alternatives to $\mathbb{H}_0$ without further restrictions on the alternative distribution. This is analogous to other conditional independence tests \cite{zhang2012kernel,runge2018conditional,christgau2023nonparametric} used for causal discovery. Therefore, to establish the power of our test, we put the following restriction on the alternative distribution:

\begin{assumption}
    We consider the local alternative $\mathbb{H}_1$, such that the following integral equation has no solution:
    \begin{equation}
        p(y|x)=\int h(y,w)p(w|x)dw.
    \label{eq.int-eq}
    \end{equation}
    \label{asm.int-eq-main}
\end{assumption}
\begin{remark}
    Empirically, we find that this assumption can hold in many cases under $X\not\ind Y|U$, as shown in Appx.~\ref{app-sec.int-eq}. Besides, we can prove that $\mathbb{H}_1$ is indeed a local alternative, that is, there exists $P$ satisfying $X\not\ind Y|U$ but does not satisfy assump.~\ref{asm.int-eq-main}. See Appx.~\ref{app-sec.int-eq} for details.
\end{remark}

To understand the role of assump.~\ref{asm.int-eq-main} in controlling the type-II error, we first note that the residues in $T$ should deviate from zero under the alternative model, which requires that Eq.~\eqref{eq.miao} has no solution. Intuitively, this means the variability of $P(\tilde{y}|\tilde{X})$ can not be fully explained $P(\tilde{W}|\tilde{X})$, which corresponds assump.~\ref{asm.int-eq-main} for continuous variables. On the other hand, we can show in Appx.~\ref{app-sec.int-eq} that the solution in Eq.~\eqref{eq.int-eq} exists under $\mathbb{H}_0$. Therefore, we can employ it to effectively distinguish $\mathbb{H}_0$ from the alternative. 

% Please refer to Appx.~\ref{app-sec.int-eq} for details.

Under this assumption, we can establish the asymptotic power for our testing procedure.  
\begin{theorem}
    Suppose that assump.~\ref{asm.comp-main},~\ref{asm.tv-smooth-main},~\ref{asm.tight-main},~\ref{asm.int-eq-main} hold, then for any $\alpha\in (0,1)$, we have that:
    \begin{equation*}
        \lim_{n,l\to\infty}P(T_{n,l}>z_{1-\alpha})=1.
    \end{equation*}
    In other words, the limiting power of our test is one.
    \label{thm.type-ii-main}
\end{theorem}

==> icml24_para/introduction.tex <==
\section{Introduction}

Causal discovery has gained increasing popularity due to its wide applications in science and machine learning. In particular, the bivariate case, which involves determining whether the causal relationship exists between two variables, constitutes the most fundamental aspect. While the golden standard for causal discovery remains the randomized controlled trial (RCT), it can be too expensive, unethical, or even impossible to conduct in the real world. For these considerations, it is desired to identify bivariate causal relationships from purely observational data.

However, a significant obstacle when attempting to draw causal conclusions from observational data is the problem of \emph{unobserved variables}, such as unobserved confounders and mediators. These variables describe the intrinsic characteristics that are widely present but difficult to quantify (\emph{e.g.}, health status, gene). The ignorance of them can lead to non-vanishing bias for causal discovery, even with an infinite number of samples \cite{pearl2009causality}.

To address this problem, recent studies have proposed using a proxy variable to correct for the bias induced by the unobserved variable. Here, the proxy variable can be a noisy measurement \cite{kuroki2014measurement} or an observed descendant \cite{liu2023causal} of the unobserved variable, from which useful information about the bias can be inferred. Examples include \cite{tchetgen2020introduction,deaner2021many,sverdrup2023proximal} that explored proxy variables for causal effect estimation; \cite{dukes2023proximal,ghassami2021proximal} that studied proximal mediation analysis; and \cite{liu2023causal,miao2018identifying,miao2022identifying} that leveraged the proxy variable for causal discovery. Particularly, the recent hypothesis testing-based methods \cite{miao2018identifying,miao2022identifying} introduced various testing procedures to examine the null hypothesis of no causal relationship, using the proxy variable. However, their procedures were either limited to the discrete case or relied on strong parametric assumptions.

In this paper, we propose a novel hypothesis testing procedure to identify the causal relationship between two continuous variables, without any parametric assumption. Our strategy here is to first discretize the variables, then connect the null hypothesis of no causal relationship to the identification problem of a system of linear equations. We show that, given proper discretization, the linear system we establish is identifiable and hence the null hypothesis is testable. For this purpose, we first introduce a discretization process which, under the completeness assumption, can ensure the discretized variables meet the rank regularities. Then, we analyze the errors induced during the discretization and show that they can be controlled to arbitrarily small, given smooth structural equations and sufficiently many bins. Finally, based on the above analyses, we introduce our testing statistic and demonstrate the asymptotic level and power of our test. Using both synthetic and real-world data, we demonstrate the validity and effectiveness of our procedure.

We summarize our contributions as follows:
\begin{enumerate}[noitemsep,topsep=1pt]
    \item We propose a discretization-based procedure for bivariate causal discovery using the proxy variable.
    \item We introduce a discretization process that renders the rank regularity over discretized variables. 
    \item We demonstrate the effectiveness of our procedure on synthetic and real-world datasets.
\end{enumerate}


==> icml24_para/introduction_xw.tex <==
\section{Introduction}

% Causal discovery has gained increasing popularity due to its wide applications in science and machine learning. In particular, the bivariate case, which involves determining whether the causal relationship exists between two variables, constitutes the most fundamental aspect. While the golden standard for causal discovery remains the randomized controlled trial (RCT), it can be too expensive, unethical, or even impossible to conduct in the real world. For these considerations, it is desired to identify bivariate causal relationships from purely observational data.

Bivariate causal discovery from observational data is fundamental in uncovering causal relationships within a system, especially in scenarios where it is expensive, unethical or even impractical to conduct controlled experiment, including domains like finance, healthcare, and social science. Although there have been many studies in this field \cite{shimizu2006linear, hoyer2008nonlinear, mitrovic2018causal, blobaum2018cause, tagasovska2020distinguishing}, most of these works focused on learning causal direction, rather than determining whether the causal relation exists, which is however crucial to differentiate causation from spurious correlation such as counfounding bias or mediation bias. 


% A key challenge  when attempting to draw casual conclusions from observational data is the problem of \emph{unobserved variables}, such as unobserved confounders and mediators. These variables describe the intrinsic characteristics that are widely present but difficult to quantify (\emph{e.g.}, health status, gene). The ignorance of them can lead to non-vanishing bias for causal discovery, even with an infinite number of samples \cite{pearl2009causality}.


A key challenge in drawing casual conclusions from observational data comes from the presence of \emph{unobserved variables}, such as latent confounders or mediators. Typically, these variables refer to attributes that are difficult to measure (\emph{e.g.}, health status, living habits) but exhibit correlations to both variables within the specific pair of causal interest. The ignorance of them in the testing procedure can incur biases for causal discovery \cite{pearl2009causality}.


To address this challenge, recent studies in proximal causal learning introduced proxy variables, which can be a noisy measurement \cite{kuroki2014measurement} or the descendant \cite{miao2018identifying} of the unobserved variables, to adjust for the bias caused by unobserveness. Examples include \cite{tchetgen2020introduction,deaner2021many,sverdrup2023proximal} that explored proxy variables for causal effect estimation; \cite{dukes2023proximal,ghassami2021proximal} that studied proximal mediation analysis. However, most of these works focused on causal inference. The works that are mostly related to us are \cite{miao2018identifying} and \cite{miao2022identifying}, which introduced testing procedures to examine the null hypothesis of no causal relationship. However, their procedures were either limited to the discrete variables \cite{miao2018identifying} or relied on strong parametric assumptions to ensure the testing validity \cite{miao2022identifying}.

% and \cite{liu2023causal,miao2018identifying,miao2022identifying} that leveraged the proxy variable for causal discovery. 

% Particularly, the recent hypothesis testing-based methods \cite{miao2018identifying,miao2022identifying} introduced various testing procedures to examine the null hypothesis of no causal relationship, using the proxy variable. However, their procedures were either limited to the discrete case or relied on strong parametric assumptions.



%To adjust for this bias, recent studies have proposed proximal causal learning, which introduced proxy variables to infer the information of unobserved variables. Here, the proxy variable can be a noisy measurement \cite{kuroki2014measurement} or an observed descendant \cite{liu2023causal} of the unobserved variable, from which useful information about the bias can be inferred. Examples include \cite{tchetgen2020introduction,deaner2021many,sverdrup2023proximal} that explored proxy variables for causal effect estimation; \cite{dukes2023proximal,ghassami2021proximal} that studied proximal mediation analysis; and \cite{liu2023causal,miao2018identifying,miao2022identifying} that leveraged the proxy variable for causal discovery. Particularly, the recent hypothesis testing-based methods \cite{miao2018identifying,miao2022identifying} introduced various testing procedures to examine the null hypothesis of no causal relationship, using the proxy variable. However, their procedures were either limited to the discrete case or relied on strong parametric assumptions.

In this paper, we propose a novel hypothesis-testing procedure that can effectively identify the causal relationship between two continuous variables, without any parametric assumption. Our strategy is to find a proper discretization procedure such that, under causal null hypothesis, the probability matrices over discretized variables satisfies a linear equation whose coefficient vector is identifiable. For this purpose, we first introduce a discretization procedure that, under the completeness assumption, makes the probability matrix over discrete variables satisfy rank regularities that are crucial for the identifiability of the coefficient vector. We proceed to analyze the errors in the linear equation after discretization and show that they can be controlled to arbitrarily small, given that the bin numbers for discretization is sufficiently large. Based on the above analyses, we introduce our testing statistic based on the residue of linear regression, and establish the asymptotic level and power of our test. We demonstrate the validity and effectiveness of our procedure on both synthetic and real-world data. 




% Our strategy here is to first discretize the variables, and then connect the null hypothesis of no causal relationship to the identification problem of a system of linear equations. We show that, given proper discretization, the linear system we establish is identifiable and hence the null hypothesis is testable. 




% meet the rank regularities in the 





We summarize our contributions as follows:
\begin{enumerate}[noitemsep,topsep=1pt]
    \item We propose a proximal hypothesis testing based on discretization for bivariate causal discovery over continuous variables.
    \item We establish the asymptotic level and power of our procedure without any parametric assumptions. 
    \item We demonstrate the validity of our procedure on both synthetic and real-world datasets.
\end{enumerate}


==> icml24_para/method_v2.tex <==
\clearpage
\section{Methodology}

In this section, we introduce a hypothesis-testing procedure based on discretization. At the core of our procedure lies finding discretization processes that establish the identifiability of Equation (\ref{eq.miao}). 

To achieve this goal, in Section~\ref{sec.comp}, we first introduce a discretization process which, under the completeness assumption, can ensure the discretized $\tilde{X},\tilde{W}$ meet the rank regularities. Then, in Section~\ref{sec.dis-error}, we analyze the errors induced during the discretization. Under smoothness conditions regarding structural equations, we show that they can be effectively controlled to be arbitrarily small if the bin number is sufficiently large. Finally, based on the above analyses, we introduce our testing statistic and discuss the asymptotic level and power of the test in Section~\ref{sec.hypo-test}.

\subsection{Discretization process}
\label{sec.comp}

In this section, we introduce a discretization process to establish the identifiability of Equation (\ref{eq.miao}). As mentioned before, this involves finding discretization for $W$ and $X$ such that the induce $P(\tilde{W}|\tilde{X})$ has full row rank. To ensure such a discretization exists, we need the following completeness assumption.

\begin{assumption}[Completeness]
    We assume the conditional distributions $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|X}$ are complete. That is, for any bounded function $g$, we assume
    \begin{align*}
        E[g(u)|x]=0 \,\, &\text{almost surely iff} \,\, g(u)=0 \,\, \text{almost surely} \\
        E[g(w)|x]=0 \,\, &\text{almost surely iff} \,\, g(w)=0 \,\, \text{almost surely}
    \end{align*}
    \label{asm.comp}
\end{assumption}
\vspace{-.5cm}


To understand the role of Assumption~\ref{asm.comp} in our method, note that for discrete variables, the completeness of $\mathcal{L}_{W|X}$ means the conditional probability matrix $P(W|X)$ has full row rank. Therefore, by assuming the completeness of $\mathcal{L}_{W|X}$, we can ensure the existence of discretization for $W$ and $X$, such that the induced $P(\tilde{W}|\tilde{X})$ has full row rank, as required by the procedure of \cite{miao2018identifying}. Moreover, when combined with the completeness of $\mathcal{L}_{U|X}$, we can demonstrate the existence of discretization for $U$ such that the matrix $P(\tilde{W}|\tilde{U})$ is invertible, which constitutes another important component for the identifiability of Equation (\ref{eq.miao}).

The following example shows that Assumption~\ref{asm.comp} is mild and can be satisfied by a wide range of Addictive Noise Models (ANMs).

\begin{example}[ANM with completeness]
    Suppose that $X,U,W$ satisfy the ANM, i.e., $X=g_X(U)+N_X, W=g_W(U)+N_W$, with $N_X,N_W$ being the noises. If $g_X$ is invertible with a non-zero derivative, and $N_X$, $N_W$ have non-zero characterization functions, then the conditional distributions $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|X}$ are both complete.
\end{example}

\begin{remark}
    We also provide an example in which $U$ is a mediator and Assumption~\ref{asm.comp} is satisfied. Please refer to Appendix~\ref{app-sec.example-comp} for details.
\end{remark}

The completeness condition has been similarly assumed by other causal discovery and inference methods. For example, the completeness of $\mathcal{L}_{U|X}$ was assumed by \cite{miao2018identifying,miao2022identifying}\footnote{See Condition~(ii) of \cite{miao2018identifying} and Assumption~3 of \cite{miao2022identifying}, respectively.}, and a discrete version of the completeness of $\mathcal{L}_{W|X}$, i.e., $P(W|X)$ has full row rank, was required by the procedure described by \cite{miao2018identifying}\footnote{See Condition~(iv) of \cite{miao2018identifying}.}. Indeed, in \cite{miao2018identifying}, they also assumed the completeness of $\mathcal{L}_{X|W}$. To see the difference, note that this assumption is required specifically for estimating the causal effect, which is not considered in this paper.

\begin{remark}
    On the other side, note that the bounded completeness we assume is strictly weaker that the $L^2$ completeness required by \cite{miao2018identifying,miao2022identifying}.
\end{remark}


Equipped with Assumption~\ref{asm.comp}, we have the following proposition, which states that for \emph{any} discretization of $W$, there exists discretization of $X$ and $U$ (with $l_{\tilde{X}}>l_{\tilde{W}}=l_{\tilde{U}}$) such that the matrix $P(\tilde{W}|\tilde{X})$ has full row rank and the matrix $P(\tilde{W}|\tilde{U})$ is invertible.

\begin{proposition}
    Suppose Assumption~\ref{asm.comp} holds. Then, for any discretization $\tilde{W}$ of $W$, there exists a discretization $\tilde{X}$ of $X$ such that the matrix $P(\tilde{W}|\tilde{X})$ has full row rank. Similarly, there also exists a discretization $\tilde{U}$ of $U$ such that the matrix $P(\tilde{W}|\tilde{U})$ is invertible.
    \label{prop.rank-dis}
\end{proposition}

Proposition~\ref{prop.rank-dis} shows that for any discretization $\tilde{W}$ of $W$, there exists a discretization $\tilde{X}$ of $X$ such that $P(\tilde{W}|\tilde{X})$ has full row rank. To practically find such a discretization, we introduce the following Algorithm~\ref{alg.dis}.

Before introducing the algorithm, we first introduce some additional notation convenience. In Algorithm~\ref{alg.dis}, $F(x|\tilde{w})$ is the conditional cdf of $x$ given $\tilde{W}=\tilde{w}$ and $F(x|\tilde{w}_{[i]}):=[F(x|\tilde{w}_1),...,F(x|\tilde{w}_i)]^T$ is the vector consists of $i$ conditional cdfs. For $\boldsymbol{x}_{[i]}:=[x_1,...,x_i]^T$, $F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]}):=[F(x_1|\tilde{w}_{[i]}),...,F(x_i|\tilde{w}_{[i]})]$ is the matrix consist of values of conditional cdfs.

We now introduce the idea of Algorithm~\ref{alg.dis}. Specifically, in line 1, we first discretize $W$ with $l_{\tilde{W}}$ uniform bins to obtain $\tilde{W}$, since according to Proposition~\ref{prop.rank-dis}, the discretization of $W$ can be arbitrarily chosen. Then, in lines 2-7, we find the same number of bins for $X$ to obtain a $\tilde{X}^\prime$ such that $P(\tilde{W}|\tilde{X}^\prime)$ is invertible, which can be achieved by requiring $P(\tilde{X}^\prime|\tilde{W})$ to be invertible. To this end, we iteratively search for separating points $x_i$ of $\mathcal{X}$ and thereby define the bins to be $\{[x_i,x_{i+1}]\}$ for $i=1,...,l_{\tilde{W}}$. 

During each step of the search, we find a new point $x_i$ such that the determinant of $P(\tilde{X}_{[i]}|\tilde{W}_{[i]})$ is non-zero, which can be achieved by requiring the determinant of the conditional cdf matrix $F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]})$ to be non-zero. We show that such a point always exists, and hence can be found by exhaustive searching. To see this, note that the determinant of
$F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]})$ can be expanded into a weighted sum of the functions in $F(x|\tilde{w}_{[i]})$, and that under Assumption~\ref{asm.comp}, these functions are linear independent. Since the previous step of the search ensures that at least one of the weighting factors, i.e., $\mathrm{det}(F(\boldsymbol{x}_{[i-1]}|\tilde{w}_{[i]\backslash j}))$, is non-zero, there exists a point $x_i$ such that the weighted sum of these linear independent functions is non-zero, and hence $\mathrm{det}(F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]}))\neq 0$.

Finally, after obtaining the $\tilde{X}^\prime$ such that $P(\tilde{W}|\tilde{X}^\prime)$ is invertible, we add another $(l_{\tilde{X}}-l_{\tilde{W}})$ levels to $\tilde{X}^\prime$ to obtain $\tilde{X}$ in lines 8-11. In this regard, the obtained $P(\tilde{W}|\tilde{X})$ can have full row rank.


\begin{algorithm}[t]
   \caption{Rank preserving discretization}
   \label{alg.dis}
\begin{flushleft}
\textbf{Input:} Continuous variables $X$, $W$; Bin numbers $l_{\tilde{X}}$, $l_{\tilde{W}}$. \\
\textbf{Output:} Discrete variables $\tilde{X}$, $\tilde{W}$ satisfying $P(\tilde{W}|\tilde{X})$ has full row rank.
\end{flushleft}
\begin{algorithmic}[1]
    \STATE Discretize $W$ with $l_{\tilde{W}}$ uniform bins to obtain $\tilde{W}$.
    \FOR{$i=1:l_{\tilde{W}}$}
        \FOR{$j=1:i$}
            \STATE Estimate $d_j=\mathrm{det}(F(x_{[i-1]}|\tilde{w}_{[i]\backslash j}))$
        \ENDFOR
        \STATE Search for $x_i$ s.t. $\sum_{j=1}^i (-1)^{1+j} d_j F(x_i|\tilde{w}_j) \neq 0$.
    \ENDFOR
    \FOR{$i=l_{\tilde{W}}+1:l_{\tilde{X}}$}
        \STATE Set $[x_i,x_{i+1}]$ to the $i$-th uniform bin of $\mathcal{X}\backslash [x_1,x_{l_{\tilde{W}}}]$.
    \ENDFOR
    \STATE Discretize $X$ with $\{[x_i,x_{i+1}]\}_{i=1}^{l_{\tilde{X}}}$ to obtain $\tilde{X}$.
    
    \STATE \textbf{return} $\tilde{X}$, $\tilde{W}$.
\end{algorithmic}
\end{algorithm}

\begin{discussion}[Choice of the bin number]
    In practice, the choice of the bin number for discretization is a trade-off between the discretization error (which will be detailed in Section~\ref{sec.dis-error}) and the estimation error of discrete probabilities. For large bin numbers, the discretization error can be effectively controlled, whereas the estimation of probabilities may be inaccurate due to insufficient samples in each bin. To balance the trade-off, we adopt the heuristics suggested by \cite{dougherty1995supervised} and set the bin number in reference to $\left \lfloor \log(n) \right \rfloor$, where $n$ is the sample size.
\end{discussion}

\begin{remark}
    Note that we do not need to explicitly discretize $U$, which is infeasible due to the unobserveness of $U$. Instead, we establish the invertibility of $P(\tilde{W}|\tilde{U})$ by an implicit binning of $U$ given the discretization $\tilde{W}$ of $W$. The existence of such implicit binning has been shown by Proposition~\ref{prop.rank-dis}.
\end{remark}


\subsection{Discretization error analysis}
\label{sec.dis-error}



\clearpage
\subsection{Hypothesis test}
\label{sec.hypo-test}

In this section, we present our hypothesis testing procedure. Specifically, we adopt the test statistic proposed by \cite{miao2018identifying} and analyze its asymptotic distribution under the null hypothesis. Additional, we investigate the behavior of the statistic under the alternative hypothesis and establish the asymptotic power of our test.

We first introduce our test statistic. The idea is that we can assess whether $\mathbb{H}_0$ is correct by looking at the residual of the least-square solution of Equation~(\ref{eq.miao}). If $\mathbb{H}_0$ is correct, then Equation~(\ref{eq.miao}) is identifiable, hence the least-square residual should be close to zero. In practice, to enhance the capacity of the statistic, we can aggregate the residuals obtained from the solutions of Equation~(\ref{eq.miao}) with respect to all levels of $\tilde{Y}$. Specifically, we let
\begin{equation*}
    q:=[P(\tilde{y}_1|\tilde{X}),...,P(\tilde{y}_{l_{\tilde{Y}}-1}|\tilde{X})]^T
\end{equation*}
be the column vector that aggregates $P(\tilde{y}|\tilde{X})$ for all (free) levels of $\tilde{Y}$, and let
\begin{equation*}
    Q:=\mathrm{diag}[P(\tilde{W}|\tilde{X}),...,P(\tilde{W}|\tilde{X})]
\end{equation*}
be the block diagonal matrix with $(l_{\tilde{Y}}-1)$ repeating blocks of $P(\tilde{W}|\tilde{X})$ in the diagonal. Consider corresponding estimators $\hat{q}$ and $\hat{Q}$ satisfy that
\begin{align*}
    n^{1/2}(\hat{q} - q) &\to N(0,\Sigma) \,\, \text{in distribution}, \\
    \hat{Q}\to Q, \hat{\Sigma} &\to \Sigma \,\, \text{in probability,} 
\end{align*}
with $\hat{\Sigma}, \Sigma$ both positive definite\footnote{We adopt maximum likelihood estimation to obtain $\hat{q}$, $\hat{Q}$, and $\hat{\Sigma}$. Please refer to Appendix~\ref{app-sec.mle} for details.}. Then, we have the least-square residual of regressing $\hat{\Sigma}^{-1/2} \hat{q}$ on $\hat{\Sigma}^{-1/2} \hat{Q}$ to be
\begin{equation*}
    \xi := \{I - \hat{\Sigma}^{-1/2} \hat{Q}^T (\hat{Q} \hat{\Sigma}^{-1} \hat{Q}^T)^{-1} \hat{Q} \hat{\Sigma}^{-1/2}\} \hat{\Sigma}^{-1/2} \hat{q}.
\end{equation*}
Following \cite{miao2018identifying}, we adopt the squared residual $T:=n\xi^T \xi$ as our test statistic. 

We then analyze the asymptotic distribution of $T$ under $\mathbb{H}_0$. Specifically, we show that $T$ asymptotically follows a chi-squared distribution $\chi^2_k$, where the degrees of freedom $k=(l_{\tilde{X}}-l_{\tilde{W}})(l_{\tilde{Y}}-1)$ is determined by the additional levels that $\tilde{X}$ has beyond $\tilde{W}$, multiplied by the level of $\tilde{Y}$. Formally, denote $l$ in short for $(l_{\tilde{X}},l_{\tilde{Y}},l_{\tilde{W}})$ and denote $z_{1-\alpha}$ as the $(1-\alpha)$-th quantile of $\chi^2_k$, we then have the following result:


\begin{theorem}
    Suppose that Assumptions~\ref{asm.comp}-\ref{asm.tv-smooth} hold, then under $H_0$, it holds that:
    \begin{equation*}
        T_{n,l} \to \chi_{k}^2 \,\, \text{in distribution}
    \end{equation*}
    as $n,l\to \infty$. As a result, for any $\alpha\in (0,1)$, we have:
    \begin{equation*}
        \lim_{n,l\to \infty} \mathbb{P}(T_{n,l}> z_{1-\alpha}) = \alpha.
    \end{equation*}
    In other words, the testing procedure we define has uniform asymptotic level $\alpha$.
\label{thm.control.type-i}
\end{theorem}

In general, we cannot expect that the test has power against alternatives to $\mathbb{H}_0$ without further restrictions on the alternative distribution. This is analogous to other conditional independence tests \cite{zhang2012kernel,runge2018conditional,christgau2023nonparametric} used for causal discovery. Therefore, to establish the power of our test, we put the following restriction on the alternative distribution:

\begin{assumption}
    We consider the local alternative $\mathbb{H}_1:\Theta$, where for each $\theta\in \Theta$, the integral equation
    \begin{equation}
        f_{\theta}(y|x)=\int h(y,w)f_{\theta}(w|x)dw
    \label{eq.int-eq}
    \end{equation}
    has no solution.
    \label{asm.int-eq}
\end{assumption}

\begin{remark}
    We show that $\mathbb{H}_1$ is indeed a local alternative, that is, there exists distributions satisfying $X\not\ind Y|U$ but do not belong to $\Theta$. Please refer to Appendix~\ref{app-sec.int-eq} for details.
\end{remark}

To understand the role of Assumption~\ref{asm.int-eq}, note that to establish the power, it is important for the statistic $T$ to deviate from zero under the alternative model, which requires that the Equation~(\ref{eq.miao}) has no solution. Intuitively, this means the variability of $P(\tilde{y}|\tilde{X})$ can not be fully explained by that of $P(\tilde{W}|\tilde{X})$. For continuous variables, this then corresponds to the condition that the integral equation~(\ref{eq.int-eq}) has no solution.

In an empirical way, we can show that $\mathbb{H}_1$ covers many cases where the casual influence from $X$ to $Y$ is strong. Please refer to Appendix~\ref{app-sec.int-eq} for details.

Equipped with the above analyses, we now establish power against the local alternative $\mathbb{H}_1$ as follows:

\begin{theorem}
    Suppose that Assumptions~\ref{asm.comp}-\ref{asm.tv-smooth} holds, then for any $\alpha\in (0,1)$, it holds that:
    \begin{equation*}
        \lim_{n,l\to\infty}\mathbb{P}_{\Theta}(T_{n,l}>z_{1-\alpha})=1.
    \end{equation*}
    In other words, the limiting power of our test is one.
    \label{thm.type-ii}
\end{theorem}


% The integral equation:
% \begin{equation}
%     f(y|x)=\int h(y,w)f(w|x)dw
%     \label{eq.int-eq}
% \end{equation}

% Denote $\mathbb{C}(\mathcal{W},\mathcal{Y})$ the set of almost surely continuous functions over $\mathcal{W}\times \mathcal{Y}$. 

% Under the model $\theta$,  let $\mathrm{res}_\theta(h):=\iint |f_\theta(y|x)-\int h(y,w)f_\theta(w|x)dw|dy f_\theta(x) dx$ be the averaged residual of fitting the function $h$ to Equation~(\ref{eq.int-eq}). 

% Let $\Theta:=\{\theta: \exists\epsilon_0>0, \min_{h\in \mathbb{C}(\mathcal{W},\mathcal{Y})} \mathrm{res}_\theta(h)>\epsilon_0\}$ be the set of alternative models in which Equation~(\ref{eq.int-eq}) has no smooth solution.




==> icml24_para/method_v2_xw.tex <==
\section{Methodology}

In this section, we introduce a hypothesis-testing procedure based on discretization. At the core of our procedure lies finding discretization processes that establish the identifiability of Equation (\ref{eq.miao}). 

To achieve this goal, in Section~\ref{sec.comp}, we first introduce a discretization process which, under the completeness assumption, can ensure the discretized $\tilde{X},\tilde{W}$ meet the rank regularities. Then, in Section~\ref{sec.dis-error}, we analyze the errors induced during the discretization. Under smoothness conditions regarding structural equations, we show that they can be effectively controlled to be arbitrarily small if the bin number is sufficiently large. Finally, based on the above analyses, we introduce our testing statistic and discuss the asymptotic level and power of the test in Section~\ref{sec.hypo-test}.

\subsection{Discretization under Completeness}
\label{sec.comp}

In this section, we introduce a discretization process to establish the identifiability of Eq.~\eqref{eq.miao}. As mentioned previously, this involves finding discretization for $W$ and $X$ such that the induce $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank. We first introduce the following completeness conditions that have been similarly adopted for continuous variables in causal inference \cite{miao2018identifying, miao2022identifying}, which ensures the existence of such a discretization. 

%To ensure such a discretization exists, we introduce the following completeness assumption.
\begin{assumption}[Completeness]
    We assume the conditional distributions $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|X}$ are complete. That is, for any bounded function $g$, we assume
    \begin{align*}
        \mathbb{E}[g(u)|x]=0 \,\, &\text{almost surely iff} \,\, g(u)=0 \,\, \text{almost surely}, \\
        \mathbb{E}[g(w)|x]=0 \,\, &\text{almost surely iff} \,\, g(w)=0 \,\, \text{almost surely}
    \end{align*}
    \label{asm.comp-main}
\end{assumption}
\vspace{-.5cm}
To understand the role of assump.~\ref{asm.comp-main} in our method, note that in the case when $W$ (\emph{resp.} $U$) is discrete, the completeness of $\mathcal{L}_{W|X}$ (\emph{resp.} $\mathcal{L}_{U|X}$) means the conditional probability matrix $\mathbb{P}(W|X)$ has full row rank, as required in the procedure for discrete variables \cite{miao2018identifying}. As will be shown later, this condition enables us to find a discretization such that $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank. Further, when combined with the completeness of $\mathcal{L}_{U|X}$, we can demonstrate the existence of discretization for $U$ such that the matrix $\mathbb{P}(\tilde{W}|\tilde{U})$ is invertible, which is also required for the identifiability of Eq.~\eqref{eq.miao}.

The following example shows that assump.~\ref{asm.comp-main} can hold for a wide range of Addictive Noise Models (ANMs).

\begin{example}[ANM with completeness]
    Suppose that $X,U,W$ satisfy the ANM, i.e., $X=g_X(U)+N_X, W=g_W(U)+N_W$, with $N_X,N_W$ being the noises. If $g_X$ is invertible with a non-zero derivative, and $N_X$, $N_W$ have non-zero characterization functions, then the conditional distributions $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|X}$ are both complete.
\end{example}

\begin{remark}
    We also provide an example in which $U$ is a mediator and assump.~\ref{asm.comp-main} is satisfied. Please refer to Appx.~\ref{app-sec.example-comp} for details.
\end{remark}

The completeness condition has been similarly assumed in causal hypothesis testing and causal inference, with the difference that our condition is not restricted to square-integrable functions. Specifically, the completeness of $\mathcal{L}_{U|X}$ was assumed by \cite{miao2018identifying,miao2022identifying}\footnote{See Condition~(ii) in \cite{miao2018identifying} (by dropping $Z$) and assump.~3 in \cite{miao2022identifying}.}. Besides, a discrete version of the completeness of $\mathcal{L}_{W|X}$, \emph{i.e.}, $\mathbb{P}(W|X)$ has full row rank, was required by the procedure described by \cite{miao2018identifying}. Indeed, in \cite{miao2018identifying}, they also assumed the completeness of $\mathcal{L}_{X|W}$\footnote{See Condition~(iii), where $z$ is replaced with $x$ to induce variation for identification.}. However, this assumption is to ensure the solution's existence in the integral function for identifying the causal effect, which therefore is not required in this paper.

% To see the difference, note that this assumption is required specifically for estimating the causal effect, which is not considered in this paper.

%\begin{remark}
%    On the other side, note that the bounded completeness we assume is strictly weaker than the $L^2$ completeness required by \cite{miao2018identifying,miao2022identifying}.
%\end{remark}


Next, we show that, under assump.~\ref{asm.comp-main}, we can find a discretization procedure such that the $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank and the matrix $\mathbb{P}(\tilde{W}|\tilde{U})$ is invertible.

\begin{proposition}
    Suppose assump.~\ref{asm.comp-main} holds. Then, for any discretization $\tilde{W}$ of $W$, there exists a discretization $\tilde{X}$ of $X$ such that the matrix $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank. Similarly, there also exists a discretization $\tilde{U}$ of $U$ such that the matrix $\mathbb{P}(\tilde{W}|\tilde{U})$ is invertible.
    \label{prop.rank-dis-main}
\end{proposition}

\begin{remark}
    We leave the proof to Appx.~\ref{app-sec.discrete}. Roughly speaking, we first show that given $\{\mathcal{W}_i\}_{i=1}^{l_W}$, the functions $F(x|\tilde{w}_1),...,F(x|\tilde{w}_{l_W})$ are linear independent under the completeness condition of $\mathcal{L}_{W|X}$. Then we prove with induction that there exists $\tilde{x}_1,...,\tilde{x}_{l_X}$ with $l_X > l_W$, such that $\left[F(\boldsymbol{x}|\tilde{w}_1),...,F(\boldsymbol{x}|\tilde{w}_{l_W})\right]$ is linear independent, where $F(\boldsymbol{x}|\tilde{w}_i) = \left[ F(\tilde{x}_1|\tilde{w}_i),...,F(\tilde{x}_{l_X}|\tilde{w}_i)\right]^\top$. 
\end{remark}

%Prop.~\ref{prop.rank-dis-main} shows that for any discretization $\tilde{W}$ of $W$, there exists a discretization $\tilde{X}$ of $X$ such that $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank. To practically find such a discretization, we introduce the following Alg.~\ref{alg.dis}. Before introducing the algorithm, we first introduce some additional notation convenience. In Alg.~\ref{alg.dis}, 

Inspired by Prop.~\ref{prop.rank-dis-main}, we introduce our discritization procedure in Alg.~\ref{alg.dis}. The algorithm mainly contains three steps. First, in line 1, we uniformly discretize $W$ into $l_{\tilde{W}}$ bins to obtain $\tilde{W}$. Indeed, the choice of discretization for $W$ is arbitrary, as indicated by Prop.~\ref{prop.rank-dis-main}. Next, in lines 2-7, we discretize $X$ to construct $\tilde{X}^\prime$ that contains the same number of bins as $W$, such that $\mathbb{P}(\tilde{X}^\prime|\tilde{W})$ and therefore $\mathbb{P}(\tilde{W}|\tilde{X}^\prime)$ is invertible. Finally, we add another $(l_{\tilde{X}}-l_{\tilde{W}})$ levels to $\tilde{X}^\prime$ to obtain $\tilde{X}$ in lines 8-11. In this regard, the obtained $\mathbb{P}(\tilde{W}|\tilde{X})$ can have full row rank.

% We now introduce the idea of Alg.~\ref{alg.dis}. Specifically, in line 1, we first discretize $W$ with $l_{\tilde{W}}$ uniform bins to obtain $\tilde{W}$, since according to Prop.~\ref{prop.rank-dis-main}, the discretization of $W$ can be arbitrarily chosen. 

% To this end, we iteratively search for separating points $x_i$ of $\mathcal{X}$ and thereby define the bins to be $\{[x_i,x_{i+1}]\}$ for $i=1,...,l_{\tilde{W}}$. To this end, we iteratively search for separating points $x_i$ of $\mathcal{X}$ and thereby define the bins to be $\{[x_i,x_{i+1}]\}$ for $i=1,...,l_{\tilde{W}}$. 

In the second step (lines 2-7), we iteratively search for $x_i$ such that the matrix $M_i:=F(\boldsymbol{x}_{[i]}|\boldsymbol{w}_{[i]})$ is invertible given $x_1,...,x_{i-1}$. This can be achieved by noting that the functions $F(x|\tilde{w}_1),...,F(x|\tilde{w}_{l_W})$ are linear independent under the completeness condition. Once we have the invertibility of $M_i$, we have $\mathbb{P}(\tilde{X}|\tilde{W}):=\{\mathbb{P}(\tilde{x}_i|\tilde{w}_j)\}_{i,j}$ is invertible, with $\mathbb{P}(\tilde{x}_i|\tilde{w}_j):= F(x_i|W \in \mathcal{W}_j)-F(x_{i-1}|W \in \mathcal{W}_j)$ and $\mathcal{X}_i:=[x_{i-1},x_i)$ $\left( (-\infty,x_1) \text{ for $i=1$}\right)$. To find such an $x_i$, note that $\mathrm{det}(M_i)$ can be expanded as:
\begin{align*}
    \mathrm{det}(M_i)(x_i) = \sum_{j=1}^i (-1)^{1+j} d_j F(x_i|\tilde{w}_j),
\end{align*}
where $d_j:=\mathrm{det}(F(x_{[i-1]}|\tilde{w}_{[i]\backslash j}))$. By induction, there exists an $i-1$ dimensional minor among $\{d_j\}$ is non-zero. Since $F(x|\tilde{w}_{[i]})$ are linear independent, there exists $x_i$ such that $\mathrm{det}_{M_i}(x_i) \neq 0$, which means $F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]})$ is invertible. 

% we find a new point $x_i$ such that the determinant of $\mathbb{P}(\tilde{X}_{[i]}|\tilde{W}_{[i]})$ is non-zero, which can be achieved by requiring the determinant of the conditional cdf matrix $F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]})$ to be non-zero. 

%We show that such a point always exists, and hence can be found by exhaustive searching. To see this, note that the determinant of
%$F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]})$ can be expanded into a weighted sum of the functions in $F(x|\tilde{w}_{[i]})$, and that under assump.~\ref{asm.comp-main}, these functions are linear independent. Since the previous step of the search ensures that at least one of the weighting factors, i.e., $\mathrm{det}(F(\boldsymbol{x}_{[i-1]}|\tilde{w}_{[i]\backslash j}))$, is non-zero, there exists a point $x_i$ such that the weighted sum of these linear independent functions is non-zero, and hence $\mathrm{det}(F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]}))\neq 0$.




\begin{algorithm}[t]
   \caption{Rank preserving discretization}
   \label{alg.dis}
\begin{flushleft}
\textbf{Input:} Continuous variables $X$, $W$; Bin numbers $l_{\tilde{X}}> l_{\tilde{W}}$. \\
\textbf{Output:} Discrete variables $\tilde{X}$, $\tilde{W}$ satisfying $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank.
\end{flushleft}
\begin{algorithmic}[1]
    \STATE Discretize $W$ with $l_{\tilde{W}}$ uniform bins to obtain $\tilde{W}$.
    \FOR{$i=1:l_{\tilde{W}}$}
        \FOR{$j=1:i$}
            \STATE Estimate $d_j=\mathrm{det}(F(x_{[i-1]}|\tilde{w}_{[i]\backslash j}))$
        \ENDFOR
        \STATE Search for $x_i$ s.t. $\sum_{j=1}^i (-1)^{1+j} d_j F(x_i|\tilde{w}_j) \neq 0$.
    \ENDFOR
    \FOR{$i=l_{\tilde{W}}+1:l_{\tilde{X}}$}
        \STATE Set $[x_i,x_{i+1}]$ to the $i$-th uniform bin of $\mathcal{X}\backslash [x_1,x_{l_{\tilde{W}}}]$.
    \ENDFOR
    \STATE Discretize $X$ with $\{[x_i,x_{i+1}]\}_{i=1}^{l_{\tilde{X}}}$ to obtain $\tilde{X}$.
    \STATE \textbf{return} $\tilde{X}$, $\tilde{W}$.
\end{algorithmic}
\end{algorithm}

\textbf{Choosing the bin number.}
    The bin number is a trade-off between the discretization error and the estimation of discrete probabilities. While a larger bin number effectively controls discretization error, it may lead to inaccurate probability estimation due to insufficient samples in each bin. To balance this trade-off, we follow the heuristics proposed by \cite{dougherty1995supervised} and set the bin number to $\left \lfloor \log(n) \right \rfloor$.
    %In practice, the choice of the bin number for discretization is a trade-off between the discretization error (which will be detailed in Section~\ref{sec.dis-error}) and the estimation error of discrete probabilities. For large bin numbers, the discretization error can be effectively controlled, whereas the estimation of probabilities may be inaccurate due to insufficient samples in each bin. To balance the trade-off, we adopt the heuristics suggested by \cite{dougherty1995supervised} and set the bin number in reference to $\left \lfloor \log(n) \right \rfloor$, where $n$ is the sample size.
    
\begin{remark}
    Since $U$ is unobserved, we cannot discretize $U$. However, according to Prop.~\ref{prop.rank-dis-main}, there exists a $\tilde{U}$ such that $\mathbb{P}(\tilde{W}|\tilde{U})$ is invertible. 
    %Note that we do not need to explicitly discretize $U$, which is infeasible due to the unobserveness of $U$. Instead, we establish the invertibility of $\mathbb{P}(\tilde{W}|\tilde{U})$ by an implicit binning of $U$ given the discretization $\tilde{W}$ of $W$. The existence of such implicit binning has been shown by.
\end{remark}


\subsection{Discretization error analysis}
\label{sec.dis-error}

In this section, we discuss the control of discretization error. Our goal is to maintain the conditional independence $X\ind Y|U$ and $X\ind W|U$ during the discretization, and hence establish Eq.~(\ref{eq.miao}) over the discretized variables. Take the structure $X\ind Y|U$ as an example, for continuous variables, we have $p(y|u)=p(y|x,u)$, which enables us to have Eq.~(\ref{eq.miao}). For discretized variables, we hope to control the distance $|p(\tilde{y}|\tilde{u})-p(\tilde{y}|\tilde{x},\tilde{u})|$, so that Eq.~(\ref{eq.miao}) still holds under some small, tractable error.

For this purpose, we first introduce the following Total Variation (TV) smoothness condition, which states that the conditional distributions $\mathcal{L}_{Y|U=u}$ and $\mathcal{L}_{W|U=u}$ should change smoothly with respect to $u$.


\begin{assumption}[TV smoothness]
    We assume the maps $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are Lipschitz continuous with respect to TV distance. That is, for any $u,u^\prime \in \mathcal{U}$, we assume there exist $L_Y$ and $L_W$, respectively, such that:
    \begin{align*}
        \mathrm{TV}(\mathcal{L}_{Y|U=u},&\mathcal{L}_{Y|U=u^\prime}) \leq L_Y |u-u^\prime|, \\
        \mathrm{TV}(\mathcal{L}_{W|U=u},&\mathcal{L}_{W|U=u^\prime}) \leq L_W |u-u^\prime|.
    \end{align*}
    \label{asm.tv-smooth}
\end{assumption}

\begin{remark}
    To be precise, what is meant here is that given \emph{regular conditional distributions} $\mathcal{L}_{Y|U=u}$ and $\mathcal{L}_{W|U=u}$, one can modify them on two sets of measure zero, respectively, so that the Lipschitz condition is satisfied. Please refer to Appx.~\ref{sec.regular-prob} for details.
\end{remark}


To understand the role of Asm.~\ref{asm.tv-smooth} in discretization error control, note that for a small bin $\mathcal{U}_i$ of $\mathcal{U}$ and any $u\in\mathcal{U}_i$, Asm.~\ref{asm.tv-smooth} means that the distance
\begin{equation*}
    \mathrm{TV}(\mathcal{L}_{Y|U\in \mathcal{U}_i},\mathcal{L}_{Y|U=u})
\end{equation*}
is small. In a similar way, it also indicates that the distance
\begin{equation*}
    \mathrm{TV}(\mathcal{L}_{Y|X\in\mathcal{X}_j,U\in \mathcal{U}_i},\mathcal{L}_{Y|X\in\mathcal{X}_j,U=u})
\end{equation*}
can be controlled. Since we have $\mathcal{L}_{Y|U=u}=\mathcal{L}_{Y|X\in\mathcal{X}_j,U=u}$ under $X\ind Y|U$. Using the triangle inequity, we can control the distance $\mathrm{TV}(\mathcal{L}_{Y|U\in \mathcal{U}_i},\mathcal{L}_{Y|X\in\mathcal{X}_j,U\in \mathcal{U}_i})$, and hence control the error $|p(\tilde{y}|\tilde{u})-p(\tilde{y}|\tilde{x},\tilde{u})|$.

The following example shows that Asm.~\ref{asm.tv-smooth} can hold for a wide range of ANM models.


\begin{example}[ANM with TV smoothness]
    Suppose that $Y,U,W$ satisfy the ANM, i.e., $Y=g_Y(U)+N_Y, W=g_W(U)+N_W$, with $N_Y, N_W$ being the noises. If $g_Y$ and $g_W$ are differentiable, and the probability densities of $N_Y$ and $N_W$ have absolutely integrable derivatives, then the maps $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are Lipschitz continuous with respect to TV distance.
\end{example}

\begin{remark}
    We also provide an example in which $U$ is a mediator and Asm.~\ref{asm.tv-smooth} is satisfied. Please refer to Appx.~\ref{app-sec.tv-example} for details.
\end{remark}

Equipped with Asm.~\ref{asm.tv-smooth}, we now introduce the following proposition:

\begin{proposition}
    Assuming Asm.~\ref{asm.tv-smooth}. Suppose that $\{\mathcal{U}_i\}_{l_{U}}$ is a partition of $\mathcal{U}$, and that for every bin $\mathcal{U}_i$,
    \begin{equation*}
        len(\mathcal{U}_i)\leq \frac{1}{2}min\{\epsilon/L_Y,\epsilon/L_W\}.
    \end{equation*}
    Then, under $\mathbb{H}_0:X\ind Y|U$, we have:
    \begin{equation*}
        |p(\tilde{y}|\tilde{u}_i) - p(\tilde{y}|\tilde{x},\tilde{u}_i)| \leq \epsilon, \,\, |p(\tilde{w}|\tilde{u}_i) - p(\tilde{w}|\tilde{x},\tilde{u}_i)| \leq \epsilon.
    \end{equation*}
\label{prop.control-err}
\end{proposition}

According to Prop.~\ref{prop.control-err}, when $\mathcal{U}$ is a compact interval, we can (implicitly) partition $\mathcal{U}$ into sufficiently refined bins. As long as the lengths of these bins are small, the discretization error can be controlled.

For non-compact domains such as $\mathbb{R}$, it is not possible to partition the infinity ends into finite, small bins. Therefore, extra errors can be induced. To  control these errors, we further require the distribution of $\mathcal{L}_{U|X}$ to be tight, meaning that for large values of $u$'s, the conditional probability $p(u|x)$ is close to zero. To this end, we first give the definition of a tight distribution:

\begin{definition}[Tight distribution] The marginal distribution $\mathcal{L}_U$ is said to be tight if $\forall \epsilon>0, \exists T, \forall t\geq T,\mathcal{L}(|U|\geq t)\leq \epsilon$. The conditional distribution $\mathcal{L}_{U|X}$ is said to be uniformly tight in $[a,b]$ if $\forall \epsilon>0, \exists T, \forall t\geq T, \forall x\in [a,b],\mathcal{L}(|U|\geq t|x)\leq \epsilon$.
\label{def.tight}
\end{definition}

\begin{remark}
    We use the term ``uniform'' because the $T$ holds uniformly for all $x\in[a,b]$. As we will show later, the uniform tightness is a mild condition (though one can imagine that uniform tightness for all $x\in \mathbb{R}$ is a strong one).
\end{remark}

We then assume the following tightness condition:

\begin{assumption}
    We assume the conditional distribution $\mathcal{L}_{U|X}$ is uniformly tight for any compact interval $[a,b]$.
    \label{asm.tight}
\end{assumption}

To see the role of Asm.~\ref{asm.tight} in discretization error control under non-compact domains, note that we can divide $\mathcal{U}$ into a compact part $\mathcal{U}_c$ and a non-compact part $\mathcal{U}_{nc}$. For the compact part, Prop.~\ref{prop.control-err} continues to apply; whereas for the non-compact part, we can use Asm.~\ref{asm.tight} to control the $p(\tilde{u}_{nc}|\tilde{x})$ to be small. In this way, we can still have Eq.~(\ref{eq.miao}) with small and controllable errors.

The following example shows that Asm.~\ref{asm.tight} is mild and can hold when the exogenous distribution is tight:

\begin{example}[ANM with tightness]
    Suppose that $X$ and $U$ satisfy the ANM, i.e., $X=g_X(U)+N_X$, with $N_X$ the noise. If $g_X$ is invertible and the distribution of $N_X$ is tight (see Def.~\ref{def.tight}), then $\mathcal{L}_{U|X}$ is uniformly tight in arbitrary compact interval $[a,b]$.
\end{example}

Equipped with Asm.~\ref{asm.tight}, we now introduce Prop.~\ref{prop.dis-err unbd} for controlling the discretization error induced by the non-compact part of the domain $\mathcal{U}$.

\begin{proposition}
    Suppose that $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$, and that the map $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz continuous wrt TV distance. Suppose that $\{\mathcal{X}_i\}_{l_X}$ is a partition of $[a,b]$ satisfying $len(\mathcal{X}_i)\leq \epsilon/2L_U$. Then, $\forall\epsilon>0, \exists T$, let $\mathcal{U}_{nc}:=\{u:|u|\geq T\}$, we have $p(\tilde{u}_{nc}|\tilde{x}_i) \leq \epsilon$.
    \label{prop.dis-err unbd}
\end{proposition}

Prop.~\ref{prop.dis-err unbd} means that we can take a compact subspace of $\mathcal{X}$ for establishing Eq.~(\ref{eq.miao}), in order to control the additional error induced by the non-compact part of $\mathcal{U}$. 


\subsection{Hypothesis test}
\label{sec.hypo-test}

In this section, we present our hypothesis testing procedure. Specifically, we adopt the test statistic proposed by \cite{miao2018identifying} and analyze its asymptotic distribution under the null hypothesis. Additionally, we investigate the behavior of the statistic under the alternative hypothesis and establish the asymptotic power of our test.

We first introduce our test statistic. The idea is that we can assess whether $\mathbb{H}_0$ is correct by looking at the residual of the least-square solution of Equation~(\ref{eq.miao}). If $\mathbb{H}_0$ is correct, then Equation~(\ref{eq.miao}) is identifiable, hence the least-square residual should be close to zero. In practice, to enhance the capacity of the statistic, we can aggregate the residuals obtained from the solutions of Equation~(\ref{eq.miao}) with respect to all levels of $\tilde{Y}$. Specifically, we let
\begin{equation*}
    q:=[\mathbb{P}(\tilde{y}_1|\tilde{X}),...,\mathbb{P}(\tilde{y}_{l_{\tilde{Y}}-1}|\tilde{X})]^T
\end{equation*}
be the column vector that aggregates $\mathbb{P}(\tilde{y}|\tilde{X})$ for all (free) levels of $\tilde{Y}$, and let
\begin{equation*}
    Q:=\mathrm{diag}[\mathbb{P}(\tilde{W}|\tilde{X}),...,\mathbb{P}(\tilde{W}|\tilde{X})]
\end{equation*}
be the block diagonal matrix with $(l_{\tilde{Y}}-1)$ repeating blocks of $\mathbb{P}(\tilde{W}|\tilde{X})$ in the diagonal. Consider corresponding estimators $\hat{q}$ and $\hat{Q}$ satisfy that
\begin{align*}
    n^{1/2}(\hat{q} - q) &\to N(0,\Sigma) \,\, \text{in distribution}, \\
    \hat{Q}\to Q, \hat{\Sigma} &\to \Sigma \,\, \text{in probability,} 
\end{align*}
with $\hat{\Sigma}, \Sigma$ both positive definite\footnote{We adopt maximum likelihood estimation to obtain $\hat{q}$, $\hat{Q}$, and $\hat{\Sigma}$. Please refer to Appx.~\ref{app-sec.mle} for details.}. Then, we have the least-square residual of regressing $\hat{\Sigma}^{-1/2} \hat{q}$ on $\hat{\Sigma}^{-1/2} \hat{Q}$ to be
\begin{equation*}
    \xi := \{I - \hat{\Sigma}^{-1/2} \hat{Q}^T (\hat{Q} \hat{\Sigma}^{-1} \hat{Q}^T)^{-1} \hat{Q} \hat{\Sigma}^{-1/2}\} \hat{\Sigma}^{-1/2} \hat{q}.
\end{equation*}
Following \cite{miao2018identifying}, we adopt the squared residual $T:=n\xi^T \xi$ as our test statistic. 

We then analyze the asymptotic distribution of $T$ under $\mathbb{H}_0$. Specifically, we show that $T$ asymptotically follows a chi-squared distribution $\chi^2_k$, where the degrees of freedom $k=(l_{\tilde{X}}-l_{\tilde{W}})(l_{\tilde{Y}}-1)$ is determined by the additional levels that $\tilde{X}$ has beyond $\tilde{W}$, multiplied by the level of $\tilde{Y}$. Formally, denote $l$ in short for $(l_{\tilde{X}},l_{\tilde{Y}},l_{\tilde{W}})$ and denote $z_{1-\alpha}$ as the $(1-\alpha)$-th quantile of $\chi^2_k$, we then have the following result:


\begin{theorem}
    Suppose that Assumptions~\ref{asm.comp-main}-\ref{asm.tv-smooth} hold, then under $H_0$, it holds that:
    \begin{equation*}
        T_{n,l} \to \chi_{k}^2 \,\, \text{in distribution}
    \end{equation*}
    as $n,l\to \infty$. As a result, for any $\alpha\in (0,1)$, we have:
    \begin{equation*}
        \lim_{n,l\to \infty} \mathbb{P}(T_{n,l}> z_{1-\alpha}) = \alpha.
    \end{equation*}
    In other words, the testing procedure we define has uniform asymptotic level $\alpha$.
\label{thm.control.type-i}
\end{theorem}

In general, we cannot expect that the test has power against alternatives to $\mathbb{H}_0$ without further restrictions on the alternative distribution. This is analogous to other conditional independence tests \cite{zhang2012kernel,runge2018conditional,christgau2023nonparametric} used for causal discovery. Therefore, to establish the power of our test, we put the following restriction on the alternative distribution:

\begin{assumption}
    We consider the local alternative $\mathbb{H}_1:\Theta$, where for each $\theta\in \Theta$, the integral equation
    \begin{equation}
        f_{\theta}(y|x)=\int h(y,w)f_{\theta}(w|x)dw
    \label{eq.int-eq}
    \end{equation}
    has no solution.
    \label{asm.int-eq}
\end{assumption}

\begin{remark}
    We show that $\mathbb{H}_1$ is indeed a local alternative, that is, there exists distributions satisfying $X\not\ind Y|U$ but do not belong to $\Theta$. Please refer to Appx.~\ref{app-sec.int-eq} for details.
\end{remark}

To understand the role of assump.~\ref{asm.int-eq}, note that to establish the power, it is important for the statistic $T$ to deviate from zero under the alternative model, which requires that the Equation~(\ref{eq.miao}) has no solution. Intuitively, this means the variability of $\mathbb{P}(\tilde{y}|\tilde{X})$ can not be fully explained by that of $\mathbb{P}(\tilde{W}|\tilde{X})$. For continuous variables, this then corresponds to the condition that the integral equation~(\ref{eq.int-eq}) has no solution.

In an empirical way, we can show that $\mathbb{H}_1$ covers many cases where the casual influence from $X$ to $Y$ is strong. Please refer to Appx.~\ref{app-sec.int-eq} for details.

Equipped with the above analyses, we now establish power against the local alternative $\mathbb{H}_1$ as follows:

\begin{theorem}
    Suppose that Assumptions~\ref{asm.comp-main}-\ref{asm.tv-smooth} holds, then for any $\alpha\in (0,1)$, it holds that:
    \begin{equation*}
        \lim_{n,l\to\infty}\mathbb{P}_{\Theta}(T_{n,l}>z_{1-\alpha})=1.
    \end{equation*}
    In other words, the limiting power of our test is one.
    \label{thm.type-ii}
\end{theorem}

==> icml24_para/method_v3_xw.tex <==
\section{Methodology}

In this section, we introduce a hypothesis-testing procedure based on discretization. At the core of our procedure lies finding a discretization procedure that establish the identifiability of Eq.~(\ref{eq.miao}). 

To achieve this goal, in Sect.~\ref{sec.comp}, we first introduce a discretization procedure which, under the completeness assumption, can ensure the discretized $\tilde{X}$ and $\tilde{W}$ meet the rank regularity. Then, in Sect.~\ref{sec.dis-error}, we analyze the errors induced during the discretization. Under smoothness conditions regarding structural equations, we show that they can be effectively controlled to be arbitrarily small if the bin number is sufficiently large. Finally, based on the above analyses, we introduce our testing statistic and discuss the asymptotic level and power of the test in Sect.~\ref{sec.hypo-test}.

\subsection{Discretization under completeness}
\label{sec.comp}

In this section, we introduce a discretization procedure to establish the identifiability of Eq.~\eqref{eq.miao}. As mentioned previously, this involves finding discretization for $W$ and $X$ such that the resulted $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank. We first introduce the following completeness conditions that have been similarly adopted for continuous variables in causal inference \cite{miao2018identifying, miao2022identifying}, which ensures the existence of such a discretization. 


\begin{assumption}[Completeness]
    We assume the conditional distributions $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|X}$ are complete. That is, for any bounded function $g$, we assume
    \begin{align*}
        \mathbb{E}[g(u)|x]=0 \,\, &\text{almost surely iff} \,\, g(u)=0 \,\, \text{almost surely}, \\
        \mathbb{E}[g(w)|x]=0 \,\, &\text{almost surely iff} \,\, g(w)=0 \,\, \text{almost surely}.
    \end{align*}
    \label{asm.comp-main}
\end{assumption}
\vspace{-.5cm}
To understand the role of assump.~\ref{asm.comp-main} in our method, note that in the case when $W$ (\emph{resp.} $U$) is discrete, the completeness of $\mathcal{L}_{W|X}$ (\emph{resp.} $\mathcal{L}_{U|X}$) means the conditional probability matrix $\mathbb{P}(W|X)$ has full row rank, as required in the procedure for discrete variables \cite{miao2018identifying}. As will be shown later, this condition enables us to find a discretization such that $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank. Further, when combined with the completeness of $\mathcal{L}_{U|X}$, we can demonstrate the existence of discretization for $U$ such that the matrix $\mathbb{P}(\tilde{W}|\tilde{U})$ is invertible, which is also required for the identifiability of Eq.~\eqref{eq.miao}.

The following example shows that assump.~\ref{asm.comp-main} can hold for a wide range of Addictive Noise Models (ANMs).

\begin{example}[ANM with completeness]
    Suppose that $X,U,W$ satisfy the ANM, i.e., $X=g_X(U)+N_X, W=g_W(U)+N_W$, with $N_X,N_W$ being the noises. If $g_X$ is invertible with a non-zero derivative, and $N_X$, $N_W$ have non-zero characterization functions, then the conditional distributions $\mathcal{L}_{U|X}$ and $\mathcal{L}_{W|X}$ are both complete.
    \label{exam.anm.completeness}
\end{example}

\begin{remark}
    We also provide an example in which $U$ is a mediator and assump.~\ref{asm.comp-main} is satisfied. Please refer to Appx.~\ref{app-sec.example-comp} for details.
\end{remark}

The completeness condition has been similarly assumed in causal hypothesis testing and causal inference, with the difference that our condition is not restricted to square-integrable functions.  For example, the completeness of $\mathcal{L}_{U|X}$ was assumed by \cite{miao2018identifying,miao2022identifying}\footnote{See Condition~(ii) in \cite{miao2018identifying} (by dropping $Z$) and assump.~3 in \cite{miao2022identifying}.}. Besides, a discrete version of the completeness of $\mathcal{L}_{W|X}$, \emph{i.e.}, $\mathbb{P}(W|X)$ has full row rank, was required by the procedure described by \cite{miao2018identifying}. Indeed, in \cite{miao2018identifying}, they also assumed the completeness of $\mathcal{L}_{X|W}$\footnote{See Condition~(iii), where $z$ is replaced with $x$ to induce variation for identification.}. However, this assumption is to ensure the solution's existence in the integral function for identifying the causal effect, which therefore is not required in this paper.

Next, we show that, under assump.~\ref{asm.comp-main}, we can find a discretization procedure such that the $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank and the matrix $\mathbb{P}(\tilde{W}|\tilde{U})$ is invertible.

\begin{proposition}
    Suppose assump.~\ref{asm.comp-main} holds. Then, for any discretization $\tilde{W}$ of $W$, there exists a discretization $\tilde{X}$ of $X$ such that the matrix $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank. Similarly, there also exists a discretization $\tilde{U}$ of $U$ such that the matrix $\mathbb{P}(\tilde{W}|\tilde{U})$ is invertible.
    \label{prop.rank-dis-main}
\end{proposition}

% [by MZ]
% \begin{remark}
%     We leave the proof to Appx.~\ref{app-sec.discrete}. Roughly speaking, we first show that for any $\{\mathcal{W}_i\}_{l_{\tilde{W}}}$, the functions $F(x|\tilde{w}_1),...,F(x|\tilde{w}_{l_{\tilde{W}}})$, with $F(x|\tilde{w}_i):=F(x|W\in\mathcal{W}_i)$, are linear independent under the completeness of $\mathcal{L}_{W|X}$. Then, we prove with induction that there exists $x_1,...,x_{l_{\tilde{X}}}$ with $l_{\tilde{X}} > l_{\tilde{W}}$, such that the vectors $F({\boldsymbol{x}}|\tilde{w}_1),...,F({\boldsymbol{x}}|\tilde{w}_{l_{\tilde{W}}})$ are linear independent, with $F({\boldsymbol{x}}|\tilde{w}_i) := \left[ F({x}_1|\tilde{w}_i),...,F({x}_{l_{\tilde{X}}}|\tilde{w}_i)\right]^\top$. In this regard, we can define the partition of $\mathcal{X}$ to be $\{[x_i,x_{i+1}]\}_{l_{\tilde{X}}}$, and show $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank by noticing that $\mathbb{P}(\tilde{W}|\tilde{X}):=[\mathbb{P}(\tilde{w}_i|\tilde{x}_j)]_{i,j}$ and $\mathbb{P}(\tilde{w}_i|\tilde{x}_j) \propto F(x_{j+1}|W \in \mathcal{W}_i)-F(x_j|W \in \mathcal{W}_i)$.
% \end{remark}

% Inspired by Prop.~\ref{prop.rank-dis-main}, we introduce our discretization process in Alg.~\ref{alg.dis}. The algorithm mainly contains three steps. First, in line 1, we uniformly discretize $W$ into $l_{\tilde{W}}$ bins to obtain $\tilde{W}$. Indeed, the choice of discretization for $W$ is arbitrary, as indicated by Prop.~\ref{prop.rank-dis-main}. Next, in lines 2-7, we discretize $X$ to construct $\tilde{X}^\prime$ that contains the same number of bins as $W$, such that $\mathbb{P}(\tilde{X}^\prime|\tilde{W})$ and therefore $\mathbb{P}(\tilde{W}|\tilde{X}^\prime)$ is invertible. Finally, we add another $(l_{\tilde{X}}-l_{\tilde{W}})$ levels to $\tilde{X}^\prime$ to obtain $\tilde{X}$ in lines 8-11. In this regard, the obtained $\mathbb{P}(\tilde{W}|\tilde{X})$ can have full row rank.

% In the second step (lines 2-7), we iteratively search for $x_i$ such that the matrix $M_i:=F(\boldsymbol{x}_{[i]}|\tilde{\boldsymbol{w}}_{[i]})$ is invertible given $x_1,...,x_{i-1}$. This can be achieved by noting that the functions $F(x|\tilde{w}_1),...,F(x|\tilde{w}_{l_W})$ are linear independent under the completeness condition. Once we have the invertibility of $M$, we have $\mathbb{P}(\tilde{W}|\tilde{X}^\prime):=[\mathbb{P}(\tilde{w}_i|\tilde{x}_j)]_{i,j}$ is invertible, by noticing $\mathbb{P}(\tilde{w}_i|\tilde{x}_j) \propto F(x_{j+1}|W \in \mathcal{W}_i)-F(x_j|W \in \mathcal{W}_i)$. To find such an $x_i$, note that $\mathrm{det}(M_i)$ can be expanded as:
% \begin{equation*}
%     \mathrm{det}(M_i)(x_i) = \sum_{j=1}^i (-1)^{1+j} d_j F(x_i|\tilde{w}_j),
% \end{equation*}
% where $d_j:=\mathrm{det}(F(x_{[i-1]}|\tilde{w}_{[i]\backslash j}))$. By induction, there exists an $i-1$ dimensional minor among $\{d_j\}$ that is non-zero. Since $F(x|\tilde{w}_1),...,F(x|\tilde{w}_{l_W})$ are linear independent, there exists $x_i$ such that $\mathrm{det}({M_i})(x_i) \neq 0$, which means $F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]})$ is invertible. 

% [XW's older version]
\begin{remark}
    We leave the proof to Appx.~\ref{app-sec.discrete}. Roughly speaking, we first show that given $\{\mathcal{W}_i\}_{i=1}^{l_W}$, the functions $F(x|\tilde{w}_1),...,F(x|\tilde{w}_{l_W})$ are linear independent under the completeness condition of $\mathcal{L}_{W|X}$. Then we prove with induction that there exists $\tilde{x}_1,...,\tilde{x}_{l_X}$ with $l_X > l_W$, such that $\left[F(\boldsymbol{x}|\tilde{w}_1),...,F(\boldsymbol{x}|\tilde{w}_{l_W})\right]$ is linear independent, where $F(\boldsymbol{x}|\tilde{w}_i) = \left[ F(\tilde{x}_1|\tilde{w}_i),...,F(\tilde{x}_{l_X}|\tilde{w}_i)\right]^\top$. 
\end{remark}

Inspired by Prop.~\ref{prop.rank-dis-main}, we introduce our discritization procedure in Alg.~\ref{alg.dis}. The algorithm mainly contains three steps. First, in line 1, we uniformly discretize $W$ into $l_{\tilde{W}}$ bins to obtain $\tilde{W}$. Indeed, the choice of discretization for $W$ is arbitrary, as indicated by Prop.~\ref{prop.rank-dis-main}. Next, in lines 2-7, we discretize $X$ to construct $\tilde{X}^\prime$ that contains the same number of bins as $W$, such that $\mathbb{P}(\tilde{X}^\prime|\tilde{W})$ and therefore $\mathbb{P}(\tilde{W}|\tilde{X}^\prime)$ is invertible. Finally, we add another $(l_{\tilde{X}}-l_{\tilde{W}})$ levels to $\tilde{X}^\prime$ to obtain $\tilde{X}$ in lines 8-11. In this regard, the obtained $\mathbb{P}(\tilde{W}|\tilde{X})$ can have full row rank.

In the second step (lines 2-7), we iteratively search for $x_i$ such that the matrix $M_i:=F(\boldsymbol{x}_{[i]}|\boldsymbol{w}_{[i]})$ is invertible given $x_1,...,x_{i-1}$. This can be achieved by noting that the functions $F(x|\tilde{w}_1),...,F(x|\tilde{w}_{l_W})$ are linear independent under the completeness condition. Once we have the invertibility of $M_i$, we have $\mathbb{P}(\tilde{X}|\tilde{W}):=\{\mathbb{P}(\tilde{x}_i|\tilde{w}_j)\}_{i,j}$ is invertible, with $\mathbb{P}(\tilde{x}_i|\tilde{w}_j):= F(x_i|W \in \mathcal{W}_j)-F(x_{i-1}|W \in \mathcal{W}_j)$ and $\mathcal{X}_i:=[x_{i-1},x_i)$ $\left( (-\infty,x_1) \text{ for $i=1$}\right)$. To find such an $x_i$, note that $\mathrm{det}(M_i)$ can be expanded as:
\begin{align*}
    \mathrm{det}(M_i)(x_i) = \sum_{j=1}^i (-1)^{1+j} d_j F(x_i|\tilde{w}_j),
\end{align*}
where $d_j:=\mathrm{det}(F(x_{[i-1]}|\tilde{w}_{[i]\backslash j}))$. By induction, there exists an $i-1$ dimensional minor among $\{d_j\}$ is non-zero. Since $F(x|\tilde{w}_{[i]})$ are linear independent, there exists $x_i$ such that $\mathrm{det}_{M_i}(x_i) \neq 0$, which means $F(\boldsymbol{x}_{[i]}|\tilde{w}_{[i]})$ is invertible. 


\begin{algorithm}[t]
   \caption{Rank preserving discretization}
   \label{alg.dis}
\begin{flushleft}
\textbf{Input:} Continuous variables $X$, $W$; Bin numbers $l_{\tilde{X}}> l_{\tilde{W}}$. \\
\textbf{Output:} Discrete variables $\tilde{X}$, $\tilde{W}$ satisfying $\mathbb{P}(\tilde{W}|\tilde{X})$ has full row rank.
\end{flushleft}
\begin{algorithmic}[1]
    \STATE Discretize $W$ with $l_{\tilde{W}}$ uniform bins to obtain $\tilde{W}$.
    \FOR{$i=1:l_{\tilde{W}}$}
        \FOR{$j=1:i$}
            \STATE Estimate $d_j=\mathrm{det}(F(x_{[i-1]}|\tilde{w}_{[i]\backslash j}))$
        \ENDFOR
        \STATE Search for $x_i$ s.t. $\sum_{j=1}^i (-1)^{1+j} d_j F(x_i|\tilde{w}_j) \neq 0$.
    \ENDFOR
    \FOR{$i=l_{\tilde{W}}+1:l_{\tilde{X}}$}
        \STATE Set $[x_i,x_{i+1}]$ to the $i$-th uniform bin of $\mathcal{X}\backslash [x_1,x_{l_{\tilde{W}}}]$.
    \ENDFOR
    \STATE Discretize $X$ with $\{[x_i,x_{i+1}]\}_{i=1}^{l_{\tilde{X}}}$ to obtain $\tilde{X}$.
    \STATE \textbf{return} $\tilde{X}$, $\tilde{W}$.
\end{algorithmic}
\end{algorithm}

\textbf{Choosing the bin number.}
    The bin number is a trade-off between the discretization error and the estimation of discrete probabilities. While a larger bin number effectively controls discretization error, it may lead to inaccurate probability estimation due to insufficient samples in each bin. To balance this trade-off, we follow the heuristics proposed by \cite{dougherty1995supervised} and set the bin number to $\left \lfloor \log(n) \right \rfloor$.
    
\begin{remark}
    Since $U$ is unobserved, we cannot discretize $U$. However, according to Prop.~\ref{prop.rank-dis-main}, there exists a $\tilde{U}$ such that $\mathbb{P}(\tilde{W}|\tilde{U})$ is invertible. 
\end{remark}







\subsection{Discretization error analysis}
\label{sec.dis-error}

In this section, we discuss the discretization error control in Eq.~\eqref{eq.miao}. Our goal is to asymptotically maintain the conditional independence $X\ind Y|U$ and $X\ind W|U$ after discretization by controlling the error $|p(\tilde{y}|\tilde{u})-p(\tilde{y}|\tilde{x},\tilde{u})|$ and $|p(\tilde{w}|\tilde{u})-p(\tilde{w}|\tilde{x},\tilde{u})|$ over discretized variables under the null hypothesis $\mathbb{H}_0$, which allows us to establish the linear relation in Eq.~\eqref{eq.miao} asymptotically. 


For this purpose, we first introduce the following Total Variation (TV) smoothness condition, which states that the conditional distributions $\mathcal{L}_{Y|U=u}$ and $\mathcal{L}_{W|U=u}$ should change smoothly with respect to $u$.


\begin{assumption}[TV smoothness]
\label{asm.tv-smooth-main}
    We assume the maps $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are Lipschitz continuous with respect to TV distance. That is, for any $u,u^\prime \in \mathcal{U}$, we assume there exist $L_Y$ and $L_W$, respectively, such that:
    \begin{align*}
        \mathrm{TV}(\mathcal{L}_{Y|U=u},&\mathcal{L}_{Y|U=u^\prime}) \leq L_Y |u-u^\prime|, \\
        \mathrm{TV}(\mathcal{L}_{W|U=u},&\mathcal{L}_{W|U=u^\prime}) \leq L_W |u-u^\prime|,
    \end{align*}
    where $TV(\mathbb{P}_1,\mathbb{P}_2) := \sup_A \left| \int_A (p_1(x) - p_2(x)) dx\right|$.
\end{assumption}



To understand the role of assump.~\ref{asm.tv-smooth-main} in discretization error control, note that for a small bin $\mathcal{U}_i$ of $\mathcal{U}$ and any $u\in\mathcal{U}_i$, assump.~\ref{asm.tv-smooth-main} means that the distance
\begin{equation*}
    \mathrm{TV}(\mathcal{L}_{Y|U\in \mathcal{U}_i},\mathcal{L}_{Y|U=u})
\end{equation*}
is small. Similarly, it also indicates that the distance
\begin{equation*}
    \mathrm{TV}(\mathcal{L}_{Y|X\in\mathcal{X}_j,U\in \mathcal{U}_i},\mathcal{L}_{Y|X\in\mathcal{X}_j,U=u})
\end{equation*}
is small. Since we have $\mathcal{L}_{Y|U=u}=\mathcal{L}_{Y|X\in\mathcal{X}_j,U=u}$ under $\mathbb{H}_0: X\ind Y|U$, by applying triangle inequality, we can control the distance $\mathrm{TV}(\mathcal{L}_{Y|U\in \mathcal{U}_i},\mathcal{L}_{Y|X\in\mathcal{X}_j,U\in \mathcal{U}_i})$, and hence control the error $|p(\tilde{y}|\tilde{u})-p(\tilde{y}|\tilde{x},\tilde{u})|$.

The following example shows that assump.~\ref{asm.tv-smooth-main} can hold for a wide range of ANM models.


\begin{example}[ANM with TV smoothness]
    Suppose that $Y,U,W$ satisfy the ANM, i.e., $Y=g_Y(U)+N_Y, W=g_W(U)+N_W$, with $N_Y, N_W$ being the noises. If $g_Y$ and $g_W$ are differentiable, and the probability densities of $N_Y$ and $N_W$ have absolutely integrable derivatives, then the maps $u\mapsto \mathcal{L}_{Y|U=u}$ and $u\mapsto \mathcal{L}_{W|U=u}$ are Lipschitz continuous with respect to TV distance.
    \label{exam.tv-smooth}
\end{example}

\begin{remark}
    We also provide an example in which $U$ is a mediator and Asm.~\ref{asm.tv-smooth-main} is satisfied. Please refer to Appx.~\ref{app-sec.tv-example} for details.
\end{remark}


Under this assumption, we show that the discretization error can be controlled, as long as the bin length is small.
\begin{proposition}
\label{prop.control-err-main}
    Suppose that $\{\mathcal{U}_i\}_{l_{U}}$ is a partition of $\mathcal{U}$, and that for every bin $\mathcal{U}_i$,
    \begin{equation*}
        len(\mathcal{U}_i)\leq \frac{1}{2}min\{\epsilon/L_Y,\epsilon/L_W\}.
    \end{equation*}
    Then, under assump.~\ref{asm.tv-smooth-main} and $\mathbb{H}_0:X\ind Y|U$, we have:
    \begin{align*}
        |p(\tilde{y}|\tilde{u}_i) - p(\tilde{y}|\tilde{x},\tilde{u}_i)| \leq \epsilon, \,\, |p(\tilde{w}|\tilde{u}_i) - p(\tilde{w}|\tilde{x},\tilde{u}_i)| \leq \epsilon.
    \end{align*}
\end{proposition}
According to Prop.~\ref{prop.control-err-main}, when $\mathcal{U}$ is a compact interval, we can (implicitly) partition $\mathcal{U}$ into sufficiently refined bins, by setting the bin number large enough. However, when considering $\mathcal{U}=\mathbb{R}$, it is intractable to partition into finite bins with finite length. To extend the above result to $\mathbb{R}$, we assume $\mathcal{L}_{U|X}$ to be tight, meaning that for large values of $u$'s, the conditional probability $p(u|x)$ is close to zero. The formal definition of tight distribution is given below. 


\begin{definition}[Tight distribution] The marginal distribution $\mathcal{L}_U$ is said to be tight if $\forall \epsilon>0, \exists T, \forall t\geq T,\mathcal{L}(|U|\geq t)\leq \epsilon$. The conditional distribution $\mathcal{L}_{U|X}$ is said to be uniformly tight\footnote{We use the term ``uniform'' because the $T$ holds uniformly for all $x\in[a,b]$.} in $[a,b]$ if $\forall \epsilon>0, \exists T, \forall t\geq T, \forall x\in [a,b],\mathcal{L}(|U|\geq t|x)\leq \epsilon$.
\label{def.tight-main}
\end{definition}
\begin{remark}
    The tightness condition holds for many distributions, encompassing those from the exponential family, such as Gaussian, Gamma, and exponential distributions.
\end{remark}

We then assume the following tightness condition:
\begin{assumption}
    We assume the conditional distribution $\mathcal{L}_{U|X}$ is uniformly tight for any compact interval $[a,b]$.
    \label{asm.tight-main}
\end{assumption}

To see the role of assump.~\ref{asm.tight-main} in discretization error control under non-compact domains, note that we can partition $\mathcal{U}$ into a compact part $\mathcal{U}_c$ and a non-compact part $\mathcal{U}_{nc}$, whose errors can be respectively controlled by Prop.~\ref{prop.control-err-main} and assump.~\ref{asm.tight-main}. In this way, we can establish Eq.~\eqref{eq.miao} asymptotically with respect to the bin length. 

The following example shows that assump.~\ref{asm.tight-main} can easily hold as long as the distribution of the noise is tight.
\begin{example}[ANM with tightness]
    Suppose that $X$ and $U$ satisfy the ANM, i.e., $X=g_X(U)+N_X$, with $N_X$ the noise. If $g_X$ is invertible and the distribution of $N_X$ is tight, then $\mathcal{L}_{U|X}$ is uniformly tight in an arbitrary compact interval $[a,b]$.
    \label{exam.anm.tight}
\end{example}

Equipped with assump.~\ref{asm.tight-main}, we have the following result for controlling the discretization error induced by the non-compact part of the domain $\mathcal{U}$.

\begin{proposition}
    Suppose that $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$, and that the map $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz continuous wrt TV distance. Suppose that $\{\mathcal{X}_i\}_{l_X}$ is a partition of $[a,b]$ satisfying $len(\mathcal{X}_i)\leq \epsilon/2L_U$. Then, $\forall\epsilon>0, \exists T$, let $\mathcal{U}_{nc}:=\{u:|u|\geq T\}$, we have $p(\tilde{u}_{nc}|\tilde{x}_i) \leq \epsilon$.
    \label{prop.dis-err unbd}
\end{proposition}

Prop.~\ref{prop.dis-err unbd} means that we can take a compact subspace of $\mathcal{X}$ for discretization to establish Eq.~\eqref{eq.miao}, since the additional error introduced by the non-compact part of $\mathcal{U}$ can be effectively controlled.





\subsection{Hypothesis test}
\label{sec.hypo-test}

In this section, we present our hypothesis testing procedure. Specifically, we adopt the test statistic proposed by \cite{miao2018identifying} and analyze its asymptotic distribution under the null hypothesis. Additionally, we investigate the behavior of the statistic under the alternative hypothesis and establish the asymptotic power of our test.

We first introduce our test statistic. The idea is that we can assess whether $\mathbb{H}_0$ is correct by looking at the residual of the least-square solution of Eq.~\eqref{eq.miao}. If $\mathbb{H}_0$ is correct, then the linear relation in Eq.~\eqref{eq.miao} holds, hence the least-square residual should be close to zero. In practice, to enhance the capacity of the statistic, we can aggregate the residuals obtained from the solutions of Eq.~\eqref{eq.miao} with respect to all levels of $\tilde{Y}$. Specifically, we let
\begin{equation*}
    q:=[\mathbb{P}(\tilde{y}_1|\tilde{X}),...,\mathbb{P}(\tilde{y}_{l_{\tilde{Y}}-1}|\tilde{X})]^T
\end{equation*}
be the column vector that aggregates $\mathbb{P}(\tilde{y}|\tilde{X})$ for all (free) levels of $\tilde{Y}$, and let
\begin{equation*}
    Q:=\mathrm{diag}[\mathbb{P}(\tilde{W}|\tilde{X}),...,\mathbb{P}(\tilde{W}|\tilde{X})]
\end{equation*}
be the block diagonal matrix with $(l_{\tilde{Y}}-1)$ repeating blocks of $\mathbb{P}(\tilde{W}|\tilde{X})$ in the diagonal. After performing maximum likelihood estimation\footnote{Please refer to Appx.~\ref{app-sec.mle} for details.}, we can estimate $\hat{q}$ and $\hat{Q}$, such that
\begin{align*}
    n^{1/2}(\hat{q} - q) &\to N(0,\Sigma) \,\, \text{in distribution}, \\
    \hat{Q}\to Q, \hat{\Sigma} &\to \Sigma \,\, \text{in probability,} 
\end{align*}
with $\hat{\Sigma}, \Sigma$ both positive definite. Then, we have the least-square residual of regressing $\hat{\Sigma}^{-1/2} \hat{q}$ on $\hat{\Sigma}^{-1/2} \hat{Q}$ to be
\begin{equation*}
    \xi := \{I - \hat{\Sigma}^{-1/2} \hat{Q}^T (\hat{Q} \hat{\Sigma}^{-1} \hat{Q}^T)^{-1} \hat{Q} \hat{\Sigma}^{-1/2}\} \hat{\Sigma}^{-1/2} \hat{q}.
\end{equation*}
Following \cite{miao2018identifying}, we adopt the squared residual $T:=n\xi^T \xi$ as our test statistic. 

We then analyze the asymptotic distribution of $T$ under $\mathbb{H}_0$. Specifically, we show that $T$ asymptotically follows a chi-squared distribution $\chi^2_k$, where the degree of freedom $k=(l_{\tilde{X}}-l_{\tilde{W}})(l_{\tilde{Y}}-1)$ is determined by the additional levels that $\tilde{X}$ has beyond $\tilde{W}$, multiplied by the level of $\tilde{Y}$. Formally, denote $l$ in short for $(l_{\tilde{X}},l_{\tilde{Y}},l_{\tilde{W}})$ and $z_{1-\alpha}$ as the $(1-\alpha)$-th quantile of $\chi^2_k$, we have the following result:


\begin{theorem}
    Suppose that assump.~\ref{asm.comp-main},~\ref{asm.tv-smooth-main},~\ref{asm.tight-main} hold, then under $H_0$, we have that:
    \begin{equation*}
        T_{n,l} \to \chi_{k}^2 \,\, \text{in distribution}
    \end{equation*}
    as $n,l\to \infty$. As a result, for any $\alpha\in (0,1)$, we have:
    \begin{equation*}
        \lim_{n,l\to \infty} \mathbb{P}(T_{n,l}> z_{1-\alpha}) = \alpha.
    \end{equation*}
    In other words, the testing procedure we define has uniform asymptotic level $\alpha$.
\label{thm.control.type-i-main}
\end{theorem}

In general, we cannot expect that the test has power against alternatives to $\mathbb{H}_0$ without further restrictions on the alternative distribution. This is analogous to other conditional independence tests \cite{zhang2012kernel,runge2018conditional,christgau2023nonparametric} used for causal discovery. Therefore, to establish the power of our test, we put the following restriction on the alternative distribution:

\begin{assumption}
    We consider the local alternative $\mathbb{H}_1$, such that the following integral equation has no solution:
    \begin{equation}
        p(y|x)=\int h(y,w)p(w|x)dw.
    \label{eq.int-eq}
    \end{equation}
    \label{asm.int-eq-main}
\end{assumption}
\begin{remark}
    Empirically, we show that $\mathbb{H}_1$ can hold in many cases. Besides, we can prove that $\mathbb{H}_1$ is indeed a local alternative, that is, there exists $\mathbb{P}$ satisfying $X\not\ind Y|U$ but does not satisfy assump.~\ref{asm.int-eq-main}. See Appx.~\ref{app-sec.int-eq} for details.
\end{remark}

To understand the role of assump.~\ref{asm.int-eq-main} in controlling the type-II error, we first note that the residues in $T$ should deviate from zero under the alternative model, which requires that Eq.~\eqref{eq.miao} has no solution. Intuitively, this means the variability of $\mathbb{P}(\tilde{y}|\tilde{X})$ can not be fully explained by that of $\mathbb{P}(\tilde{U}|\tilde{X})$ and therefore $\mathbb{P}(\tilde{W}|\tilde{X})$, which corresponds assump.~\ref{asm.int-eq-main} for continuous variables. On the other hand, we can establish the existence of the solution in Eq.~\eqref{eq.int-eq} under $\mathbb{H}_0$. Therefore, this assumption can effectively distinguish $\mathbb{H}_0$ from the alternative. 

% Please refer to Appx.~\ref{app-sec.int-eq} for details.

Under this assumption, we can establish the asymptotic power for our testing procedure.  
\begin{theorem}
    Suppose that assump.~\ref{asm.comp-main},~\ref{asm.tv-smooth-main},~\ref{asm.tight-main},~\ref{asm.int-eq-main} hold, then for any $\alpha\in (0,1)$, we have that:
    \begin{equation*}
        \lim_{n,l\to\infty}\mathbb{P}(T_{n,l}>z_{1-\alpha})=1.
    \end{equation*}
    In other words, the limiting power of our test is one.
    \label{thm.type-ii-main}
\end{theorem}

==> icml24_para/mz_v1/experiment.tex <==
\clearpage
\section{Experiment}

In this section, we evaluate \xw{apply} our method on synthetic data and a real-world causal discovery task \xw{causal discovery on a real-world dataset}.

\textbf{Compared baselines.} To the best of our knowledge, there has not been any existing method for continuous CI testing under measurement bias. Therefore, we compared our method to \xw{We therefore compare to} three classical hypothesis testing methods \xw{procedures}: \textbf{i)} the Kernel-based CI (KCI) test \cite{zhang2012kernel} that tested the conditional independence $X\ind Y|W$ given the proxy variable $W$ using kernel matrices; \textbf{ii)} the Integrated Conditional Moment (ICM) method \cite{bierens1997asymptotic} that tested whether the conditional moment equation $E[Y-g(W)|X]$ has a solution; and \textbf{iii)} the Miao method \xw{procedure described by} \cite{miao2018identifying} (\xw{Miao for simplicity}) that was designed for testing CI with a discrete conditional variable and its corresponding proxy \xw{for CI testing over discrete variables using the proxy variable.}.

\textbf{Evaluation metrics.} We use two metrics to evaluate the performance: type I error and type II error. \xw{We report the type-I and type-II error rates}. Type I error is the rate of \xw{falsely} rejecting a true null hypothesis \xw{when it is true}, and type II error is the rate of \xw{failing to reject} accepting a null hypothesis \xw{when it is false}. Note that \xw{Ideally} for a good testing method \xw{a valid testing procedure}, the type I error is \xw{should be} close to the significance level $\alpha$, and \xw{while the} type II error as small as possible \xw{should be close to 0}.

\textbf{Implementation details.} For all methods \xw{delete}, the significance level is set to $\alpha=0.05$ \xw{We set the significance level $\alpha$ to 0.05}. For our method, the bin numbers are set to \xw{We set the bin numbers of our method to} $I=14,J=5,L=12$, respectively. The maximum likelihood estimators of $q,Q,\Sigma$ are detailed in Appendix~\ref{app-sec.mle}. \xw{We employ the maximum likelihood estimation to estimate $q,Q,\Sigma$, with details left in Appendix~\ref{app-sec.mle}.}  For the \xw{delete ``the"} KCI and ICM baselines \xw{delete ``baselines"}, we used \xw{adopt} the implementations provided in the $\mathrm{causallearn}$\footnote{\url{https://github.com/py-why/causal-learn}} and $\mathrm{mliv}$\footnote{\url{https://github.com/causal-machine-learning-lab/mliv}} APIs, respectively. For the Miao baseline \xw{procedure of Miao}, we used \xw{implement} the author's \xw{delete} R code \xw{released in the paper \cite{miao2018identifying}} and set $I=3,J=3,L=2$ as \xw{by} default.

\subsection{Synthetic data}

\textbf{Data generation.} We consider two cases, case I and case II, in which the data was respectively generated using the confounding graph in Figure~??, and the mediation graph in Figure~??. \xw{We consider two cases for data generation: the confounding graph in Fig.?? and the mediation graph in Fig.??.} For both cases, we considered \xw{follow} the addictive noise model \xw{to generate $V_i$, \emph{i.e.},}, $V_i=\sum_{j\in\mathbf{PA}_i} f_{ij}(V_i) + E_i$, where $V_i\in \{X,Y,U,W\}$ is a vertex in the graph, $\mathbf{PA}_i$ is the parent of $V_i$, and $E_i$ is the noise variable \xw{for each $V_i \in \{X,Y,U,W\}$, with $\mathbf{PA}_i$ and $E_i$ denoting its associated parent nodes and the noise}. For each $V_i$, the function $f_{ij}$ was randomly selected from $\{\mathrm{linear},\mathrm{tanh},\mathrm{sin},\mathrm{sigmoid}\}$, and the noise distribution was randomly chosen from $\{\mathrm{Gaussian},\mathrm{uniform},\mathrm{exponential},\mathrm{gamma}\}$. To remove the effect of randomness, we repeat the process $20$ times. \xw{For} Each time, we generate $100$ replications under $\mathbb{H}_0$ and $\mathbb{H}_1$, respectively, in order to \xw{to} compute \xw{record} the type I error \xw{rate} and the type II error \xw{rate}.

\textbf{Controlling the discretization error.} To demonstrate the effectiveness of \xw{our method guided by} Proposition~\ref{prop.control-err} in controlling the discretization error $\boldsymbol{e}_{\mathrm{dis}}=|\mathbb{P}(\tilde{y}|\tilde{u},\tilde{x})-\mathbb{P}(\tilde{y}|\tilde{u})|$, we compute $\boldsymbol{e}_{\mathrm{dis}}$ under different models (smooth v.s. nonsmooth) and bin lengths \xw{we compute ... with different bin numbers}, and show \xw{present} the results in Figure~\ref{fig.dis-err-control}. For the smooth model (blue line), we use the continuous $f_{ij}$ to generate data, thus Assumption~\ref{asm.tv-smooth} holds; meanwhile, for the nonsmooth model (orange line), we introduce several discontinuities to $f_{ij}$ to violate Assumption~\ref{asm.tv-smooth}.

\xw{In the first paragraph, we can only introduce the main result: $e \to 0$ as bin number goes to infinity. In the second paragraph, we introduce the result when the smoothness condition is violated. }

As we can see, for the smooth model, $\boldsymbol{e}_{\mathrm{dis}}$ quickly decreases to zero as the bin length becomes small. This result validates the effectiveness of Proposition~\ref{prop.control-err} in controlling the discretization error. In contrast, for the nonsmooth model, $\boldsymbol{e}_{\mathrm{dis}}$ is consistently large for all bin lengths, due to the jump of the conditional distribution $\mathcal{L}_{Y|U=u}$ under different $u$s in the same bin.

\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{icml24_figs/dis_err_control.pdf}
    \caption{Discretization error under \xw{with respect to} different bin lengths \xw{bin numbers}. Assumption~\ref{asm.tv-smooth} holds (resp. does not hold) in the smooth (resp. nonsmooth) model. \xw{Left (\emph{resp}.) corresponds to the case when the smoothness condition, \emph{i.e.}, assump.~\ref{asm.tv-smooth}, holds (\emph{resp.} does not hold).}}
    \label{fig.dis-err-control}
\end{figure}

\textbf{Influence of the bin number and the sample size.} In Figure~\ref{fig.samplesize-binnumber}, we report the type I and type II errors \xw{error rates} for different bin numbers $L=\{4,6,8,10,12,14\}$ and sample sizes $n=\{200,400,600,800,1200\}$. As shown, when the bin number and the sample size are both large \xw{as .... grow}, the type I error approaches the significance level $\alpha=0.05$, and the type II error is close to zero. These results demonstrate \xw{align with} the asymptotic \xw{level and power} power of our test \xw{testing procedure}, as derived \xw{claimed} in Theorem~\ref{thm.control.type-i} and Theorem~\ref{thm.type-ii}. We can also observe that for sample-insufficient cases (e.g., $n=200$) \xw{for small sample size (e.g....)}, the type II error increases a little bit \xw{slightly increases} as the bin number increases \xw{grows}. This may be because, for small $n$s, the number of samples in each bin is small, which induces errors for the estimation of $\hat{q}$ and $\hat{Q}$, and hence influences the type II error control process \xw{which may due to insufficient samples in each bin number to estimate the discrete probability?}.

\textbf{Comparison with baselines. \xw{Type-I and Type-II error rates.} \xw{We shall put this paragraph (the main result) before the sensitive analysis (e.g., discretization error) or others.}} We report the performance of our test and baseline methods in Figure~\ref{fig.cmp-baselines}. As we can see, our method demonstrates significant outperformance compared to the baselines. Specifically, the improvement over KCI can be attributed to the proper use of the proxy variable $W$; the advantage over ICM may stem from the relaxation of the parametric assumptions required to fit the moment equations; and the enhancement over Miao can be attributed to our comprehensive analysis of error control and rank preservation in the discretization process. \xw{This style is suitable for performance comparisons in prediction tasks because the advantage typically comes from the contribution in the proposed methodology. In statistical inference where the advantage often comes from theoretical insights, the common procedure is i) introduce the result ii) analyze the reason from the theoretical perspectives if any, why the baseline does not have inferential precision. For example, KCI cannot control the type-I error rate since conditioning on $W$ still introduce the bias. Another example: Miao's bin number is too small to make the independence hold...}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{icml24_figs/sample_size_bin_number.pdf}
    \caption{Type I and type II errors \xw{error rates} under \xw{w.r.t.} different bin numbers and sample sizes \xw{the bin number and the sample size}. We consider two cases, case I (left) and case II (right), where the data is respectively generated with \xw{from} the confounding graph (Figure~??) and the mediation graph (Figure~??).}
    \label{fig.samplesize-binnumber}
\end{figure*}

\begin{figure*}[t]
     \centering
    \includegraphics[width=\textwidth]{icml24_figs/cmp_baselines.pdf}
    \caption{Comparison between our method and baselines under different sample sizes.\xw{Type-I and Type-II error rates of our procedure and baselines.} For a good \xw{valid} testing method, the type I error should be close to the significant level $\alpha$ (the dashed line), and the type II error should be as small as possible \xw{close to 0}.}
    \label{fig.cmp-baselines}
\end{figure*}

\subsection{Application in causal discovery}

% there are two important points
% 1. connection between ci-test and causal identification: markov & faithfulness, x-y is both marginal and conditional correlated (given U); U is sufficient confounder (health), we assume U can be partially measure (with error) by a proxy variable W
% 2. briefly introduce the sepsis diease, and why identify the causal relation between the two pairs of variables are important

In this section, we apply the proposed test to a real-world causal discovery task. We consider the sepsis disease \xw{we apply our procedure to causal relations identification in the sepsis disease}, which is a systemic inflammatory response to infection \cite{matot2001definition} and the leading cause of death in the Intensive Care Unit (ICU) \cite{o2007sepsis}. 

For sepsis disease \xw{Specifically}, we examine two pairs of causal relationships: $\text{Vancomycin}\to \text{White Blood Cell count (WBC)}$ and $\text{Morphine}\to \text{WBC}$. Vancomycin and morphine are two common medications for sepsis, with vancomycin being used to control bacterial infection \cite{moellering2006vancomycin} and morphine being used for pain management \cite{mcquay1999opioids}, and the WBC is a common biomarker used to evaluate patient's responses to medications \cite{castelli2006procalcitonin}. 

For \xw{In} both cases \xw{pairs}, we assume that \xw{it is believed that the confounder is accounted for by } the patient's health status ($U$) is a sufficient confounder between the cause-effect pair \xw{in the pair or between the cause and the effect}, which can be measured with error by the proxy variable blood pressure ($W$). In this regard \xw{delete}, assuming \xw{under} the Markov and causal faithfulness assumptions \cite{pearl2009causality}, we have the causal relation exists (or does not exist) if the null hypothesis $\mathbb{H}_0:X\ind Y|U$ is rejected (or accepted).

\textbf{Golden standards from RCTs.} We consider \xw{take} results from two Random Controlled Trials (RCTs) to be \xw{as} the golden standard for causal discovery. Specifically, \cite{rosini2015randomized} showed \xw{found} that vancomycin can causally influence the WBC; while \cite{anand2004effects} showed \xw{found} that morphine has no causal effect on WBC. In other words, the correlation between morphine usage and an increase in WBC (as found in \cite{zhang2018prescription}) is likely due to confounding bias.

\textbf{Data extraction from MIMIC.} We consider the Medical Information Mart for Intensive Care (MIMIC III) database \cite{johnson2016mimic}, which contains the electronic health records for patients in the ICU. From MIMIC III, we extracted data for 3251 \xw{3,251} patients diagnosed with sepsis during their ICU stays. Among these patients, 1888 \xw{1,888} individuals received vancomycin, and 559 individuals received morphine.

\textbf{Results analysis.} We report the identified causal relationships using our test and baseline methods \xw{other procedures} in Table~\ref{tab.sepsis}. Results that are inconsistent with the golden standard are highlighted in red. As we can see, the proposed test identifies causal relations that well align with the RCT results in both cases, which demonstrate the effectiveness and utility of our method. In contrast, there is a large discrepancy between the results of the baseline methods and the RCTs. For instance, the KCI and ICM methods both detect that morphine has a causal influence on WBC, which could be a false positive result due to the failure to adjust the confounding bias; the Miao method falsely concludes \xw{fails to reject the null hypothesis} that vancomycin has no causal effect on WBC, which may be attributed to the loss of power in the proxy variable \xw{I do not understand this explanation. The discretization error may increase the power?} without careful discretization.

\begin{figure}[t]
    \centering
    \includegraphics[width=.4\textwidth]{icml24_figs/sepsis_causalgraph.pdf}
    \caption{Applying the proposed test to causal discovery for sepsis disease. \xw{Illustration of the causal structure in the sepsis disease.} Observable variables are marked in gray. WBC denotes the count of White Blood Cells, which is a common biomarker used to assess the patient's responses to medicines. By using blood pressure as the proxy variable for health status, we can determine whether the edge $\mathrm{Medicine} \,-\!\!\to \mathrm{WBC}$ exists. \xw{This graph does not show you ``can" determine something. It is more precise to say ``our goal is to"}}
    \label{fig.sepsis}
\end{figure}


\begin{table}[t]
\caption{Identified causal relationships in sepsis disease. We use results from Random Controlled Trials (RCTs) \cite{anand2004effects,rosini2015randomized} as the golden standard. Results that contradict the golden standard are marked in red.}
\label{tab.sepsis}
\begin{center}
\resizebox{.48\textwidth}{!}{
\begin{tabular}{lccc}
\toprule
Method & Vancomycin$\to $WBC & Morphine$\to$ WBC \\
\midrule
RCT (gold. stand.)    & $\surd$ &  $\times$  \\
KCI & $\surd$ & \textcolor{red}{$\surd$}  \\
ICM  & $\surd$ & \textcolor{red}{$\surd$} \\
Miao    & \textcolor{red}{$\times$} &   \textcolor{red}{$\surd$} \\
Ours   & $\surd$ &  $\times$   \\
\bottomrule
\end{tabular}}
\end{center}
\end{table}


==> icml24_para/mz_v1/introduction.tex <==
\clearpage
\section{Introduction}

Causal discovery is becoming an increasingly popular topic in machine learning, as the result of which has been shown to be indispensable for designing robust and transferable machine learning systems \cite{scholkopf2021toward,anonymous2024robust}. While the golden standard for causal discovery remains randomized controlled trials (RCTs), it can be too expensive, unethical, or even impossible to conduct in the real world. For this reason, the ability of identifying causal relationships from purely observational data is desired. 


However, a significant obstacle when attempting to draw casual conclusions from observational data is the problem of \emph{unobserved confounders}: factors that affect both the cause variable and the effect variable at the same time, but are hard to quantify in the observation. Usually, these factors describe the intrinsic characteristics of the studied system (e.g. health status, gene), and ignoring them can lead to non-vanishing bias for causal discovery, even with an infinite number of samples \cite{pearl2009causality}.


==> icml24_para/mz_v1/preliminary.tex <==
\section{Preliminary}

In this section, we introduce the preliminary notations and backgrounds needed to understand our work.

\textbf{Notations.} Throughout the paper, $X,Y,$ and $U$ are random variables, with domains $\mathcal{X},\mathcal{Y},$ and $\mathcal{U}$, respectively. The probability law of $X$ is denoted as $\mathcal{L}_X$, and similarly for the joint law $\mathcal{L}_{X Y}$ and the conditional law $\mathcal{L}_{X|Y}$. For discrete variables $X$ and $Y$ with respectively $I$ and $J$ levels, we use the column vector $P(X|y):=[\mathrm{pr}(x_1|y),...,\mathrm{pr}(x_I|y)]^T$, the row vector $P(x|Y):=[\mathrm{pr}(x|y_1),...,\mathrm{pr}(x|y_J)]$, and the matrix $P(X|Y):=[P(X|y_1),...,P(X|y_J)]$ to represent the conditional distribution $\mathcal{L}_{X|Y}$. For the continuous case, we assume all domains are intervals or the real line. We denote $\{\mathcal{X}_i\}_I$ a partition of $\mathcal{X}$ with $I$ subintervals, satisfying that $\cup_i^I \mathcal{X}_i=\mathcal{X}$ and $\mathcal{X}_i \cap \mathcal{X}_j =\emptyset$ for $i\neq j$. We thereby define the discretized version of $X$ as $\tilde{X}$, by assigning $\tilde{X}$ to $\tilde{x}_i$ iff $X\in\mathcal{X}_i$. We use $n$ to denote the sample size.

The problem we consider here is to identify whether $X$ has a causal inference on $Y$, in the presence of an unobserved, sufficient confounder $U$. Under the Markovian and faithfulness assumptions \cite{pearl2009causality}, this is equivalent to the problem of testing the causal null hypothesis $\mathbb{H}_0: X\ind Y|U$. The $\mathbb{H}_0$ means there is no causal influence from $X$ to $Y$, and a rejection of $\mathbb{H}_0$ is the evidence in favor of causation.

\textbf{Proxy variable} \cite{kuroki2014measurement} \textbf{.} To test $\mathbb{H}_0$ under the unobserveness of $U$, we assume the availability of a proxy variable $W$ of $U$ satisfying $X\ind W|U$ (Figure~\ref{fig.proxy}). In practice, the proxy variable can be a noisy measurement \cite{kuroki2014measurement} or an observed descendant \cite{liu2023causal} of the unobserved confounder.

\begin{remark}
    Note that the proposed procedure in this paper can apply to cases with a single or multiple proxies. We illustrate with the single-proxy case because it is the most challenging one.
\end{remark}

\begin{figure}[t]
    \centering
    \includegraphics[width=.2\textwidth]{icml24_figs/proxy.pdf}
    \caption{A causal diagram illustrating the proxy variable setting. Note that the proposed procedure is not restricted to this diagram, but can apply to any scenario satisfying $X\ind W|U$.}
    \label{fig.proxy}
\end{figure}

\textbf{Proxy-based characterization of} $\mathbb{H}_0$ \textbf{.} For discrete data, the work of \cite{miao2018identifying} (Section~4) provided a characterization of the null hypothesis $\mathbb{H}_0$ based on the proxy variable $W$. In details, they connected $\mathbb{H}_0$ with the following system of linear equations:
\begin{equation}
    \underbrace{P(y|X)^T}_{\text{response}} = \underbrace{P(W|X)^T}_{\text{design matrix}} \{\underbrace{P(y|U) P(W|U)^{-1}}_{\text{coefficient}}\}^T, \label{eq.miao}
\end{equation}
by noticing that
\begin{align*}
    P(y|X) &= P(y|U) P(U|X), \quad \# \, \mathbb{H}_0:X\ind Y|U\\ 
    P(W|X) &= P(W|U) P(U|X). \quad \# \, X\ind W|U
\end{align*}

In this regard, the problem of testing $\mathbb{H}_0$ is equivalent to that of identifying the system~(\ref{eq.miao}). Given that the matrices $P(W|U)$ and $P(W|X)$ are both full ranks, they showed that system~(\ref{eq.miao}) is identifiable, and hence $\mathbb{H}_0$ is testable.

However, for continuous data, it remains unknown whether such a connection can be built, considering the facts that the conditional independence $\tilde{X}\ind \tilde{W}|\tilde{U}$ may not hold, and that the matrix $P(\tilde{W}|\tilde{U})$ could be singular (see Figure~\ref{fig.introduction}). In the subsequent section, we will provide a comprehensive analysis to answer this question.


\begin{figure}[t]
    \centering
    \includegraphics[width=.4\textwidth]{icml24_figs/introduction.pdf}
    \caption{Top: conditional independence between continuous variables $X\ind W|U$ does not necessarily implies that between discrete ones $\tilde{X}\ind\tilde{W}|\tilde{U}$. Bottom: an example in which the conditional probability matrix $P(\tilde{W}|\tilde{U})$ is singular.}
    \label{fig.introduction}
\end{figure}

==> icml24_para/mz_v1/test.tex <==
\section{Hypothesis test}

In this section, we introduce a hypothesis testing procedure based on the characterization of $\mathbb{H}_0$ discussed in Section~\ref{sec.dis-theory}.


\subsection{Test statistic}

To this end, we first introduce a test statistic that reflects the property of the null hypothesis $\mathbb{H}_0$. According to the analysis in Section~\ref{sec.dis-theory}, when the null hypothesis is true, the system described by (\ref{eq.ours}) is identifiable. Therefore, we can design a test statistic for $\mathbb{H}_0$ by looking at the identifiability of the system (\ref{eq.ours}). 

Particularly, we note that the identifiability of the linear system can be reflected by the squared residual of regressing $P(\tilde{y}|\tilde{X})$ on $P(\tilde{W}|\tilde{X})$. When the null hypothesis is true, the linear system is identifiable, and therefore the squared residual is small. Moreover, to enhance the power of the test statistic, we can aggregate together the square residuals obtained from the regressing of each level of $\tilde{Y}$. 

Formally, denote $q^T:=[P(\tilde{y}_1|\tilde{X}),...,P(\tilde{y}_{J-1}|\tilde{X})]$ as the vector that aggregates $P(\tilde{y}|\tilde{X})$ for all levels of $\tilde{Y}$, and denote $Q:=\mathrm{diag}[P(\tilde{W}|\tilde{X}),...,P(\tilde{W}|\tilde{X})]$ as the block diagonal matrix with $(J-1)$ blocks of $P(\tilde{W}|\tilde{X})$ in the diagonal. Suppose that we have available estimators $\hat{q}$ and $\hat{Q}$\footnote{We adopt the Maximum Likelihood Estimation (MLE) to obtain $\hat{q}$ and $\hat{Q}$. Please refer to Appendix~\ref{app-sec.mle} for details.} satisfying that:
\begin{align*}
    n^{1/2}(\hat{q} - q) &\to N(0,\Sigma) \,\, \text{in distribution}, \\
    \hat{Q}\to Q, \hat{\Sigma} &\to \Sigma \,\, \text{in probability,} 
\end{align*}
with $\hat{\Sigma}, \Sigma$ both positive definite. Denote the least square residual of regressing $\hat{\Sigma}^{-1/2} \hat{q}$ on $\hat{\Sigma}^{-1/2} \hat{Q}$ as:
\begin{equation*}
    \hat{\xi} := \{\mathrm{I} - \hat{\Sigma}^{-1/2} \hat{Q}^T (\hat{Q} \hat{\Sigma}^{-1} \hat{Q}^T)^{-1} \hat{Q} \hat{\Sigma}^{-1/2}\} \hat{\Sigma}^{-1/2} \hat{q},
\end{equation*}
where $\mathrm{I}$ denotes the identity matrix. 

Then, we define the squared least residual $T:=n^{1/2}\xi^T \xi$ as our test statistics and denote the corresponding estimator as $\hat{T}:=n^{1/2}\hat{\xi}^T \hat{\xi}$.

\subsection{Type I and type II error control}

In this section, we proceed to show the distribution of the test statistic and analyze the asymptotic behaviours of the testing procedure.

Particularly, we first show that under $H_0$, the test statistic $\hat{T}$ we define follows a chi-square distribution $\chi^2_k$, where the freedom $k=(l_{\tilde{X}}-l_{\tilde{W}})(l_{\tilde{Y}}-1)$ is the free dimensions that $\tilde{X}$ has beyond $\tilde{W}$ (aggregated with levels of $\tilde{Y}$). Intuitively, this means we use the first $l_{\tilde{W}}$ dimensions of equation~(\ref{eq.ours}) to fit a solution, then test whether this solution is unique on the rest $(l_{\tilde{X}}-l_{\tilde{W}})$ dimensions of the equation.

In this regard, given a significance level $\alpha$, let $z_{1-\alpha}$ be the $(1-\alpha)$-quantile of $\chi^2_k$, we define our testing procedure as:
\begin{equation*}
    \Psi_{n,N} = \Psi_{n,N}^\alpha = \mathbbm{1}(\hat{T}_{n,N}>z_{1-\alpha})
\end{equation*}
where $n$ is the sample size and $N$ is the bin levels.

Based on the analysis from Propositions~\ref{prop.control-err}-\ref{prop.rank-dis}, we can now deduce the asymptotic properties of our testing procedure under the null hypothesis $H_0$. Specifically:

\begin{theorem}
    Suppose that Assumptions~\ref{asm.tv-smooth}-\ref{asm.comp} and the condition in Proposition~\ref{prop.dis-err unbd} hold, then under $H_0$, it holds that:
    \begin{equation*}
        \hat{T}_{n,N} \to \chi_{k}^2 \,\, \text{in distribution}
    \end{equation*}
    as $n,N\to \infty$. As a consequence, for any $\alpha\in (0,1)$,
    \begin{equation*}
        \lim_{n,N\to \infty} \mathbb{P}(\Psi_{n,N}^\alpha=1) = \alpha
    \end{equation*}
    In other words, the testing procedure we define has uniform asymptotic level $\alpha$.
\label{thm.control.type-i}
\end{theorem}


In general, we can not expect the testing procedure has power against the alternative $H_1 :X\not \ind Y|U$, without further restriction on the alternative distribution. This is analogous to other conditional independence tests, such as \cite{zhang2012kernel,runge2018conditional,christgau2023nonparametric}, that were used for causal discovery.

Nonetheless, as shown below, we can establish power against the local alternative in which the integral equation $f(y|x)=\int h(y,w)f(w|x)dw$ has no smooth solution. Intuitively, this condition means the influence from $X$ to $Y$ can not be (totally) explained by the that between $X,U$ and $U,Y$. Under this condition, the square residual obtained from regressing the linear system becomes large, leading to a deviation of the test statistic from zero. Heuristic studies show that this condition applies when the causal influence from $X$ to $Y$ is strong (Please refer to Appendix~\ref{sec.example-integral-eq} for details).

Formally, denote $\mathbb{C}(\mathcal{W},\mathcal{Y})$ the set of almost surely continuous functions over $\mathcal{W}\times \mathcal{Y}$. For $h\in \mathbb{C}(\mathcal{W},\mathcal{Y})$, let the averaged residual of fitting the integral equation $f_\theta(y|x)=\int h(y,w)f_\theta(w|x)dw$ be $\mathrm{res}_\theta:=\iint |f_\theta(y|x)-\int h(y,w)f_\theta(w|x)dw|dy f_\theta(x) dx$. Let $\Theta:=\{\theta: \exists\epsilon_0>0, \min_{h\in \mathbb{C}(\mathcal{W},\mathcal{Y})} \mathrm{res}_\theta>\epsilon_0\}$ be the set of alternative models in which the integral equation has no solution. Then, we have the following result:

\begin{theorem}
    Suppose that Assumptions~\ref{asm.tv-smooth}, \ref{asm.comp} and the conditions in Proposition~\ref{prop.dis-err unbd} hold, then for any $0<\alpha<1$, it holds that:
    \begin{equation*}
        \lim_{n,N\to\infty}\mathbb{P}_{\Theta}(\Psi_{n,N}^\alpha)=0
    \end{equation*}
    In other words, the probability of making a type II error can be controlled to zero asymptotically.
    \label{thm.type-ii}
\end{theorem}


==> icml24_para/mz_v1/theory.tex <==
% todo (problems)
% 1. partition of X,Y,U,W, and define the discretized variable X,Y,U,W
%    define that level(U)=level(W) => this should be done in sec.outline
% 2. moreover, for sec.outline, our objective at sec.dis and sec.comp should be more clearified;
%    P(W|U) has full row rank means the rows of P(W|U) are linear independent, in other workds, W has enough variability (dimensions) to reflect that of U; put this into the analysis of sec.outline
% 3. examples or characterization of assumptions should follow directly after it, as in Warren and Miao; you should also cite some paper to show this assumption has been used before
% 2. discuss the practical method to decide the bin number => where should this be done, sec.dis-err, sec.implementation-details, or sec.conclusion-discussion ??
% 3. add "note that we do not need to discretize U", but where ??
% 4. need to put more words on why p(w|u), p(w|x) has full rank means system is identifiable

% Except for the above problems, I think many points of sec.preliminary and sec.dis-theory need 细化讨论


% this section should be re-organized as follow
% Discretization theories
% - outline
% - regularity conditions -> tv-smooth, tightness, completeness
% - examples of conditions
% - algorithm

\section{Discretization theory}
\label{sec.dis-theory}

In this section, we introduce a discretization-based strategy to characterize $\mathbb{H}_0$ under continuous data. Before proceeding technical details, we first outline our idea below.

\subsection{Outline}
\label{sec.outline}

The general idea is to first discretize the continuous variables $X$, $Y$, and $W$ into their discrete counterparts $\tilde{X}$, $\tilde{Y}$, and $\tilde{W}$, and then link $\mathbb{H}_0$ to the identification of the following system of linear equations:
\begin{equation}
P(\tilde{y}|\tilde{X})^T = P(\tilde{W}|\tilde{X})^T \{P(\tilde{y}|\tilde{U}) P(\tilde{W}|\tilde{U})^{-1}\}^T,
\label{eq.ours}
\end{equation}

To achieve this, in Section~\ref{sec.regularity}, we investigate the regularity conditions that allow for the linking. First, we establish the conditions under which the conditional independence ${X} \ind Y|U$ and $X \ind {W}|{U}$ can be maintained, which is crucial for establishing the relationships $P(\tilde{y}|\tilde{X}) = P(\tilde{y}|\tilde{U}) P(\tilde{U}|\tilde{X})$ and $P(\tilde{W}|\tilde{X}) = P(\tilde{W}|\tilde{U}) P(\tilde{U}|\tilde{X})$. Then, we show the conditions under which the matrices $P(\tilde{W}|\tilde{U})$ and $P(\tilde{W}|\tilde{X})$ can have independent rows, leading to the identifiability of the system described in (\ref{eq.ours}).

To illustrate the identified conditions, in Section~\ref{sec.example}, we provide examples based on the causal Addictive Noise Model (ANM). We show that our conditions are moderate and can be met by commonly used structural functions and exogenous distributions. 

Finally, in Section~\ref{sec.alg}, inspired by the theoretical results, we introduce a discretization algorithm that practically establishes the linking.

\subsection{Regularity conditions}
\label{sec.regularity}

In this section, we identify regularity conditions that allow for the linking between $\mathbb{H}_0$ and the system (\ref{eq.ours}). 

We first discuss the maintaining of the conditional independence structures $X\ind Y|U$ and $X\ind W|U$. Particularly, we establish conditions to control the distance between the vectors $P(\tilde{y}|\tilde{U})$ and $P(\tilde{y}|\tilde{x},\tilde{U})$ (and similarly for the matrix $P(\tilde{W}|\tilde{U})$ and $P(\tilde{W}|\tilde{x},\tilde{U})$) obtained after discretization. In this regard, we have the equations:
\begin{align}
    P(\tilde{y}|\tilde{X})&=P(\tilde{y}|\tilde{U}) P(\tilde{U}|\tilde{X}) + E_y, \label{eq.dis-ind-1}\\
    P(\tilde{W}|\tilde{X})&=P(\tilde{W}|\tilde{U}) P(\tilde{U}|\tilde{X}) + E_w, \label{eq.dis-ind-2}
\end{align}
with the error terms $E_y$ and $E_w$ controlled to zero asymptotically. 

Taking the control of $|P(\tilde{y}|\tilde{U})-P(\tilde{y}|\tilde{x},\tilde{U})|$ as an example, to achieve this, we require the map $u\mapsto \mathcal{L}_{Y|U=u}$ to change smoothly with respect to $u$. In this regard, for a small bin $\mathcal{U}_k$ and any $u\in\mathcal{U}_k$, the distributions $\mathcal{L}_{Y|U\in \mathcal{U}_k}$ and $\mathcal{L}_{Y|U=u}$ are close (and similarly for the distributions $\mathcal{L}_{Y|X\in\mathcal{X}_i,U\in \mathcal{U}_k}$ and $\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u}$). Since we have $\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u}=\mathcal{L}_{Y|U=u}$ under $X\ind Y|U$, using the triangle inequity, we have the closeness of the distributions $\mathcal{L}_{Y|U\in \mathcal{U}_k}$ and $\mathcal{L}_{Y|X\in\mathcal{X}_i,U\in \mathcal{U}_k}$, and therefore the control of $|P(\tilde{y}|\tilde{U})-P(\tilde{y}|\tilde{x},\tilde{U})|$.

Formally, we assume the following smoothness condition defined with the Total Variation (TV) distance between distributions:

\begin{assumption}[TV smoothness]
    We assume the map $u\mapsto \mathcal{L}_{Y|U=u}$ is $L_Y$-Lipschitz continuous with respect to TV distance, that is, for any $u,u^\prime \in \mathcal{U}$, we require $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime}) \leq L_Y|u-u^\prime|$. We also assume the map $u\mapsto \mathcal{L}_{W|U=u}$ is $L_W$-Lipschitz continuous.
\label{asm.tv-smooth}
\end{assumption}

\begin{remark}
    To be precise, what is meant here is that given a \emph{regular conditional distribution} $\mathcal{L}_{Y|U=u}$, one can modify it on a set of measure zero so that the Lipschitz condition is satisfied. Please refer to Appendix~\ref{sec.regular-prob} for details.
\end{remark}

Under Assumption~\ref{asm.tv-smooth}, we formalize our control strategy in the following proposition:

\begin{proposition}
    Suppose Assumption~\ref{asm.tv-smooth} holds. Then, for any $\epsilon>0$, as long as $len(\mathcal{U}_k)\leq min\{\epsilon/2L_Y,\epsilon/2L_W\}$, we have $|\mathrm{pr}(\tilde{y}|\tilde{u}_k)-\mathrm{pr}(\tilde{y}|\tilde{x},\tilde{u}_k)|\leq \epsilon$ under $X\ind Y|U$ and $|\mathrm{pr}(\tilde{w}|\tilde{u}_k)-\mathrm{pr}(\tilde{w}|\tilde{x},\tilde{u}_k)|\leq \epsilon$ under $X\ind W|U$.
\label{prop.control-err}
\end{proposition}

Equipped with Proposition~\ref{prop.control-err}, for cases where $\mathcal{U}$ is a compact interval, we can partition $\mathcal{U}$ into sufficiently refined bins. As long as the the lengths of the bins are small, we can effectively control the distances $|P(\tilde{y}|\tilde{U})-P(\tilde{y}|\tilde{x},\tilde{U})|$ and $|P(\tilde{W}|\tilde{U})-P(\tilde{W}|\tilde{x},\tilde{U})|$.

For non-compact domains, we further assume that the distribution $\mathcal{L}_{U|X}$ is tight, meaning that for large values of $u$, the conditional probability $\mathrm{pr}(u|x)$ is small. In this regard, we can divide $\mathcal{U}$ into a compact part $\mathcal{U}_c$ and a non-compact part $\mathcal{U}_{nc}$. Proposition~\ref{prop.control-err} continues to apply for the compact part, while for the non-compact part, we can control $\mathrm{pr}(\tilde{u}_{nc}|\tilde{x})$ to be small. By combining these two parts, we can still maintain equations (\ref{eq.dis-ind-1})-(\ref{eq.dis-ind-2}), whereas the error term now contains one part from $\mathcal{U}_c$ and another one from $\mathcal{U}_{nc}$.

To formalize the intuition above, we first introduce the definition of a tight distribution.

\begin{definition}[Tight distribution] The marginal distribution $\mathcal{L}_U$ is tight if $\forall \epsilon>0, \exists T, \forall t\geq T,\mathcal{L}(|U|\geq t)\leq \epsilon$. The conditional distribution $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$ if $\forall \epsilon>0, \exists T, \forall t\geq T, \forall x\in [a,b],\mathcal{L}(|U|\geq t|x)\leq \epsilon$.
\label{def.tight}
\end{definition}

\begin{remark}
    We use the term ``uniform'' because the $T$ holds uniformly for all $x\in[a,b]$. As we will show later, the uniform tightness is a mild condition (though one can image that uniform tightness for all $x\in \mathbb{R}$ is a strong one).
\end{remark}

With the above of tightness of distribution, we now introduce the following proposition to work with the non-compact domain:

\begin{proposition}
    Suppose that $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$, and that the map $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz continuous wrt TV distance. Then, partition the interval $[a,b]$ into $I$ bins $\{\mathcal{X}_i\}_I$ such that $len(\mathcal{X}_i)\leq \epsilon/2L_U$, $\forall\epsilon>0, \exists T$, let $\mathcal{U}_{nc}:=\{u:|u|\geq T\}$, we have $\mathrm{pr}(\tilde{u}_{nc}|\tilde{x}_i) \leq \epsilon$.
    \label{prop.dis-err unbd}
\end{proposition}

Having shown the preservation of the conditional independent structures, in the following, we discuss the identifiability of the system described by (\ref{eq.ours}). 

As mentioned before, this requires that the discretization process yields conditional probability matrices $P(\tilde{W}|\tilde{U})$ and $P(\tilde{W}|\tilde{X})$ with full row rank. To assure such a discretization process exists, we need the following completeness assumption:

\begin{assumption}[Completeness]
    We assume the conditional distribution $\mathcal{L}_{W|U}$ is bounded complete. That is, for any bounded function $g$, $E[g(w)|u]=0$ almost surely iff $g(w)=0$ almost surely. We also assume that $\mathcal{L}_{W|X}$ is bounded complete.
    \label{asm.comp}
\end{assumption}

The completeness condition has been widely used in semiparametric and nonparametric models for identifiability. Intuitively, the completeness of $\mathcal{L}_{W|U}$ means $W$ exhibits sufficient variability to full reflect the information from $U$. Therefore, it is no wonder that under the completeness condition, there always exists a discretization process that can produce conditional probability matrices with full rank. Specifically, we have the following result:

\begin{proposition}
    Suppose Assumption~\ref{asm.comp} holds. Then, for any discretization $\tilde{W}$ of $W$, there exists a discretization $\tilde{U}$ of $U$ such that the matrix $P(\tilde{W}|\tilde{U})$ is invertible. Similarly, there also exists a discretization $\tilde{X}$ of $X$ such that the matrix $P(\tilde{W}|\tilde{X})$ has full row rank.
    \label{prop.rank-dis}
\end{proposition}


\subsection{Examples}
\label{sec.example}

In this section, we provide examples for characterizing the conditions in Section~\ref{sec.regularity}. Specifically, consider the following causal Addictive Noise Model (ANM):
\begin{equation*}
    V = g_V(U) + N_V, \,\, \text{for} \,\, V \in \{X,Y,W\},
\end{equation*}
where $g_V$ is the structural function and $N_V\sim f_V$ is the exogenous noise. Then, we have the following results:

\begin{example}[ANM with TV smoothness]
    Suppose that the structural functions $g_Y$ and $g_W$ are differentiable, and that the pdfs $f_Y$ and $f_W$ of the exogenous distributions have absolutely integrable derivatives, then the TV smoothness conditions in Assumption~\ref{asm.tv-smooth} hold.
\end{example}

\begin{example}[ANM with tightness]
    Suppose that the structural functions $g_X$ is invertible, and that the distribution of $N_X$ is tight (see Definition~\ref{def.tight}), then the uniform tightness condition in Proposition~\ref{prop.dis-err unbd} holds for arbitrary compact interval $[a,b]$.
\end{example}

\begin{example}[ANM with completeness]
    Suppose that the structural functions $g_X$ is invertible with a non-zero derivative, and that the exogenous noises $N_X$ and $N_W$ both have non-zero characterization functions, then the completeness conditions in Assumption~\ref{asm.comp} holds.
\end{example}

To summarize, for causal ANMs, the major sufficient conditions for regularities in Section~\ref{sec.regularity} are: \textbf{i)} the differentiability and invertibility of structural functions, and \textbf{ii)} the tightness of the exogenous distributions and the non-vanishing of their characterization functions. These conditions are mild, with the former satisfied by common analytic functions, and the latter satisfied by, for example, the exponential family of distributions.


\subsection{Algorithm}
\label{sec.alg}

In this section, we introduce an Algorithm~\ref{alg.dis} to practically find a discretization satisfying the properties in Section~\ref{sec.outline}.

Specifically, given $n$ iid samples, we first set the bin numbers for $Y$ and $W$ to $\left\lfloor \log n \right\rfloor$, according to the heuristic rule suggested in \cite{dougherty1995supervised}. Then, we adopt uniform binning to generate data for $\tilde{Y}$ and $\tilde{W}$. 

Next, to generate $\tilde{X}$ satisfying $P(\tilde{W}|\tilde{X})$ being full row rank, we propose an iterative searching strategy. In each step of the search, we generate a new partition point $x_i$ of the domain $\mathcal{X}$ such that the vectors $P(X\leq x_1|\tilde{W}), ..., P(X\leq x_i|\tilde{W})$ are linear independent. We set the total number of bins for $X$ to be larger than that of $W$, in order to make sure $P(\tilde{W}|\tilde{X})$ contains more columns than rows. Finally, we consider an \emph{implicit} binning of the unobserved confounder $U$, which can maintain the conditional independence $X\perp Y|U$ and $X\ind W|U$, as well as the invertibility of $P(\tilde{W}|\tilde{U})$. Thanks to Proposition~\ref{prop.control-err} and Proposition~\ref{prop.rank-dis}, such an implicit binning always exists.

For Algorithm~\ref{alg.dis}, let $[i]$ be the index set $\{1,...,i\}$ and let $[i]\backslash j$ be the set obtained by removing $j$ from $[i]$. We use $x_{[i]}$ in short for $[x_1,...,x_i]^T$. $F(x|\tilde{w})$ is the conditional cdf of $X$ given $\tilde{W}=\tilde{w}$. We use the notations $F(x|\tilde{w}_{[i]}):=[F(x|\tilde{w}_1),...,F(x|\tilde{w}_i)]^T$ and $F(x_{[i]}|\tilde{w}_{[i]}):=[F(x_1|\tilde{w}_{[i]}),...,F(x_i|\tilde{w}_{[i]})]$ for convention. $\mathrm{det}(M)$ is the determinant of the matrix $M$.

\begin{algorithm}[t]
   \caption{Discretization}
   \label{alg.dis}
\begin{flushleft}
\textbf{Input:} Continuous observation of $X$, $Y$, $W$. \\
\textbf{Output:} Discrete data for $\tilde{X}$, $\tilde{Y}$, $\tilde{W}$.
\end{flushleft}
\begin{algorithmic}[1]
    \STATE Uniformly bin $Y,W$ to obtain $\tilde{Y}$, $\tilde{W}$.
    \FOR{$i=1:N$}
        \FOR{$j=1:i$}
            \STATE Estimate $d_j=\mathrm{det}(F(x_{[i-1]}|\tilde{w}_{[i]\backslash j}))$
        \ENDFOR
        \STATE Search $x_i$ s.t. $\sum_{j=1}^i (-1)^{1+j} d_j F(x_i|\tilde{w}_j) \neq 0$.
    \ENDFOR
    \STATE Bin $X$ with the partition $\{[x_i,x_{i+1}]\}_i^N$ to obtain $\tilde{X}$.
    \STATE \textbf{return} $\tilde{X}$, $\tilde{Y}$, $\tilde{W}$.
\end{algorithmic}
\end{algorithm}

==> icml24_para/mz_v1/theory_comment.tex <==
% todo (problems)
% 1. partition of X,Y,U,W, and define the discretized variable X,Y,U,W
%    define that level(U)=level(W) => this should be done in sec.outline
% 2. moreover, for sec.outline, our objective at sec.dis and sec.comp should be more clearified;
%    P(W|U) has full row rank means the rows of P(W|U) are linear independent, in other workds, W has enough variability (dimensions) to reflect that of U; put this into the analysis of sec.outline
% 3. examples or characterization of assumptions should follow directly after it, as in Warren and Miao; you should also cite some paper to show this assumption has been used before
% 2. discuss the practical method to decide the bin number => where should this be done, sec.dis-err, sec.implementation-details, or sec.conclusion-discussion ??
% 3. add "note that we do not need to discretize U", but where ??


% this section should be re-organized as follow
% Discretization theories
% - outline
% - regularity conditions -> tv-smooth, tightness, completeness
% - examples of conditions
% - algorithm

\section{Discretization theory}

In this section, we introduce a discretization-based strategy to characterize $\mathbb{H}_0$ under continuous data. Before proceeding with technical details, we first outline our idea below.

\subsection{Outline}
\label{sec.outline}

The general idea is to first discretize the continuous variables $X$, $Y$, and $W$ into their discrete counterparts $\tilde{X}$, $\tilde{Y}$, and $\tilde{W}$, and then link $\mathbb{H}_0$ to the identification of the following system of linear equations: 
\begin{equation}
P(\tilde{y}|\tilde{X})^T = P(\tilde{W}|\tilde{X})^T \{P(\tilde{y}|\tilde{U}) P(\tilde{W}|\tilde{U})^{-1}\}^T,
\label{eq.ours}
\end{equation}
\xw{directly cite Eq.~\eqref{eq.miao}?}

To achieve this, in Section~\ref{sec.regularity}, we investigate the regularity conditions that allow for the linking. First, we establish the conditions under which the conditional independence ${X} \ind Y|U$ and $X \ind {W}|{U}$ can be maintained, which is crucial for establishing the relationships $P(\tilde{y}|\tilde{X}) = P(\tilde{y}|\tilde{U}) P(\tilde{U}|\tilde{X})$ and $P(\tilde{W}|\tilde{X}) = P(\tilde{W}|\tilde{U}) P(\tilde{U}|\tilde{X})$. Then, we show the conditions under which the matrices $P(\tilde{W}|\tilde{U})$ and $P(\tilde{W}|\tilde{X})$ can have independent rows, leading to the identifiability of the system described in (\ref{eq.ours}).

To illustrate the identified conditions, in Section~\ref{sec.example}, we provide examples based on the causal Addictive Noise Model (ANM). We show that our conditions are moderate and can be met by commonly used structural functions and exogenous distributions. 

Finally, in Section~\ref{sec.alg}, inspired by the theoretical results, we introduce a discretization algorithm that practically establishes the linking.

\subsection{Regularity conditions}
\label{sec.regularity}

In this section, we identify regularity conditions that allow for the linking between $\mathbb{H}_0$ and the system (\ref{eq.ours}). 

We first discuss the maintaining of the conditional independence structures $X\ind Y|U$ and $X\ind W|U$. Particularly, we establish conditions to control the distance between the vectors $P(\tilde{y}|\tilde{U})$ and $P(\tilde{y}|\tilde{x},\tilde{U})$ (and similarly for the matrix $P(\tilde{W}|\tilde{U})$ and $P(\tilde{W}|\tilde{x},\tilde{U})$) obtained after discretization. In this regard, we have the equations:
\begin{align}
    P(\tilde{y}|\tilde{X})&=P(\tilde{y}|\tilde{U}) P(\tilde{U}|\tilde{X}) + E_y, \label{eq.dis-ind-1}\\
    P(\tilde{W}|\tilde{X})&=P(\tilde{W}|\tilde{U}) P(\tilde{U}|\tilde{X}) + E_w, \label{eq.dis-ind-2}
\end{align}
with the error terms $E_y$ and $E_w$ controlled to zero asymptotically. 

Taking the control of $|P(\tilde{y}|\tilde{U})-P(\tilde{y}|\tilde{x},\tilde{U})|$ as an example, to achieve this, we require the map $u\mapsto \mathcal{L}_{Y|U=u}$ to change smoothly with respect to $u$. In this regard, for a small bin $\mathcal{U}_k$ and any $u\in\mathcal{U}_k$, the distributions $\mathcal{L}_{Y|U\in \mathcal{U}_k}$ and $\mathcal{L}_{Y|U=u}$ are close (and similarly for the distributions $\mathcal{L}_{Y|X\in\mathcal{X}_i,U\in \mathcal{U}_k}$ and $\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u}$). Since we have $\mathcal{L}_{Y|X\in\mathcal{X}_i,U=u}=\mathcal{L}_{Y|U=u}$ under $X\ind Y|U$, using the triangle inequity, we have the closeness of the distributions $\mathcal{L}_{Y|U\in \mathcal{U}_k}$ and $\mathcal{L}_{Y|X\in\mathcal{X}_i,U\in \mathcal{U}_k}$, and therefore the control of $|P(\tilde{y}|\tilde{U})-P(\tilde{y}|\tilde{x},\tilde{U})|$.

Formally, we assume the following smoothness condition defined with the Total Variation (TV) distance between distributions:

\begin{assumption}[TV smoothness]
    We assume the map $u\mapsto \mathcal{L}_{Y|U=u}$ is $L_Y$-Lipschitz continuous with respect to TV distance, that is, for any $u,u^\prime \in \mathcal{U}$, we require $\mathrm{TV}(\mathcal{L}_{Y|U=u},\mathcal{L}_{Y|U=u^\prime}) \leq L_Y|u-u^\prime|$. We also assume the map $u\mapsto \mathcal{L}_{W|U=u}$ is $L_W$-Lipschitz continuous.
\label{asm.tv-smooth}
\end{assumption}

\begin{remark}
    To be precise, what is meant here is that given a \emph{regular conditional distribution} $\mathcal{L}_{Y|U=u}$, one can modify it on a set of measure zero so that the Lipschitz condition is satisfied. Please refer to Appendix~\ref{sec.regular-prob} for details.
\end{remark}

Under Assumption~\ref{asm.tv-smooth}, we formalize our control strategy in the following proposition:

\begin{proposition}
    Suppose Assumption~\ref{asm.tv-smooth} holds. Then, for any $\epsilon>0$, as long as $len(\mathcal{U}_k)\leq min\{\epsilon/2L_Y,\epsilon/2L_W\}$, we have $|\mathrm{pr}(\tilde{y}|\tilde{u}_k)-\mathrm{pr}(\tilde{y}|\tilde{x},\tilde{u}_k)|\leq \epsilon$ under $X\ind Y|U$ and $|\mathrm{pr}(\tilde{w}|\tilde{u}_k)-\mathrm{pr}(\tilde{w}|\tilde{x},\tilde{u}_k)|\leq \epsilon$ under $X\ind W|U$.
\label{prop.control-err}
\end{proposition}

Equipped with Proposition~\ref{prop.control-err}, for cases where $\mathcal{U}$ is a compact interval, we can partition $\mathcal{U}$ into sufficiently refined bins. As long as the the lengths of the bins are small, we can effectively control the distances $|P(\tilde{y}|\tilde{U})-P(\tilde{y}|\tilde{x},\tilde{U})|$ and $|P(\tilde{W}|\tilde{U})-P(\tilde{W}|\tilde{x},\tilde{U})|$.

For non-compact domains, we further assume that the distribution $\mathcal{L}_{U|X}$ is tight, meaning that for large values of $u$, the conditional probability $\mathrm{pr}(u|x)$ is small. In this regard, we can divide $\mathcal{U}$ into a compact part $\mathcal{U}_c$ and a non-compact part $\mathcal{U}_{nc}$. Proposition~\ref{prop.control-err} continues to apply for the compact part, while for the non-compact part, we can control $\mathrm{pr}(\tilde{u}_{nc}|\tilde{x})$ to be small. By combining these two parts, we can still maintain equations (\ref{eq.dis-ind-1})-(\ref{eq.dis-ind-2}), whereas the error term now contains one part from $\mathcal{U}_c$ and another one from $\mathcal{U}_{nc}$.

To formalize the intuition above, we first introduce the definition of a tight distribution.

\begin{definition}[Tight distribution] The marginal distribution $\mathcal{L}_U$ is tight if $\forall \epsilon>0, \exists T, \forall t\geq T,\mathcal{L}(|U|\geq t)\leq \epsilon$. The conditional distribution $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$ if $\forall \epsilon>0, \exists T, \forall t\geq T, \forall x\in [a,b],\mathcal{L}(|U|\geq t|x)\leq \epsilon$.
\label{def.tight}
\end{definition}

\begin{remark}
    We use the term ``uniform'' because the $T$ holds uniformly for all $x\in[a,b]$. As we will show later, the uniform tightness is a mild condition (though one can image that uniform tightness for all $x\in \mathbb{R}$ is a strong one).
\end{remark}

With the above of tightness of distribution, we now introduce the following proposition to work with the non-compact domain:

\begin{proposition}
    Suppose that $\mathcal{L}_{U|X}$ is uniformly tight in $[a,b]$, and that the map $x\mapsto\mathcal{L}_{U|X=x}$ is $L_U$-Lipschitz continuous wrt TV distance. Then, partition the interval $[a,b]$ into $I$ bins $\{\mathcal{X}_i\}_I$ such that $len(\mathcal{X}_i)\leq \epsilon/2L_U$, $\forall\epsilon>0, \exists T$, let $\mathcal{U}_{nc}:=\{u:|u|\geq T\}$, we have $\mathrm{pr}(\tilde{u}_{nc}|\tilde{x}_i) \leq \epsilon$.
    \label{prop.dis-err unbd}
\end{proposition}

Having shown the preservation of the conditional independent structures, in the following, we discuss the identifiability of the system described by (\ref{eq.ours}). 

As mentioned before, this requires that the discretization process yields conditional probability matrices $P(\tilde{W}|\tilde{U})$ and $P(\tilde{W}|\tilde{X})$ with full row rank. To assure such a discretization process exists, we need the following completeness assumption:

\begin{assumption}[Completeness]
    We assume the conditional distribution $\mathcal{L}_{W|U}$ is bounded complete. That is, for any bounded function $g$, $E[g(w)|u]=0$ almost surely iff $g(w)=0$ almost surely. We also assume that $\mathcal{L}_{W|X}$ is bounded complete. \xw{we also need the completeness for $P(U|X)$?}
    \label{asm.comp}
\end{assumption}

The completeness condition has been widely used in semiparametric and nonparametric models for identifiability \xw{the condition for $P(W|U)$ is firstly introduced by us?}. Intuitively, the completeness of $\mathcal{L}_{W|U}$ means $W$ exhibits sufficient variability to full reflect the information from $U$. Therefore, it is no wonder \xw{we should explain why we have this result with completeness} that under the completeness condition, there always exists a discretization process that can produce conditional probability matrices with full rank. Specifically, we have the following result:

\begin{proposition}
    Suppose Assumption~\ref{asm.comp} holds. Then, for any discretization $\tilde{W}$ of $W$, there exists a discretization $\tilde{U}$ of $U$ such that the matrix $P(\tilde{W}|\tilde{U})$ is invertible. Similarly, there also exists a discretization $\tilde{X}$ of $X$ such that the matrix $P(\tilde{W}|\tilde{X})$ has full row rank.
    \label{prop.rank-dis}
\end{proposition}


\subsection{Examples}
\label{sec.example}

In this section, we provide examples for characterizing the conditions in Section~\ref{sec.regularity}. Specifically, consider the following causal Addictive Noise Model (ANM):
\begin{equation*}
    V = g_V(U) + N_V, \,\, \text{for} \,\, V \in \{X,Y,W\},
\end{equation*}
where $g_V$ is the structural function and $N_V\sim f_V$ is the exogenous noise. Then, we have the following results:

\begin{example}[ANM with TV smoothness]
    Suppose that the structural functions $g_Y$ and $g_W$ are differentiable, and that the pdfs $f_Y$ and $f_W$ of the exogenous distributions have absolutely integrable derivatives, then the TV smoothness conditions in Assumption~\ref{asm.tv-smooth} hold.
\end{example}

\begin{example}[ANM with tightness]
    Suppose that the structural functions $g_X$ is invertible, and that the distribution of $N_X$ is tight (see Definition~\ref{def.tight}), then the uniform tightness condition in Proposition~\ref{prop.dis-err unbd} holds for arbitrary compact interval $[a,b]$.
\end{example}

\begin{example}[ANM with completeness]
    Suppose that the structural functions $g_X$ is invertible with a non-zero derivative, and that the exogenous noises $N_X$ and $N_W$ both have non-zero characterization functions, then the completeness conditions in Assumption~\ref{asm.comp} holds.
\end{example}

\xw{It is better to split these examples and put them into appropriate places in the above section.}

To summarize, for causal ANMs, the major sufficient conditions for regularities in Section~\ref{sec.regularity} are: \textbf{i)} the differentiability and invertibility of structural functions, and \textbf{ii)} the tightness of the exogenous distributions and the non-vanishing of their characterization functions. These conditions are mild, with the former satisfied by common analytic functions, and the latter satisfied by, for example, the exponential family of distributions.


\subsection{Algorithm}
\label{sec.alg}

\xw{this algorithm is actually about invertibility, as we do not know in practice how to choose the number of bins. Therefore, it is clearer to present the algorithm for any given discretization number.}

In this section, we introduce an Algorithm~\ref{alg.dis} to practically find a discretization satisfying the properties in Section~\ref{sec.outline}.

Specifically, given $n$ iid samples, we first set the bin numbers for $Y$ and $W$ to $\left\lfloor \log n \right\rfloor$, according to the heuristic rule suggested in \cite{dougherty1995supervised}. Then, we adopt uniform binning to generate data for $\tilde{Y}$ and $\tilde{W}$. 

Next, to generate $\tilde{X}$ satisfying $P(\tilde{W}|\tilde{X})$ being full row rank, we propose an iterative searching strategy. In each step of the search, we generate a new partition point $x_i$ of the domain $\mathcal{X}$ such that the vectors $P(X\leq x_1|\tilde{W}), ..., P(X\leq x_i|\tilde{W})$ are linear independent. We set the total number of bins for $X$ to be larger than that of $W$, in order to make sure $P(\tilde{W}|\tilde{X})$ contains more columns than rows. Finally, we consider an \emph{implicit} binning of the unobserved confounder $U$, which can maintain the conditional independence $X\perp Y|U$ and $X\ind W|U$, as well as the invertibility of $P(\tilde{W}|\tilde{U})$. Thanks to Proposition~\ref{prop.control-err} and Proposition~\ref{prop.rank-dis}, such an implicit binning always exists.

For Algorithm~\ref{alg.dis}, let $[i]$ be the index set $\{1,...,i\}$ and let $[i]\backslash j$ be the set obtained by removing $j$ from $[i]$. We use $x_{[i]}$ in short for $[x_1,...,x_i]^T$. $F(x|\tilde{w})$ is the conditional cdf of $X$ given $\tilde{W}=\tilde{w}$. We use the notations $F(x|\tilde{w}_{[i]}):=[F(x|\tilde{w}_1),...,F(x|\tilde{w}_i)]^T$ and $F(x_{[i]}|\tilde{w}_{[i]}):=[F(x_1|\tilde{w}_{[i]}),...,F(x_i|\tilde{w}_{[i]})]$ for convention. $\mathrm{det}(M)$ is the determinant of the matrix $M$.

\begin{algorithm}[t]
   \caption{Discretization}
   \label{alg.dis}
\begin{flushleft}
\textbf{Input:} Continuous observation of $X$, $Y$, $W$. \\
\textbf{Output:} Discrete data for $\tilde{X}$, $\tilde{Y}$, $\tilde{W}$.
\end{flushleft}
\begin{algorithmic}[1]
    \STATE Uniformly bin $Y,W$ to obtain $\tilde{Y}$, $\tilde{W}$.
    \FOR{$i=1:N$}
        \FOR{$j=1:i$}
            \STATE Estimate $d_j=\mathrm{det}(F(x_{[i-1]}|\tilde{w}_{[i]\backslash j}))$
        \ENDFOR
        \STATE Search $x_i$ s.t. $\sum_{j=1}^i (-1)^{1+j} d_j F(x_i|\tilde{w}_j) \neq 0$.
    \ENDFOR
    \STATE Bin $X$ with the partition $\{[x_i,x_{i+1}]\}_i^N$ to obtain $\tilde{X}$.
    \STATE \textbf{return} $\tilde{X}$, $\tilde{Y}$, $\tilde{W}$.
\end{algorithmic}
\end{algorithm}

==> icml24_para/preliminary_v2.tex <==
\clearpage
\section{Preliminary}

In this section, we introduce the problem setup and backgrounds on proxy variables needed to understand our work.

\textbf{Problem setup.} We consider the problem of identifying the casual relationship between a pairs of variables $X$ and $Y$. The system also includes an unobserved variable $U$, which can be either a sufficient confounder or mediator between $X$ and $Y$. For this case, causal identification is generally not feasible, due to the confounding bias \cite{jager2008confounding} or the mediation bias \cite{hicks2011causal}. To adjust for the bias, we assume the availability of a proxy variable $W$ \cite{kuroki2014measurement} satisfying $X\ind W|U$. In practice, the proxy variable can be a noisy measurement \cite{kuroki2014measurement} or an observed descendant \cite{liu2023causal} of the unobserved variable $U$. We illustrate the relationships between $X$, $Y$, $U$, and $W$ in Figure~\ref{fig.proxy}.

\begin{remark}
    Note that the propose procedure in this paper can apply to cases with a single or multiple proxy variables. We illustrate with the single-proxy case since it is the most challenging one.
\end{remark}

Under the Markovian and faithfulness assumptions \cite{pearl2009causality}, this is equivalent to the problem of testing the causal null hypothesis $\mathbb{H}_0: X\ind Y|U$ using the proxy variable $W$. The $\mathbb{H}_0$ means that there is no causal relationship between $X$ and $Y$, and a rejection of $\mathbb{H}_0$ is, therefore, evidence in favor of causation.

\begin{remark}
    Our procedure can identify whether the causal relationship exists between $X$ and $Y$. For the direction of the causal influence, one can seek for prior knowledge such as time, or adopt causal direction identification methods such as \cite{duong2022bivariate,tu2022optimal}.
\end{remark}

\textbf{Notations.} We adopt the following notational convenience. $(\Omega,\mathcal{F},\mathbb{P})$ is our probability space and $X,Y,U,W$ are all measurable functions, with domains $\mathcal{X},\mathcal{Y},\mathcal{U},$ and $\mathcal{W}$, respectively. We denote the probability law of $X$ as $\mathcal{L}_X:=\mathbb{P}\circ X^{-1}$ and denote the cumulative density function (cdf) as $F_X$. For discrete variables, we denote their levels as $l_{X}, l_{Y}$, etc. We use the the column vector $P(X|y):=[p(x_1|y),...,p(x_{l_{X}}|y)]^T$, the row vector $P(x|Y):=[p(x|y_1),...,p(x|y_{l_{Y}})]$, and the matrix $P(X|Y):=[P(X|y_{1}),...,P(X|y_{l_{Y}})]$ to represent their transition probabilities. We use $I$ to denote the identity matrix. For the continuous case, we assume the domains of all variables are $\mathbb{R}^d$. We denote $\{\mathcal{X}_i\}_{l_X}$ a partition of $\mathcal{X}$ with $l_{X}$ subspaces, satisfying that $\cup_i^I \mathcal{X}_i=\mathcal{X}$ and $\mathcal{X}_i \cap \mathcal{X}_j =\emptyset$ for $i\neq j$. We thereby define the discretized version of $X$ as $\tilde{X}$, assigning $\tilde{X}:=\tilde{x}_i$ iff $X\in\mathcal{X}_i$. Throughout, $n$ denotes the sample size.

\textbf{The procedure described by \cite{miao2018identifying}.} For discrete data, the work of \cite{miao2018identifying} (Section 4) provided a hypothesis testing procedure based on the proxy variable $W$\footnote{Their procedure was originally illustrated with two proxy variables $W$ and $Z$, satisfying $l_{X}l_{Z}>l_{W}$. For the case of a single proxy, we can treat the $Z$ as a constant and require $l_{X}>l_{W}$.}. In details, they connected $\mathbb{H}_0:X\ind Y|U$ with the following equation:
\begin{equation}
    \underbrace{P(y|X)^T}_{\text{response}} = \underbrace{P(W|X)^T}_{\text{design matrix}} \{\underbrace{P(y|U) P(W|U)^{-1}}_{\text{coefficient}}\}^T, 
    \label{eq.miao}
\end{equation}
by noticing that
\begin{align*}
    P(y|X) &= P(y|U) P(U|X) \quad \mathbb{H}_0:X\ind Y|U,\\ 
    P(W|X) &= P(W|U) P(U|X) \quad X\ind W|U.
\end{align*}

Under the assumptions that the matrix $P(W|X)$ has full row rank and $P(W|U)$ is invertible, the system described by Equation~(\ref{eq.miao}) is identifiable under $\mathbb{H}_0$. Therefore, they proposed to test $\mathbb{H}_0$ by testing the identifiability of Equation~(\ref{eq.miao}).

However, for continuous variables, it remain unclear whether such a connection can be built, which involves the the problems of designing discretization processes to ensure the identifiability of Equation~(\ref{eq.miao}), and that of controlling the discretization errors. In the subsequent section, we will provide a comprehensive analysis to answer these questions.


\begin{figure}[t]
    \centering
    \includegraphics[width=.4\textwidth]{icml24_figs/proxy.pdf}
    \caption{Causal diagrams illustrating causal discovery with proxy variables. (a) and (b) respectively represent the cases where $U$ is an unobserved confounder and an unobserved mediator. Note that our procedure is not restricted to these diagrams, but can apply to any scenario satisfying $X\ind W|U$.}
    \label{fig.proxy}
\end{figure}





==> icml24_para/related_work.tex <==
\clearpage
\section{Related works}

\textbf{Proxy variable.} The proxy variable was first introduced by \cite{kuroki2014measurement} for causal effect estimation in the presence of latent confounders. Subsequent works include \cite{tchetgen2020introduction,deaner2021many,sverdrup2023proximal,ghassami2023partial} that relaxed the condition required for identification and \cite{mastouri2021proximal,ghassami2022minimax} that introduced the kernel trick for estimation. For causal discovery, \cite{rojas2017causal} mentioned the proxy variable, where it was more of a motivation since no latent variable is considered. \cite{liu2023causal} employed the proxy variable for time series causal discovery, where the focus is the subsampling problem in temporal data rather than the proxy variable itself. The works most relevant to ours are \cite{miao2018identifying,miao2022identifying}. In \cite{miao2018identifying}, the authors introduced a hypothesis testing procedure that used the proxy variable to test the null hypothesis of no causal effect, however, their procedure is limited to discrete variables. For continuous variables, \cite{miao2022identifying} introduced a testing procedure by examining the existence of solution of the integral equation. However, they rely on parametric assumptions to establish the asymptotic behaviour of the test statistic. \textbf{In contrast}, we proposed a testing procedure based on discretization, which does not rely on any parametric assumption.


\textbf{Bivariate causal discovery.} There are emerging works on bivariate causal discovery, focusing on distinguishing cause from effect by asymmetry properties. These include functional causal models such as the linear non-Gaussian model \cite{shimizu2006linear}, additive noise model \cite{hoyer2008nonlinear,hu2018causal,tu2022optimal}, and post non-linear model \cite{zhang2012identifiability,reick2021estimation}. Other methods are based on the independence of cause and mechanism \cite{sgouritsa2015inference,blobaum2018cause,tagasovska2020distinguishing}, and the stability of causation \cite{janzing2010causal,mitrovic2018causal,duong2022bivariate}. However, these work presume the existence of causal relationships, with only the direction of the causal influence being unknown. Moreover, they usually rely on the assumption of no unobserved confounder to achieve identification. \textbf{In contrast}, we address the fundamental problem of identifying the existence of causal relationships, in the presence of latent confounders. 



==> icml24_para/related_work_v2_mz.tex <==
\section{Related works}


\textbf{Proxy causal learning.} The proximal causal learning was first introduced by \cite{kuroki2014measurement} for causal inference with unobserved confounders, and was later studied in \cite{miao2018identifying, tchetgen2020introduction,deaner2021many,sverdrup2023proximal,ghassami2023partial} for causal effect identification and in \cite{mastouri2021proximal,ghassami2022minimax} for estimation. Recently, \cite{rojas2017causal, liu2023causal} leveraged the proxy variable for causal discovery; however, they respectively focused on causal orientation and time-series causal discovery, which are different from the problem considered in this paper. The works most relevant to ours are \cite{miao2018identifying,miao2022identifying}. In \cite{miao2018identifying}, the authors introduced a hypothesis testing procedure with the proxy variable to adjust for the bias introduced by latent confounders; however, their procedure is limited to discrete variables. For continuous variables, \cite{miao2022identifying} constructed a testing procedure by examining the existence of the solution of the integral equation. However, they rely on parametric assumptions to establish the asymptotic behavior of the test statistic under the null hypothesis. \textbf{In this paper}, we propose a novel testing procedure to effectively identify causal relationships between continuous variables, applicable to both parametric and non-parametric models.


\textbf{Conditional Independence (CI) testing.} There are emerging works considering the CI test problem. Examples include \cite{zhang2012kernel,doran2014permutation,pfister2018kernel,strobl2019approximate} that explored the kernel embedding and the Hilbert-Schimidt Independence Criterion (HSIC) for CI testing, \cite{runge2018conditional,mukherjee2020ccmi,ai2022testing} that used the mutual information as a measure to quantify the CI, and \cite{margaritis2005distribution,neykov2021minimax,warren2021wasserstein} that introduced discretization-based procedures for CI testing. However, these works rely on the assumption that the conditional variable is observable. \textbf{As a contrast}, we proposed a proxy-based hypothesis testing procedure that can test the CI when the the conditional variable is unobserved.


% Kernel-based \cite{zhang2012kernel,doran2014permutation,pfister2018kernel,strobl2019approximate}

% Mutual information-based \cite{runge2018conditional,mukherjee2020ccmi,ai2022testing}

% Discretization-based \cite{margaritis2005distribution,neykov2021minimax,warren2021wasserstein}

% Deep learning-based \cite{sen2017model,shi2021double}

==> icml24_para/related_work_xw.tex <==
\section{Related works}

\textbf{Bivariate causal discovery.} There have been extensive studies in bivariate causal discovery. Within this area, one branch of these works distinguished cause from effect by exploiting asymmetry properties in functional causal models, which include but are not limited to the linear non-Gaussian model \cite{shimizu2006linear}, additive noise model \cite{hoyer2008nonlinear,hu2018causal,tu2022optimal}, and post non-linear model \cite{zhang2012identifiability,reick2021estimation}. Other methods are based on the independence of cause and mechanism \cite{sgouritsa2015inference,blobaum2018cause,tagasovska2020distinguishing}, and the stability of causation \cite{janzing2010causal,mitrovic2018causal,duong2022bivariate}. However, these works focused on learning causal direction, rather than establishing causal relations that can be more fundamental in real applications. Besides, the identifiability in these works relied on the strong ignorability condition, which may not hold in many scenarios. \textbf{In this paper}, we consider the causal relation identification problem in the presence of latent variables. 



\textbf{Proxy causal learning.} The proximal causal learning was first introduced by \cite{kuroki2014measurement} for causal inference with unobserved confounders, and was later studied in \cite{miao2018identifying, tchetgen2020introduction,deaner2021many,sverdrup2023proximal,ghassami2023partial} for causal effect identification and in \cite{mastouri2021proximal,ghassami2022minimax} for estimation. Recently, \cite{rojas2017causal, liu2023causal} leveraged the proxy variable for causal discovery; however, they respectively focused on causal orientation and time-series causal discovery, which are different from the problem considered in this paper. The works most relevant to ours are \cite{miao2018identifying,miao2022identifying}. In \cite{miao2018identifying}, the authors introduced a hypothesis testing procedure with the proxy variable to adjust for the bias introduced by latent confounders; however, their procedure is limited to discrete variables. For continuous variables, \cite{miao2022identifying} constructed a testing procedure by examining the existence of the solution of the integral equation. However, they rely on parametric assumptions to establish the asymptotic behavior of the test statistic under the null hypothesis. \textbf{In this paper}, we propose a novel testing procedure to effectively identify causal relationships between continuous variables, applicable to both parametric and non-parametric models.
